Decoding Recommendation Behaviors of In-Context Learning LLMs Through Gradient Descent

Recently, there has been a growing trend in utilizing large language models (LLMs) for recommender systems, referred to as LLMRec. A notable approach within this trend is not to fine-tune these models directly but instead to leverage In-Context Learning (ICL) methods tailored for LLMRec, denoted as LLM-ICL Rec. Many contemporary techniques focus on harnessing ICL content to enhance LLMRec performance. However, optimizing LLMRec with ICL content presents unresolved challenges. Specifically, two key issues stand out: (1) the limited understanding of why using a few demonstrations without model fine-tuning can lead to better performance compared to zero-shot recommendations. (2) the lack of evaluation metrics for demonstrations in LLM-ICL Rec and the absence of the theoretical analysis and practical design for optimizing the generation of ICL content for recommendation contexts. To address these two main issues, we propose a theoretical model, the LLM-ICL Recommendation Equivalent Gradient Descent model (LRGD) in this paper, which connects recommendation generation with gradient descent dynamics. We demonstrate that the ICL inference process in LLM aligns with the training procedure of its dual model, producing token predictions equivalent to the dual model's testing outputs. Building on these theoretical insights, we propose an evaluation metric for assessing demonstration quality. We integrate perturbations and regularizations in LRGD to enhance the robustness of the recommender system. To further improve demonstration effectiveness, prevent performance collapse, and ensure long-term adaptability, we also propose a two-stage optimization process in practice. Extensive experiments and detailed analysis on three Amazon datasets validate the theoretical equivalence and support the effectiveness of our theoretical analysis and practical module design.

==> 2_preliminary.tex <==
\section{Preliminary}
By exploring the connections between gradient descent and linear attention mechanisms, as well as bridging softmax and linear attention through kernel transformations, we provide the groundwork for the proposed method.


% To better understand the contents in Sec.~\ref{sec:method:theory}, which associates LLM-ICL Rec outputs with gradient descent, we first introduce the method for associating linear attention with gradient descent in this section. Then, we present the kernel-based approach to equivalently relate linear attention with softmax attention.
%为更好地理解之后Section 3中将LLM-ICL Rec输出同梯度下降关联的内容，我们在本节先介绍将线性attention同线性层梯度下降进行关联的方法，然后介绍用核方法将linear attention与softmax attention进行等价关联。


% \subsection{In-context Learning (ICL) in LLMs}
% \label{pre:icl}
% In-context learning (ICL) does not involve re-training or fine-tuning the LLM, but rather directly uses the decoder layers of the LLM Transformer to autoregressively generate content. Therefore, one fundamental assumption in this study is to consider only the decoding process, i.e., the tokens output by LLM inference are generated autoregressively, meaning the newly generated token depends on all the previous tokens. For simplicity, we neglect the residual connections between decoder layers and layer normalization, but the content of positional encoding, masked softmax attention layer, and the feed-forward network (FFN) will be retained. In this context, we consider the following ICL input content: the input $\bm X_{input}$ consists of two parts, the task instruction $\bm X_T$ and the demonstration $\bm X_D$, where $\bm X_T$ is mandatory and $\bm X_D$ is optional. Considering the effects of positional encoding \cite{vaswani2017attention}, we have made certain modifications to the input structure from [ren2024towards][dai2022why]: $\bm X_T$ must appear before $\bm X_D$. The input format can be represented as $\bm X_{input} = [\bm X_T, \bm X_D] \in \mathbb{R}^{d_i \times (N_T + N_D)}$, where $\bm X_T = [\bm x_1, \bm x_2, ..., \bm x_{N_T}] \in \mathbb{R}^{d_i \times N_T}$ and $\bm X_D = [\bm x_{N_{T}+1}, \bm x_{N_{T}+2}, ..., \bm x_{N_{T}+N_{D}}] \in \mathbb{R}^{d_i \times N_D}$. Based on the widely used RoPE (Rotary Position Embedding) \cite{su2024roFormer}, positional encoding is simplified to a single query/key mapping matrix $\bm W_q, \bm W_k \in \mathbb{R}^{d_o \times d_i}$, and the output token corresponding to this mapping, $\bm W_q \bm x_i, \bm W_k \bm x_i \in \mathbb{R}^{d_o}$, is pre-multiplied by a rotation matrix $\bm R_i \in \mathbb{R}^{d_o \times d_o}$, i.e., $\bm q_i = \bm R_i \bm W_q \bm x_i$, $\bm k_i = \bm R_i \bm W_k \bm x_i$, with the rotation matrix $\bm R$ satisfying $\bm R_i^\top \bm R_j = \bm R_{i-j}, \forall i,j \in \mathbb{N_+}$. The value mapping matrix's output token does not consider the rotational effect, i.e., $\bm v_i = \bm W_v \bm x_i$. Therefore, the query, key, and value parts of attention can be represented as follows:
% \[
% \bm Q = [\bm Q_T, \bm Q_D] = [\bm q_1, \bm q_2, ..., \bm q_{N_T + N_D}] \in \mathbb{R}^{d_o \times (N_T + N_D)},
% \]
% \[
% \bm K = [\bm K_T, \bm K_D] = [\bm k_1, \bm k_2, ..., \bm k_{N_T + N_D}] \in \mathbb{R}^{d_o \times (N_T + N_D)},
% \]
% \[
% \bm V = [\bm V_T, \bm V_D] = [\bm v_1, \bm v_2, ..., \bm v_{N_T + N_D}] \in \mathbb{R}^{d_o \times (N_T + N_D)}.
% \]
% Here, we focus on the content of the LLM transformer decoder layer's inference output. For the current input $\bm X_{input}$, its next output token in a single transformer decoder layer can be expressed as (with $\bm \Sigma_{act}$ being the activation function matrix):
% \[
% \bm h_{N_T + N_D + 1} = \bm V \text{softmax}\left(\frac{\bm K^\top \bm q_{N_T + N_D + 1}}{\sqrt{d_o}}\right),
% \]
% \begin{equation}
% \label{eq:pre:trm}
% \hat{\bm x}_{N_T + N_D + 1} = \bm W_{FFN_1} \bm \Sigma_{act}\left(\bm W_{FFN_2} \bm h_{N_T + N_D + 1} + \bm b_{FFN_2}\right) + \bm b_{FFN_1},
% \end{equation}
% where $\bm W_{FFN_1} \in \mathbb{R}^{d_o \times d_h}$, $\bm b_{FFN_1} \in \mathbb{R}^{d_o}$, $\bm W_{FFN_2} \in \mathbb{R}^{d_h \times d_o}$, and $\bm b_{FFN_2} \in \mathbb{R}^{d_h}$ are the transformer FFN parameters. After pretraining and during ICL, these FFN parameters will be fixed.

% The simplified output pattern of the LLM-ICL in a single transformer decoder layer also preserves the possibility for exploration in more complex real-world LLM structures. For instance, it can extend the single-head masked softmax attention to multi-head attention, scenarios like GQA\nc{}, or stack single-layer models to form multi-layer structures, ultimately expanding to real LLM models (such as llama-3 and other multi-layer decoder-only models).

% \subsection{Linear Layer's Gradient Descent is the Dual Form for Linear Attention}
\subsection{Gradient Descent and Linear Attention: A Duality}
Recent studies \cite{ren2024towards, dai2023why, zhang2023batch, yao2024enhancing} have established a connection between linear attention and gradient descent on linear layers, interpreting the gradient descent process as the dual equivalent of linear attention. Consider the simplest single-layer linear model, defined as follows:
$$
f(x) = \bm W_0 \bm x,
$$
where $\bm W_0 \in \mathbb{R}^{d_o \times d_i}$ represents the weight matrix of the linear layer, and $\bm x \in \mathbb{R}^{d_i}$ is the input vector. During training, given an input sequence $[\bm x_k]_{k=1}^{N} \in \mathbb{R}^{d_i\times N}$ and corresponding label sequence $[\bm y_k]_{k=1}^{N} \in \mathbb{R}^{d_o\times N}$, the model is trained by minimizing the loss function $[\mathcal{L}(\hat{\bm y}_k, \bm y_k)]_{k=1}^{N}$, where $[\hat{\bm y}_k]_{k=1}^{N} = [\bm W_0 \bm x_k]_{k=1}^{N} \in \mathbb{R}^{d_o\times N}$ are the predicted outputs. Based on the current losses, an error signal $[\bm e_k]_{k=1}^{N} = [-\beta \frac{\partial \mathcal{L}}{\partial \bm y_k}]_{k=1}^{N} \in \mathbb{R}^{d_o\times N}$ (with $\beta$ being the learning rate) is computed and propagated back through the network during the backpropagation process, resulting in updates to the model parameters from $\bm W_0$ to $\bm W'$. The update rule is given by:
$$
\bm W' = \bm W_0 + \Delta \bm W = \bm W_0 + \sum_{k=1}^{N} \bm e_k \otimes \bm x_k.
$$
where $\otimes$ denotes the outer product of vectors.

Next, we examine the content of linear attention (LA). Let $\bm V=[\bm v_k]_{k=1}^{N}, \bm K =[\bm k_k]_{k=1}^{N}  \in \mathbb{R}^{d_o \times N}$ represent the value and key matrices, respectively. Given a query vector $\bm q\in \mathbb{R}^{d_o}$, linear attention can be expressed as:
$$
\mathrm{LA}(\bm V, \bm K, \bm q) = \bm V \bm K^\top \bm q  = \left( \sum_{k=1}^{N} \bm v_k \otimes \bm k_k \right) \bm q.
$$
For a trained linear layer model, during the test phase, given an input
$\bm x'\in \mathbb{R}^{d_i}$ 
we can derive the equivalent form of gradient descent and linear attention from the above equations:
$$
f(\bm x') = \bm W' \bm x' = (\bm W_0 + \sum_{k=1}^{N} \bm e_k \otimes \bm x_k) \bm x' = \bm W_0 \bm x' + \mathrm{LA}(\bm E, \bm X, \bm x').
$$
This demonstrates that the gradient descent process in training a linear model can be interpreted as a linear attention mechanism, with the model parameters $\bm W'$ adjusted by the error terms and the resulting attention computation during inference.


% Existing works \cite{ren2024towards, dai2023why, zhang2023batch, yao2024enhancing} associate linear attention with gradient descent on linear layers, viewing gradient descent on the linear layer as the dual equivalent form of linear attention. The simplest single-layer linear model can be defined as:
% $$
% f(x) = \bm W_0 \bm x,
% $$
% where $\bm W_0 \in \mathbb{R}^{d_o \times d_i}$ is the parameter of the linear mapping layer, and $\bm x \in \mathbb{R}^{d_i}$ is the input vector. During training, given an input vector sequence $[\bm x_k]_{k=1}^{N} \in \mathbb{R}^{d_i\times N}$ and a label sequence $[\bm y_k]_{k=1}^{N} \in \mathbb{R}^{d_o\times N}$, the linear model can be trained by computing the specific loss $[\mathcal{L}(\hat{\bm y}_k, \bm y_k)]_{k=1}^{N}$ based on predicted outputs $[\hat{\bm y}_k]_{k=1}^{N} = [\bm W_0 \bm x_k]_{k=1}^{N} \in \mathbb{R}^{d_o\times N}$ and the given labels. Based on the current losses, an error signal $[\bm e_k]_{k=1}^{N} = [-\beta \frac{\partial \mathcal{L}}{\partial \bm y_k}]_{k=1}^{N} \in \mathbb{R}^{d_o\times N}$ ($\beta$ is the learning rate) is generated and passed back during the backpropagation process, updating the model parameters from $\bm W_0$ to $\bm W'$. The specific optimization form is as follows ($\otimes$ denotes the outer product of vectors):
% $$
% \bm W' = \bm W_0 + \Delta \bm W = \bm W_0 + \sum_{k=1}^{N} \bm e_k \otimes \bm x_k.
% $$

% Meanwhile, we consider analyzing the content of linear attention (LA). Let %$, \in \mathbb{R}^{d_i}$ be the $N$ value and key vectors, respectively, and their corresponding 
% value and key matrices be $\bm V=[\bm v_k]_{k=1}^{N}, \bm K =[\bm k_k]_{k=1}^{N}  \in \mathbb{R}^{d_i \times N}$. Given a query vector $\bm q\in \mathbb{R}^{d_i} $, linear attention can be expressed as the sum of the products with $\bm V$ and $\bm K$, as follows:
% $$
% \mathrm{LA}(\bm V, \bm K, \bm q) = \bm V \bm K^\top \bm q  = \left( \sum_{k=1}^{N} \bm v_k \otimes \bm k_k \right) \bm q.
% $$
% Therefore, for the trained linear layer model, given the input $\bm x'\in \mathbb{R}^{d_i}$ during the test phase, we can derive the equivalent form of gradient descent and linear attention from the above equations:
% $$
% f(\bm x') = \bm W' \bm x' = (\bm W_0 + \sum_{k=1}^{N} \bm e_k \otimes \bm x_k) \bm x' = \bm W_0 \bm x' + \mathrm{LA}(\bm E, \bm X, \bm x').
% $$

\subsection{Connecting Softmax Attention to Linear Attention with Kernels}
\label{sec:connect}
Due to the nonlinear normalization differences between softmax attention in the transformer decoder layers of LLMs and linear attention, we follow \cite{ren2024towards} to approximate softmax attention using kernel methods, with the aim of transforming the softmax component into an equivalent linear attention form. 

We begin by expressing the softmax function as the product of an unnormalized exponential term and a normalization vector \(\bm c\):
$$
\mathrm{softmax}(\bm X_1^\top \bm X_2) = \exp(\bm X_1^\top \bm X_2) \bm c,
$$
where \(\bm X_1 \in \mathbb{R}^{d_o \times d_1}\), \(\bm X_2 \in \mathbb{R}^{d_o \times d_2}\), \(\exp(\cdot)\) denotes element-wise exponentiation, and \(\bm c = \mathrm{diag}(\bm 1_{d_2 \times d_1} \exp(\bm X_1^\top \bm X_2))^{-1} \in \mathbb{R}^{d_2}\) is the normalization vector.

% For individual vectors $\bm x, \bm y \in \mathbb{R}^{d_o}$, we can rewrite $\mathrm{exp}(\bm x, \bm y)$ as:
% $$
% \mathrm{exp}(\bm x, \bm y) = e^{\bm x^\top \bm y} = e^{||\bm x||^2_2 / 2} \cdot e^{-||\bm x - \bm y||^2_2 / 2} \cdot e^{||\bm y||^2_2 / 2},
% $$
% where $e^{-||\bm x - \bm y||^2_2 / 2}$ represents the common Radial Basis Function (RBF) kernel with \(\sigma^2 = 1\). This kernel can be approximated using various kernel approximation techniques. A common approach is to use the following:
% $$
% e^{-||\bm x - \bm y||^2_2 / 2} = \phi_0(\bm x)^\top \phi_0(\bm y),
% $$
% where 
% $$
% \phi_0(\bm x) = \frac{1}{\sqrt{D}} \left( \sin(\bm u_1^\top \bm x), \dots, \sin(\bm u_{D/2}^\top \bm x), \cos(\bm u_1^\top \bm x), \dots, \cos(\bm u_{D/2}^\top \bm x) \right)^\top,
% $$
% and \(D\) is a constant (typically around 100), with \(\bm u_i\) being random vectors drawn from \(\mathcal{N}(0, \bm I_{d_o})\). The mapping \(\phi_0(\bm x)\) transforms \(\bm x \in \mathbb{R}^{d_o}\) to \(\mathbb{R}^{d_D}\).
% Thus, the exponential kernel approximation \(\phi(\bm x): \mathbb{R}^{d_o} \to \mathbb{R}^{d_D}\) can be written as:
% $$
% \mathrm{exp}(\bm x, \bm y) = \phi(\bm{x})^\top \phi(\bm{y})
% ,\ \phi(\bm{x}) = e^{||\bm x||^2_2 / 2} \phi_0(\bm x).
% $$
% This kernel approximation is consistent with the form proposed in \cite{choromanski2020rethinking} and will be utilized in this paper.
For individual vectors $\bm x, \bm y \in \mathbb{R}^{d_o}$, we can rewrite $\mathrm{exp}(\bm x, \bm y)$ with random Fourier mapping $\phi(\bm \cdot)$ based on the approximation of common RBF kernel\cite{rahimi2007random} with $\sigma^2=1$ as:
\begin{equation}
\label{eq:pre:kernel}
\mathrm{exp}(\bm x, \bm y) = e^{\bm x^\top \bm y} = \phi(\bm x)^\top \phi(\bm y),
\end{equation}
where 
$$
\phi(\bm x) = \frac{ e^{||\bm x||^2_2 / 2}}{\sqrt{D}} \left( \sin(\bm u_1^\top \bm x), .., \sin(\bm u_{D/2}^\top \bm x), \cos(\bm u_1^\top \bm x), .., \cos(\bm u_{D/2}^\top \bm x) \right)^\top,
$$
and \(D\) is a constant (typically around 100), with \(\bm u_i\) being random vectors drawn from \(\mathcal{N}(0, \sigma\bm I_{d_o})\). The mapping \(\phi(\bm x)\) transforms \(\bm x \in \mathbb{R}^{d_o}\) to \(\mathbb{R}^{d_D}\). $\phi(\bm \cdot)$ is consistent with the form proposed in \cite{choromanski2020rethinking} and will be utilized in this paper.


After applying the $\phi(\bm \cdot)$ to the individual vectors in \(\bm X_1\) and \(\bm X_2\) as described above, we obtain:
$$
\exp(\bm X_1^\top \bm X_2) = \phi(\bm X_1)^\top \phi(\bm X_2).
$$
Thus, the approximate form of the softmax function is:
$$
\mathrm{softmax}(\bm X_1^\top \bm X_2) = \phi(\bm X_1)^\top \phi(\bm X_2) \bm c,
$$
where \(\bm c = \mathrm{diag}(\bm 1_{d_2 \times d_1} \phi(\bm X_1)^\top \phi(\bm X_2))^{-1} \in \mathbb{R}^{d_2}\).

Finally, the output of the softmax attention can be rewritten as:
\begin{equation*}
% \label{eq:pre:kernel}
    \bm h = \bm V \, \mathrm{softmax}\left(\frac{\bm K^\top \bm q}{\sqrt{d_o}}\right) = c\bm V \, \phi(\bm K)^\top \phi(\bm q) = \mathrm{LA}(c \bm V, \phi(\bm K)^\top, \phi(\bm q)),
\end{equation*}
where
$c = \left( \bm 1_{N}^\top \phi(\bm K)^\top \phi(\bm q) \right)^{-1} \in \mathbb{R}^1
$, $\bm q \in \mathbb{R}^{d_i}$ is query vector.

This demonstrates how softmax attention in transformers can be approximated using kernel methods, transforming the softmax component into a linear attention form. 


% Due to the nonlinear normalization difference between softmax attention in the transformer decoder layer of real-world LLMs and linear attention, we follow the method in \cite{ren2024towards} to modify softmax attention using kernel approximation, aiming to transform the softmax part into the equivalent form of linear attention. Firstly, we treat the softmax function as the product of the unnormalized exponential term and the normalization vector $\bm c$, i.e., 
% $$
% \mathrm{softmax}(\bm X_1^\top \bm X_2) = \mathrm{exp}(\bm X_1^\top \bm X_2)\bm c,
% $$
% where $\bm X_1 \in \mathbb{R}^{d_o \times d_1}$, $\bm X_2 \in \mathbb{R}^{d_o \times d_2}$, $\mathrm{exp}(\cdot)$ denotes element-wise exponentiation, and $\bm c = \mathrm{diag}(\bm 1_{d_2 \times d_1} \mathrm{exp}(\bm X_1^\top \bm X_2))^{-1} \in \mathbb{R}^{d_2}$ is the normalization vector.

% For individual vectors $\bm x, \bm y \in \mathbb{R}^{d_o}$, we can rewrite $\mathrm{exp}(\bm x, \bm y)$ as:
% $$
% \mathrm{exp}(\bm x, \bm y) = e^{\bm x^\top \bm y} = e^{||\bm x||^2_2 / 2} \cdot e^{-||\bm x - \bm y||^2_2 / 2} \cdot e^{||\bm y||^2_2 / 2},
% $$
% where $e^{||\bm x - \bm y||^2_2 / 2}$ represents the common RBF kernel with $\sigma^2 = 1$. This kernel can be approximated using many existing kernel approximation methods. A common approximation method is:
% $$
% e^{||\bm x - \bm y||^2_2 / 2} = \phi_0(\bm x)^\top \phi_0(\bm y),
% $$
% $$
% \phi_0(\bm x) = \frac{1}{\sqrt{D}} \left( \mathrm{sin}(\bm{u}_1^\top \bm{x}), ..., \mathrm{sin}(\bm{u}_{D/2}^\top \bm{x}), \mathrm{cos}(\bm{u}_1^\top \bm{x}), ..., \mathrm{cos}(\bm{u}_{D/2}^\top \bm{x}) \right)^\top,
% $$
% where $D$ is a constant (typically around 100), with $\bm u_i$ being random vectors drawn from $\mathcal{N}(0, \bm I_{d_o})$, and $\phi_0(\bm x): \mathbb{R}^{d_o}\to\mathbb{R}^{d_D}$.

% Thus, the exponential kernel approximation $\phi(\bm x):\mathbb{R}^{d_o}\to\mathbb{R}^{d_D}$ can be:
% $$
% \mathrm{exp}(\bm x, \bm y) = \phi(\bm{x})^\top \phi(\bm{y})
% ,\ \phi(\bm{x}) = e^{||\bm x||^2_2 / 2} \phi_0(\bm x).
% $$
% This kernel is also consistent with the form proposed in \cite{choromanski2020rethinking}, and will be used in this paper.

% After applying kernel approximation mappings to the individual vectors in $\bm X_1, \bm X_2$ as defined former part, we have:
% $$
% \mathrm{exp}(\bm X_1^\top \bm X_2) = \phi(\bm X_1)^\top \phi(\bm X_2).
% $$
% Thus, we can obtain the approximate form of the softmax function:
% $$
% \mathrm{softmax}(\bm X_1^\top \bm X_2) = \phi(\bm X_1)^\top \phi(\bm X_2) \bm c,
% $$
% where $\bm c = \mathrm{diag}(\bm 1_{d_2 \times d_1} \phi(\bm X_1)^\top \phi(\bm X_2))^{-1} \in \mathbb{R}^{d_2}$.

% Finally, the softmax attention output can be rewritten as:
% \begin{equation}
% \label{eq:pre:kernel}
%     \bm h = \bm V \, \mathrm{softmax}\left(\frac{\bm K^\top \bm q}{\sqrt{d_o}}\right) = c\bm V \, \phi(\bm K)^\top \phi(\bm q) = \mathrm{LA}(c \bm V, \phi(\bm K)^\top, \phi(\bm q)),
% \end{equation}
% where
% $c = \left( \bm 1_{N}^\top \phi(\bm K)^\top \phi(\bm q) \right)^{-1} \in \mathbb{R}^1
% $, $\bm q \in \mathbb{R}^{d_i}$ is query vector.


==> 4.1_experiment_settings.tex <==
\textbf{Dataset.} Following~\cite{zheng2024adapting}, we conduct our experiments on three subsets of the Amazon dataset~\cite{ni2019justifying}: ``Arts'', ``Video'', and ``Instruments''\footnote{Note that ``Arts'', ``Games'' and ``Instruments'' represent the abbreviations of ``Arts, Crafts and Sewing'', ``Video Games'' and ``Musical Instruments'' respectively in the Amazon Review dataset (2018).}. We follow the preprocessing strategy in~\cite{zheng2024adapting,qin2024enhancing}, with the detailed statistics of the pre-processed datasets presented in Tab.~\ref{tab:dataset}.


% \qwc{Each item has attributes that reflect both explicit user preferences (e.g., titles) and implicit preferences (e.g., brands and categories). Following~\cite{zheng2024adapting}, we provide the SeqRec format and filter out unpopular users and items with fewer than five interactions. The statistics of the pre-processed datasets are summarized in Table~\ref{tab:dataset}.
% }
% can be found in App.~\ref{app:dataset}.\\

% \begin{table}[!htbp]
% \centering
% \setlength{\tabcolsep}{3.2pt}
% \caption{Statistics of the 3 pre-processed datasets. Avg. len represents the average length of interacted items per user.}
% \label{tab:dataset}
% {\small\begin{tabular}{l|p{2cm}|p{2cm}|p{2cm}}
% \toprule
%          & \textbf{Arts}    & \textbf{Games}   & \textbf{Instruments} \\ \midrule
% \#Users & 55970   & 55145   & 27404       \\
% \#Items & 22612   & 17287   & 10450       \\
% Avg. len & 8.80    & 9.01    & 8.41        \\
% Sparsity & 99.96\% & 99.95\% & 99.92\%     \\ \bottomrule
% \end{tabular}}
% \end{table}


% \xy{We evaluate our proposed method using three subsets of the Amazon review dataset~\cite{ni2019justifying}:  ``Arts, Crafts and Sewin'', ``Video Games'', and ``Musical Instruments''. 
% In the following text, we will concisely refer to them as ``Arts'', ``Games'', and ``Instruments'', respectively. These datasets contains user reviews from May 1996 to Oct 2018. Each item in the datasets includes a title and a description with side information (e.g. brands, categories). Following previous work~\cite{zheng2024adapting}, we exclude users and items that have fewer than 5 interactions. Subsequently, we construct user behavior sequences based on chronological order. %We evaluated our proposed approach on three subsets of Amazon review data~\cite{ni2019justifying}, including “Musical Instruments”, “Arts, Crafts and Sewing”, and “Video Games”. All three datasets contain user review data from May 1996 to October 2018. Each item in the dataset is associated with a title and a description. Following previous work~\cite{zheng2024adapting}, we filtered out unpopular users and items with less than 5 interactions. Then, we create user behavior sequences based on the chronological order.
% Details of the pre-processed datasets statistics can be found in App.~\ref{app:dataset}}
\textbf{Baselines.}
We adopt three types of representative SeqRec methods as baselines to validate the effectiveness of \texttt{MoRE}:
% We adopt three categories of baselines: traditional deep recommendation methods (e.g., SASRec~\cite{kang2018self}, etc.), training-free LLM-based methods (e.g., LLM4RS~\cite{dai2023uncovering}, etc.), and training-required LLM-based methods (e.g., Re2LLM~\cite{wang2024re2llm}, etc.). See App.~\ref{app:details:Baselines} for details. 
% \\
% We adopt the following representative SeqRec models as baselines for comparison with \texttt{MoRE}:
% \textbf{Caser}~\cite{tang2018personalized} is a CNN-based method that models user-item interactions as sequences to capture both local and global patterns.
% \textbf{GRU4Rec}~\cite{hidasi2015session} is an RNN-based SeqRec model with GRU modeling the user behavior sequences.
% \textbf{BERT4Rec}~\cite{sun2019bert4rec} adopts a bidirectional Transformer model and incorporates a masked prediction approach to capture the patterns in item sequences. 
% \textbf{SASRec}~\cite{kang2018self} exploits a unidirectional Transformer-based neural network to model the item sequences and predict the next item. 
% \textbf{FDSA}~\cite{zhang2019feature}  models both item-level and feature-level transition patterns through a dual self-attention mechanism. \textbf{LLM4RS}~\cite{dai2023uncovering} investigates the potential of LLMs in enhancing recommendation capabilities by aligning it with traditional information retrieval (IR) ranking techniques, specifically point-wise, pair-wise, and list-wise ranking. 
% \textbf{LLMRank}~\cite{hou2024large} leverages LLMs for zero-shot ranking in recommendation tasks, addressing challenges related to interaction order and bias through specialized prompting techniques.
% \textbf{LC-Rec}\footnote{To ensure a fair comparison, we ensured that each model's recommendation process for each user was based on the same item candidate set of size 50. However, since LC-Rec's training is based on the full item set as the shared candidate set, it is challenging to guarantee that the model does not output items outside the size 50 candidate set for a user solely through the prompt. To address this, we implemented output constraints for the generation process of LC-Rec, ensuring that it outputs only the permitted 50 items for each user}~\cite{zheng2024adapting} is  a fine-tuning LLMREC method that incorporates collaborative filtering information by expanding the vocabulary space with special token embeddings. It is currently the state-of-the-art method for LLMREC in the full-candidate SeqRec setting.
% % is a large language model recommendation method that incorporates collaborative filtering information. LC-Rec expands the vocabulary space of the large language model backbone by introducing learnable item IDs and special token embeddings for training. LC-Rec designs various recommendation question-answering tasks involving item IDs, enabling the model to understand the relationship between special tokens and text tokens but incurring significant training costs. It is currently the state-of-the-art method for large model recommendations in the full candidate set setting.
% \textbf{BinLLM}\footnote{BinLLM introduces collaborative filtering knowledge to LLMs from the perspective of input text. However, it can only predict the relationship between one user and one item at a time, necessitating multiple inferences to provide recommendations for a user. To ensure a fair comparison, we modified the format of its prompt and reproduced it to make it output a list.}~\cite{zhang2024text} is a fine-tuning LLMREC method that incorporates collaborative filtering information by injecting user and item embeddings as binary text sequences into the LLM's input, without modifying the model's vocabulary space. It is currently the state-of-the-art method for LLMREC conditioned on the given user-item pair.
% % is a LLMREC method that incorporates collaborative filtering information without modifying the vocabulary space. Researchers of BinLLM believe that altering the model's vocabulary space would compromise the original generation capabilities of LLMs, leading to a loss in performance. They propose a fine-tuning method that injects user and item embeddings as binary text sequences into the LLM's input, attempting to leverage the implicit "logical AND" capability of the LLM to understand and capture the relationship between the given user and the target item.
%  \textbf{Re2LLM}~\cite{wang2024re2llm} is a reflection-based LLMREC method. It first constructs a reflection knowledge base (KB) with domain knowledge, and then retrieves suitable text in the fixed KB to insert into the LLM's input, adapting the LLM to session-based recommendation.

(1) \textbf{Traditional deep learning recommendation models} include:
\textbf{Caser}~\cite{tang2018personalized}, a CNN-based model that treats user-item interactions as sequences to capture both local and global patterns;
\textbf{GRU4Rec}~\cite{hidasi2015session}, an RNN-based model that leverages GRUs to model user behavior sequences;
\textbf{BERT4Rec}~\cite{sun2019bert4rec}, a bidirectional Transformer-based model that employs a masked item prediction strategy to learn sequence patterns.
\textbf{SASRec}~\cite{kang2018self}, a unidirectional Transformer-based model designed to model item sequences and predict the next item.
\textbf{FDSA}~\cite{zhang2019feature}, utilizing a dual self-attention mechanism to jointly model item-level and feature-level transition patterns.
% \textbf{Caser}~\cite{tang2018personalized} is a CNN-based method that models user-item interactions as sequences to capture both local and global patterns. \textbf{GRU4Rec}~\cite{hidasi2015session} is an RNN-based SeqRec model with GRU modeling the user behavior sequences. \textbf{BERT4Rec}~\cite{sun2019bert4rec} adopts a bidirectional Transformer model and incorporates a masked prediction approach to capture the patterns in item sequences. \textbf{SASRec}~\cite{kang2018self} exploits a unidirectional Transformer-based neural network to model the item sequences and predict the next item. \textbf{FDSA}~\cite{zhang2019feature}  models both item-level and feature-level transition patterns through a dual self-attention mechanism. 


(2) \textbf{Training-free LLM-based methods}, i.e.,
the prompt-based recommendation methods include: \textbf{LLM4RS}~\cite{dai2023uncovering}  aligns LLMs with traditional information retrieval (IR) ranking techniques, specifically point-wise, pair-wise, and list-wise ranking. \textbf{LLMRank}~\cite{hou2024large} leverages LLMs for zero-shot ranking in recommendation tasks through specialized prompting techniques.

(3) \textbf{Training-required LLM-based methods} include: \textbf{LC-Rec}
% \footnote{\xy{NEED TO CHANGE FULL CANDIDATE: To ensure a fair comparison, we ensured that each model's recommendation process for each user was based on the same item candidate set of size 50. However, since LC-Rec's training is based on the full item set as the shared candidate set, it is challenging to guarantee that the model does not output items outside the size 50 candidate set for a user solely through the prompt. To address this, we implemented output constraints for the generation process of LC-Rec, ensuring that it outputs only the permitted 50 items for each user}}
~\cite{zheng2024adapting} fine-tunes a LLM and incorporates collaborative filtering information by expanding the vocabulary with special tokens.
\textbf{TALLRec}~\cite{bao2023tallrec} adopts instruction fine-tuning by providing a text description and selecting one target through LLM.
\textbf{BinLLM}~\cite{zhang2024text} fine-tunes a LLM with binary sequence texts as user and item embeddings, without altering its vocabulary. \textbf{Re2LLM}~\cite{wang2024re2llm} constructs a fixed reflection pool to provide proper suggestions when recommend.  \textbf{LLaRA} integrates both world knowledge and behavioral patterns into hybrid item representations with LoRA tuning. 
\textbf{A-LLMREC}~\cite{hgsb} inserts CF embeddings into the LLM vocabulary through an alignment module.
% \textbf{BinLLM}
% \footnote{BinLLM can only predict the relationship between one user and one item at a time, necessitating multiple inferences to provide recommendations for a user. To ensure a fair comparison, we modified the format of its prompt and reproduced it to make it output a list.}
% ~\cite{zhang2024text} is a fine-tuning LLMREC method that incorporates collaborative filtering information by injecting user and item embeddings as binary text sequences into the LLM's input, without modifying the model's vocabulary space. It is currently the state-of-the-art method for LLMREC conditioned on the given user-item pair. \textbf{Re2LLM}~\cite{wang2024re2llm} is a reflection-based LLMREC method. It first constructs a reflection knowledge base (KB) with domain knowledge, and then retrieves suitable text in the fixed KB to insert into the LLM's input, adapting the LLM to session-based recommendation.

\textbf{Evaluation Metrics.} 
% To evaluate the performance of
% \texttt{MoRE} and other baselines,
We adopt two widely used metrics, top-$k$ Hit Ratio (HR@$k$) and Normalized Discounted Cumulative Gain (NDCG@$k$), with $k\in\{5, 10\}$. Following~\cite{zheng2024adapting, zhou2022filter}, we employ the leave-one-out strategy for the obtaining of training, validation, and test data. Specifically, for each user behavior sequence, the last item is used as the test data, the penultimate item is used as the validation data, and the remaining interaction records are used for training. Following~\cite{hou2024large,wang2024re2llm,hgsb,liao2024llara}, we randomly sample $|\mathcal{C}_u|-1$ negative items to construct $|\mathcal{C}_u|$ candidates with 1 target item for each user.
Following ~\cite{wang2024re2llm},  $|\mathcal{C}_u|$ is set to 50 for all methods.  \texttt{MoRE} and all baselines are required to give a top-10 ranked predictions for the next item of each user.
Please note that for baseline methods that can only predict one single item without ranking capabilities (i.e., TALLRec, BinLLM, LLaRA, and A-LLMREC), we've attempted to adjust these baselines to obtain metrics more than hit@1. However, their performances severely declined after the adjustments. To ensure a fair comparison, we adhere to their respective training process and only report their hit@1.
% \footnote{For baseline models that can only predict one single item without ranking capabilities (e.g., TALLRec, BinLLM, LLaRA, and A-LLMREC), we've attempted to adjust these baselines to obtain metrics other than hit@1. However, their performance severely declined after the adjustments. To ensure a fair comparison, we adhere to their respective training process and only report their hit@1.}

%\scl{this is an example of text}
\textbf{Implementation Details.}
%We use LLaMa-3\footnote{https://huggingface.co/gradientai/Meta-Llama-3-8B-bf16. }~\cite{dubey2024llama} as the LLM backbone for \texttt{MoRE} and LLM-based baselines.   Implementation details can be found in App.~\ref{app:details:imp}.
We use LLaMa-3-8B-Instruct~\cite{dubey2024llama} as the  backbone for all LLM-based methods. Following~\cite{hou2024large,hgsb,bao2023tallrec,wang2024re2llm}, we respectively perform random sampling from three datasets for efficiency, and exclude users with overly long interaction sequences and then randomly we sample 1,000 users, with items remaining unchanged. For simplicity, we trained DMF\footnote{Please note that other CF models can be easily incorporated into \texttt{MoRE}.}~\cite{xue2017deep} with an embedding size of 64 to provide CF scores for reflection (Sec.~\ref{sec:multi:perspective}) and to assist with user clustering within refining (Sec.~\ref{sec:meta:main}). The number of clusters is set to 20.
%For simplicity, we train DMF~\cite{xue2017deep} to provide CF score for reflection (Sec.~\ref{sec:multi:perspective}). The embedding size is 64. This DMF model is also used to implement the user clustering mentioned in the Refining process in Sec.~\ref{sec:meta:main}. DMF model provides embedding vectors for users in the three datasets, and these embeddings are used to cluster the users in each dataset. We define 20 clusters for each dataset, with the cluster ID being an integer in $[0, 19]$, inclusive. For Iteration process in Sec.~\ref{sec:meta:main}, we set the total iteration to 15, and impacts of Refining and Iteration can be found in Sec.~\ref{sec:exp:ri}.}
We use RecBole~\cite{zhao2021recbole} to implement all traditional SeqRec baselines (e.g. SASRec) with the Adam optimizer and grid search where the embedding size is tuned among \{32, 64, 128\}; the learning rate is tuned among \{$1e^{-2}, 1e^{-3},1e^{-4}$\}; and the batch size is tuned among \{1024, 2048, 4096\}.
% \footnote{Grid search space was set as: \textit{embedding size} : \{32, 64, 128\}, \textit{learning rate} : \{$1e^{-2}, 1e^{-3},1e^{-4}$\} and \textit{batch size} : \{1024, 2048, 4096\}.}. 
For LLM baselines, we follow the origin settings and make proper adaption to our scenario. For constrained generative retrieval baselines, we construct the constraints following the corresponding setting. For baselines that only provide top-1 prediction, we provide the same candidate set as MoRE and, following the original settings, do not require predictions beyond the top-1, thereby obtaining their best top-1 results under a lower task difficulty. For baselines that only answer yes or no, we adjust it to the next item in the same way as LLaRA~\cite{liao2024llara}.
All experiments are run on a 4$\times$A800-PCIE-80GB GPUs server.

==> backup.tex <==
\section{\texttt{MoRE}: The Proposed Framework}
\subsection{Problem Formulation}
In SeqRec, let $\mathcal{V} = \{v_1, v_2, ..., v_{|\mathcal{V}|}\}$ denote the item set, $\mathcal{U} = \{u_1, u_2, ..., u_{|\mathcal{U}|}\}$ denote the user set, and 
$\mathcal{S}_u=[v_1^u, v_2^u, ..., v_t^u]$ denote the interaction sequence in chronological order for user $u\in\mathcal{U}$, where $v_t^{u} \in \mathcal{V}$ is the item that $u$ has interacted with at time step $t$.
% and $L$ is the length of the interaction sequence. 
The goal of this task is to predict the item that $u$ will interact with at $t+1$ given $\mathcal{S}_u$:
\begin{equation}
\label{eq:rec}
    \hat{v}=\operatorname*{arg\,max}_{v\in \mathcal{V}}\Pr(v_{t+1}^{u} = v \mid \mathcal{S}_u).
\end{equation}
In this study, we focus on the LLM-based recommendation. Following~\cite{dai2023uncovering,hou2024large}, we adopt LLM to directly make the prediction as follows:
\begin{equation}
\label{eq:llm4rec}
    % i^*=\text{LLM}(P,u,\mathcal{S}_u),
\hat{\mathcal{O}}_u=\mathrm{LLM}_{\mathrm{REC}}(P(u, \mathcal{S}_u, \mathcal{C}_u)), \hat{\mathcal{O}}_u\subseteq\mathcal{C}_u,
\end{equation}
where $P$ denotes the manually crafted recommendation prompt; $\mathcal{C}_u$ and $\mathcal{O}_u$ respectively denote the candidate and predicted item list for $u$; all the parameters are concatenated in the text form; and $\mathrm{LLM}_{\mathrm{REC}}$, the LLM for recommendation, is frozen. 
Please note that reflections are essentially a form of prompts generated by the LLM based on interaction history.
Therefore, replacing $P()$ with $Ref()$ in Eq.~\ref{eq:llm4rec} denotes the reflection-based recommendation.
% \xy{In this section, we introduce our proposed MoRE method. MoRE consists of two key modules: the Multi-Perspective Reflection Experts and the Meta-Reflector equipped with refining iteration and PPO selector.
\subsection{Overall Framework}
We propose \texttt{MoRE}, a novel reflection-based framework, to model the dynamic preferences in LLM-based SeqRec. As shown in Fig.~\ref{fig:main}, \texttt{MoRE} consist of two key modules:

\begin{figure*}[t]
    % \setlength{\belowcaptionskip}{-10pt}
    \centering
\includegraphics[width=0.9\textwidth]{fig_updated/fig2.pdf}
    \caption{
    The overall architecture of our \texttt{MoRE} framework. \texttt{MoRE} incorporates multi-perspective reflectors to generate reflections offline~\ding{172} and a meta-reflector to self-improve these reflections~\ding{173} and learn to select the most appropriate one~\ding{174}. During online recommendation~\ding{175}, the meta-reflector selects the suitable reflections for the current user.
    % The overall architecture of our proposed \texttt{MoRE} framework. The overall approach includes a basic recommendation flow (grey), Multi-Perspective Reflectors (green) for the generation of reflections with different perspectives, Meta-Reflector's memory Reflection Memory Maintenance (yellow) for the good reflection example's selection and re-generation, and Reflection Selection (blue) for choosing the proper perspective of reflection for specific users.
    }
    \label{fig:main}
\end{figure*}

\textbf{Multi-Perspective Reflectors.} As discussed in Sec.~\ref{sec:intro}, user preferences are often implicitly embedded in the attributes of items and can be inferred through collaborative filtering information. Therefore, \texttt{MoRE} incorporates this module to drive LLMs to generate reflections from the perspectives of a user's explicit preferences, implicit preferences, and collaborative filtering information. These derived reflections based on historical interactions are considered as hints to enhance LLMs' future recommendations. The details of this module will be introduced in Sec.~\ref{sec:multi:perspective}.

% multiple perspectives given a user interaction history.
% corresponding recommendation reflection text content from different perspectives, including the user's explicit preferences, implicit preferences, and collaborative filtering information from user-item interactions. Its aim is to personalize the approach from specific rather than overly broad angles, generating highly personalized corrective recommendation reflections for the current user, avoiding overgeneralization.%generic statements that may be off-putting to users.

\textbf{Meta-Reflector.} 
This module has two main objectives. First, it maintains three memory banks for each user to collect reflections from the corresponding three reflectors and uses a refining-and-iteration strategy to self-improve the reflections and update the current reflection memories for each user. Second, it is responsible for deciding which of the three perspectives of reflection should be chosen to enhance the current recommendation at each step for the user. This decision-making process is formulated as a contextual bandit problem~\cite{Li2010Contextual}. These two parts will be elaborated in Sec.~\ref{sec:meta:main} and Sec.~\ref{sec:meta:selection}, respectively.
% equipped with refining iteration and PPO selector, is tasked with selecting appropriate examples from the reflections generated by the various reflection expert groups and effectively extracting, filtering, and iterating them. Subsequently, PPO algorithm~\cite{schulman2017proximal} is used to train a lightweight reflection perspective selector to further enhance the re-recommendation effects, avoiding excessive fine-tuning training costs, while reducing inference consumption %and eliminating potential hallucinations 
% during the inference process of the reflection expert s. Ultimately, LLMREC uses high-quality reflections selected and generated by MoRE to enhance its understanding of different users, providing them with higher quality, personalized recommendations. The overall architecture of MoRE is illustrated in Figure XXX.

\subsection{Multi-Perspective Reflections Generation}
\label{sec:multi:perspective}
As illustrated in the left of Fig.~\ref{fig:main}, \texttt{MoRE} aims at exploiting users' historical interaction to generate reflections from the perspectives of explicit preference, implicit preference, and collaborative signals. We achieve this goal through the following reflectors:

\textbf{Explicit Preference Reflector} 
% infer user $u$'s explicit preferences by driving a LLM to reflect the titles of interacted items $\mathcal{S}_u$. LLM generate reflections $R_\mathrm{EP}$, based on the titles of items the user has interacted with and the titles of the current candidate items as follows:
infers user $u$'s explicit preferences (e.g., item titles) by driving a LLM to reflect the interacted items $\mathcal{S}_u$, the candidate items $\mathcal{C}_u$, and the difference between LLM's prediction $\hat{\mathcal{O}}_u$ and ground-truth $\mathcal{O}_u$. 
LLM generate these reflections simultaneously and return the overall reflection $Ref_\mathrm{EP}$, which can be formulated as:
\begin{equation}
    \label{eq:EP}
    % X_\mathrm{base} = \{u, \mathcal{S}_u^{l-1}, \mathcal{C}_u, P_\mathrm{base}, \mathcal{K}_\mathrm{base}(u, \mathcal{S}_u^{l-1}), gt_u^l\} \\
    % X_\mathrm{EP} = \{\mathrm{EP}(\mathcal{S}_u^{l-1}, \mathcal{C}_u, \mathcal{I}_\mathrm{EP})\}\\
    Ref_\mathrm{EP} = \mathrm{LLM}_{\mathrm{REF}}(P_\mathrm{EP}(u,\mathcal{S}_u,\mathcal{C}_u, \hat{\mathcal{O}}_u, \mathcal{O}_u)),
\end{equation}
where $\mathrm{LLM}_{\mathrm{REF}}$ is a frozen LLM specific for reflection generation, and $P_{\mathrm{EP}}$ denotes the prompt for reflecting from the perspective of explicit user preferences, which represents items using their titles.
% All inputs are sampled from $u$'s interaction history. 
The details are shown in App.~\ref{app:details:EP}.

% infers the users' specific item purchase intents by driving a LLM to analyze the titles of items purchased by the user and generates reflections  $\mathrm{Refl}_{EP}$ based on the titles of items the user has interacted with and the titles of the current candidate items. 
% \xy{
% % Intuitively, in SeqRec tasks, generating satisfactory, accurate, and personalized recommendations for different users requires accurately capturing individual user's preference characteristics and effectively leveraging knowledge about items. However, many current SeqRec algorithms that incorporate LLMs struggle to align the LLM's general text understanding capabilities with the specific interaction intentions of users (explicit and implicit recommendation preferences). Moreover, during the LLM recommendation process, it is challenging to effectively embed both user and item features simultaneously in prompts, making it difficult for the LLM to understand corresponding collaborative filtering information.

% In this section, for the items in a user's past interaction sequences and the candidate items for the next recommendation, we introduce three different reflection generation designs: explicit preference (EP) reflection, implicit preference (IP) reflection, and collaborative filtering (CF) reflection. Each of these is handled by a dedicated reflection expert \textbf{in one group} to synthesize and control the generation of effective, personalized multi-perspective reflections based on user-specific characteristics, aiming to better leverage the reflective insights in subsequent recommendations.}

% \subsubsection{Explicit Preference(EP) Reflection}
% \xy{User's purchase behavior is often directly prompted by the titles of items, which can capture the specific items that users show preference on. Therefore, explicit preference (EP) reflection involves analyzing the titles of items. Specifically, the EP reflection expert infers the user's specific item purchase tendencies by analyzing the titles of items purchased by the user and generates reflective content $\mathrm{Refl}_{EP}$ based on the titles of items the user has interacted with and the titles of the current candidate items. The mechanism of EP reflection is shown below:}
% \begin{equation}
%     \label{eq:EP}
%     \begin{aligned}
%     &X_\mathrm{base} = \{u, \mathcal{S}_u^{l-1}, \mathcal{C}_u, P_\mathrm{base}, \mathcal{K}_\mathrm{base}(u, \mathcal{S}_u^{l-1}), gt_u^l\} \\
%     &X_\mathrm{EP} = \{\mathrm{EP}(\mathcal{S}_u^{l-1}, \mathcal{C}_u, \mathcal{I}_\mathrm{EP})\}\\
%     &P_\mathrm{Refl_{EP}}=\mathrm{Refl}_\mathrm{EP}(u, \mathcal{S}_u^{l-1}) = \mathrm{LLMgen}(P_\mathrm{EP}, \{X_\mathrm{base}, X_\mathrm{EP}\})
%     \end{aligned}
% \end{equation}
% where %$gt_u^l$ is the ground truth item, $\mathcal{I}_\mathrm{EP}$ is item set's title set, and $\mathrm{EP}(\cdot)$ is EP reflection's information pre-processing function.
% $X_\mathrm{base}$ is additional information set of last base recommendation, containing user $u$, sequential session before last recommendation $\mathcal{S}_u^{l-1}$, candidate set $\mathcal{C}_u$ including $|\mathcal{C}_u|$ items, prompt of last base recommendation $P_\mathrm{base}$, last base recommendation's ranked item list $\mathcal{K}_\mathrm{base}$ and last recommendation's ground truth item $gt_u^l$. $X_\mathrm{EP}$ is additional information set of EP reflection, containing $\mathcal{S}_u^{l-1}$, $\mathcal{C}_u$, item set's title set $\mathcal{I}_\mathrm{EP}$. $\mathrm{EP}(\cdot)$ is EP reflection's information pre-processing function which is used to provide item titles. $P_\mathrm{EP}$ is the EP reflection's generation prompt. A specific EP reflection prompt example is provided in Section XXX.

\textbf{Implicit Preference Reflector} is designed to capture the preference embedded in the other item attributes (e.g., item brands) from the interaction sequences $\mathcal{S}_u$, the candidate set $\mathcal{C}_u$ and the LLM prediction $\hat{\mathcal{O}}_u$ and label list $\mathcal{O}_u$. This reflector functions similarly to the explicit preference reflector and adopts a frozen LLM to generate reflections:
\begin{equation}
    \label{eq:IP}
    Ref_\mathrm{IP} = \mathrm{LLM}_{\mathrm{REF}}(P_\mathrm{IP}(u,\mathcal{S}_u,\mathcal{C}_u, \hat{\mathcal{O}}_u, \mathcal{O}_u)),
\end{equation}
where $P_{\mathrm{IP}}$ denotes the reflection prompt from the perspective of implicit user preferences, representing items using their brand names, as detailed in App.~\ref{app:details:IP}.

\textbf{Collaborative Filtering Reflector} targets guiding LLM to reflect from the perspectives of collaborative filtering information.
% that identifies patterns and similarities in user behaviors. 
To incorporate the CF signals, instead of introducing new token embeddings into the vocabulary~\cite{zheng2024adapting} or inserting special sequences into prompts~\cite{zhang2024text}, we adopt a pre-trained CF model to rate the CF scores $\mathcal{M}_u^\mathcal{S}$ and $\mathcal{M}_u^\mathcal{C}$ respectively for the interacted items for $\mathcal{S}_u$ and the candidate items $\mathcal{C}_u$. These scores are then involved in the input of the reflector, which is formulated as:
\begin{equation}
    \label{eq:CF}
    Ref_\mathrm{CF} = \mathrm{LLM}_{\mathrm{REF}}(P_\mathrm{CF}(u,\mathcal{S}_u,\mathcal{C}_u, \mathcal{M}_u^\mathcal{S}, \mathcal{M}_u^\mathcal{C}, \hat{\mathcal{O}}_u, \mathcal{O}_u)),
\end{equation}
where $P_{\mathrm{CF}}$ denotes the reflection prompt from the perspective of CF, as detailed in App.~\ref{app:details:CF}.

We maintain three memory banks for each user to store the generated reflections from the corresponding three perspectives. These memory banks are guided by the meta-reflector to improve the reflections, as will be elaborated in the following section.
% \subsubsection{Implicit Preference(IP) Reflection}

% \xy{The starting point for implicit preference (IP) reflection  is to delve deeper into the sequence of items purchased by the user to capture their implicit preferences. Specifically, this involves analyzing side information about the items, such as brand, product category, and so forth, to indirectly infer the user's preference characteristics. For example, if a user is particularly enthusiastic about purchasing musical instruments and corresponding accessories from a specific brand, many of their purchases are likely driven by loyalty to that brand. This kind of information typically resides within the side features of the items. If these details can be effectively captured and reflected upon, the recommendation effectiveness for brand-loyal users will be improved. Specifically, the IP reflection expert infers the user's indirect item purchase tendencies by analyzing the side information (such as brand, sales volume, and color) of items purchased by the user and the candidate items, other than their titles, generating reflective content based on this analysis. The mechanism of EP reflection %with user $u$ ,candidate set $\mathcal{C}_u$ containing $|\mathcal{C}_u|$ items and sequential session $\mathcal{S}_u^{l-1}$ 
% is shown below:}
% \begin{equation}
%     \label{eq:IP}
%     \begin{aligned}
%     %&X_\mathrm{base} = \{u, \mathcal{S}_u^{l-1}, \mathcal{C}_u, P_\mathrm{base}, \mathcal{K}_\mathrm{base}(u, \mathcal{S}_u^{l-1}), gt_u^l\} \\
%     &X_\mathrm{IP} = \{\mathrm{IP}(\mathcal{S}_u^{l-1}, \mathcal{C}_u, \mathcal{I}_\mathrm{IP})\}\\
%     &P_\mathrm{Refl_{IP}}=\mathrm{Refl}_\mathrm{IP}(u, \mathcal{S}_u^{l-1}) = \mathrm{LLMgen}(P_\mathrm{IP}, \{X_\mathrm{base}, X_\mathrm{IP}\})
%     \end{aligned}
% \end{equation}
% %where $gt_u^l$ is the ground truth item. 
% where $X_\mathrm{base}$ is same as that in Eq.\eqref{eq:EP}. $X_\mathrm{IP}$ is additional information set of IP reflection, containing $\mathcal{S}_u^{l-1}$, $\mathcal{C}_u$, item set's side information set $\mathcal{I}_\mathrm{IP}$. $\mathrm{IP}(\cdot)$ is IP reflection's information pre-processing function which is used to provide item's side information. $P_\mathrm{IP}$ is the IP reflection's generation prompt. A specific IP reflection prompt example is provided in Section XXX.

% \subsubsection{Collaborative Filtering Reflector} 

% \xy{Similar items and similar users can help LLM make better recommendations. 
% % However, unlike methods like BinLLM\nc, which directly concatenate item and user embeddings into a sequence and add them to the reflection prompt, 
% To accommodate these collaborative filtering (CF) signals, current LLM approaches either introduce new token embeddings into the vocabulary or insert special sequences into prompts~\cite{zhang2024text}. 
% % These methods inevitably require fine-tuning and create a significant gap with natural language ability of LLMs. 
% However, besides inevitably requiring costly fine-tuning, the introduced embeddings~\nc{} or sequences create an inherent discrepancy with the natural language form that LLMs excel in, making comprehension challenging.
% We use an LLM-friendly CF information embedding approach. Specifically, our CF information reflection provides a set of possible [user, item] CF scores for previous interactions and items in the candidate set through a tiny CF model. %These scores are then used to teach the CF information reflection expert to better understand the source and validity of the CF information. 
% This information is incorporated into the reflection prompt as CF content, enabling the LLM to have better overall control over the recommendation results. The mechanism of CF reflection with user $u$ ,candidate set $\mathcal{C}_u$ containing $|\mathcal{C}_u|$ items and sequential session $\mathcal{S}_u^{l-1}$ is shown below:}

% \begin{equation}
%     \label{eq:CF}
%     \begin{aligned}
%     %&X_\mathrm{base} = \{u, \mathcal{S}_u^{l-1}, \mathcal{C}_u, P_\mathrm{base}, \mathcal{K}_\mathrm{base}(u, \mathcal{S}_u^{l-1}), gt_u^l\} \\
%     &X_\mathrm{CF} = \{\mathrm{CF}(u, \mathcal{S}_u^{l-1}, \mathcal{C}_u, M_\mathrm{CF})\}\\
%     &P_\mathrm{Refl_{CF}}=\mathrm{Refl}_\mathrm{CF}(u, \mathcal{S}_u^{l-1}) = \mathrm{LLMgen}(P_\mathrm{CF}, \{X_\mathrm{base}, X_\mathrm{CF}\})
%     \end{aligned}
% \end{equation}
% where $X_\mathrm{base}$ is same as that in Eq.\eqref{eq:EP}. $X_\mathrm{CF}$ is additional information set of CF reflection, containing $\mathcal{S}_u^{l-1}$, $\mathcal{C}_u$, a CF sub-model $M_\mathrm{CF}$. $\mathrm{CF}(\cdot)$ is CF reflection's information pre-processing function which is used to provide user-item collaborative filtering information based on $M_\mathrm{CF}$. $P_\mathrm{CF}$ is the CF reflection's generation prompt. A specific CF reflection prompt example is provided in Section XXX.

\subsection{Reflection Memory Maintenance}
\label{sec:meta:main}
Considering that LLMs may not always accurately generate reflection results, we need a mechanism to ensure the validity of reflections after the meta-reflector obtains them from the three reflectors. Therefore, we define a measure called the reflection improvement effect to assess the reflections and devise a refining-and-iteration strategy to update the reflections generated by the LLM.

% \qwc{After gathering reflections from multiple perspectives, we still face two challenges: whether the insight from each perspective is accurate, and which of the three perspectives best suits the user. On one hand, without proper guidance, experts may deviate from their designated perspectives, leading to reflections that miss the mark. Hence, we need an efficient, low-cost method to control experts appropriately, optimizing the reflective knowledge they produce. On the other hand, insights acquired from different reflective perspectives frequently diverge, with their utility varying significantly from one user to another. As users' preferences evolve, so too does the ideal perspective for reflection. Hence, there's a requirement for a        selector mechanism that can adaptively match users with the most fitting perspective dynamically .}

\textbf{Reflection Improvement Effect} is defined as the difference in LLM recommendation performance on the validation set, with or without the reflections. In other words, if incorporating reflections improves the LLM's performance, it indicates that the reflection is effective for recommendation. The greater the performance improvement, the more effective the reflection. If the reflection improvement effect of a reflection exceeds a preset threshold, we regard it as an effective one.
% we call it a ``gold reflection" and add it to the corresponding memory bank.
 Formally, we formulate the reflection improvement effect as:
% \begin{equation}
%     \label{eq:refl}
%     \begin{aligned}
%         \mathcal{K}_{\mathrm{Refl}_s} (u, \mathcal{S}_u^{l-1})&=\mathrm{LLMgen}(P_{\mathrm{Refl}_s}, \{\mathcal{C}_u, u, \mathcal{S}_u^{l-1}\})\\
%         s &\in \mathrm{\{IP, EP, CF\}}
%     \end{aligned}
% \end{equation}
\begin{equation}
\begin{aligned}
     \label{eq:refl:imp}
        Imp &= \mathrm{Metric}(\hat{\mathcal{O}}_{u}^\mathrm{REF}) - \mathrm{Metric}(\hat{\mathcal{O}}_{u}^\mathrm{REC})\\
        % \text{where} \quad
        \hat{\mathcal{O}}_{u}^\mathrm{REF} &=\mathrm{LLM}_{\mathrm{REC}}(Ref_i(u, \mathcal{S}_u, \mathcal{C}_u)), \\
        \hat{\mathcal{O}}_{u}^\mathrm{REC} &=\mathrm{LLM}_{\mathrm{REC}}(P(u, \mathcal{S}_u, \mathcal{C}_u)),
\end{aligned}
\end{equation}
where $Ref_i\in\{Ref_{\mathrm{EP}},Ref_{\mathrm{IP}},Ref_{\mathrm{CF}}\}$, $\mathrm{Metric}$ denotes the recommendation metric, e.g., NDCG@10.  

\textbf{Refining.} 
As we filter out reflections that offer less or negative SeqRec improvement using the above measure, we further refine the selected reflections with three strategies:

(1) \textit{Global Level:} We select the reflections that bring the greatest average improvement for all users. In this approach, all users share the same reflections.

(2) \textit{Group Level}: We use a collaborative filtering (CF) model to construct embeddings for all users and then cluster them using the K-means++ algorithm~\cite{bahmani2012scalable}. We then choose the reflections that provide the greatest average improvement for users within the same cluster, ensuring that users in the same cluster share the same reflections.

(3) \textit{Individual Level:} We select the reflections that bring the greatest improvement for each user. This strategy leads to personalized reflections.

All three of the aforementioned strategies are greedy, which may lead to local optima. To mitigate this issue, we propose using the improvement effect brought about by each reflection as the sampling probability. Reflections sampled from the filtered set serve as demonstrations and are exploited in the subsequent iteration step.

% Reflections are then sampled from the filtered set and added to the meta-reflector's memory bank.

\textbf{Iteration.} 
Since both reflection generation and refining are based on users' historical interactions, a major advantage of \texttt{MoRE} is that these two processes can be completed offline. 
As such, we can further use the sampled reflections as demonstrations and task the three reflectors with generating improved reflections in an in-context learning fashion~\cite{dong2022survey}. In this reflection generation and iteration loop, we enable the LLM to self-improve the reflections. We will further validate the impact of reflection iteration on LLM recommendation performance in the experiments.
% Consequently, we can iterate the reflection generation and refining multiple times to achieve self-improving.

% When we obtain reflections that bring greater improvements in recommendation performance, we can update the current reflection memory bank. 



%After obtaining various types of reflections across different perspectives, a critical question arises: how can we effectively plan and utilize these diverse reflections for different users to further enhance personalized recommendation results? In practical scenarios, continuously online-querying users to improve recommendation outcomes is highly costly. Moreover, since the value of different reflection perspectives varies among users, selecting suitable reflection perspectives becomes essential. For instance, brand-loyal users may particularly prefer other items from the same brand, which means that implicit preference reflection may be the best type. Using a fixed perspective of reflections or always choosing the reflection that seems most valuable to the current user at any given moment might not always be the best strategy.
% To address these challenges, we first propose using the "refining+iteration" approach (Sec.~\ref{sec:meta:main}) %(as described in Section XXX) 
% to offline optimize the use of high-quality reflection examples and iteratively generate effective reflections for different users. Then, we store these reflections and their related information (e.g. user logs and interacted histories) into a container, i.e.  Meta-Reflector's Memory.} %Then, we employ DRL method to explore and exploit the value of different reflections for different users. Specifically, We train a lightweight context-aware PPO selector (in Sec.~\ref{sec:meta:ppo}) to efficiently guide the selection of reflection perspectives, avoiding local optima and incorrect reasoning by the LLM.}



% \subsection{}
% \subsubsection{Refining Iteration Definition}
% \xy{Considering the high cost of obtaining user feedback online and improving the effectiveness of reflections (for example, users might exit the recommendation session due to poor recommendations)
% , we suggest an offline optimization method for enhancing the generation of reflections, which we call "refining+iteration".

% \subsubsection{Reflection Improvement Effect}

% First, we define the reflection improvement effect ($refl\_imp$) as the difference between the recommendation evaluation metric (such as NDCG@10) $\mathrm{Metric}(\mathcal{K}_{\mathrm{Refl}_s})$ after adding $s$ reflection and the base recommendation evaluation metric without reflections $\mathrm{Metric}(\mathcal{K}_\mathrm{base})$ on a validation set. Clearly, the greater the $refl\_imp$, the better the performance of the re-recommendation with the added reflection on the validation set, indicating a higher quality of the reflection. We first define the ($\mathcal{K}_\mathrm{base}$, $\mathcal{K}_{\mathrm{Refl}_s}$, $refl\_imp$) as follows:}
% \begin{equation}
%     \label{eq:base}
%     \begin{aligned}
%         \mathcal{K}_\mathrm{base} (u, \mathcal{S}_u^{l-1})=\mathrm{LLMgen}(P_\mathrm{base}, \{\mathcal{C}_u, u, \mathcal{S}_u^{l-1}\})
%     \end{aligned}
% \end{equation}
% \begin{equation}
%     \label{eq:refl}
%     \begin{aligned}
%         \mathcal{K}_{\mathrm{Refl}_s} (u, \mathcal{S}_u^{l-1})&=\mathrm{LLMgen}(P_{\mathrm{Refl}_s}, \{\mathcal{C}_u, u, \mathcal{S}_u^{l-1}\})\\
%         s &\in \mathrm{\{IP, EP, CF\}}
%     \end{aligned}
% \end{equation}
% \begin{equation}
%     \label{eq:refl:imp}
%     \begin{gathered}
%         refl\_imp(u, \mathcal{S}_u^{l-1}, s) = \mathrm{Metric}(\mathcal{K}_{\mathrm{Refl}_s}) - \mathrm{Metric}(\mathcal{K}_\mathrm{base})\\
%         s \in {\{\mathrm{IP}, \mathrm{EP}, \mathrm{CF}\}}, \quad ref\_imp > thresh\\
%         \mathrm{Metric} = \mathrm{NDCG@10}
%     \end{gathered}
% \end{equation}
% where $\mathcal{K}_\mathrm{base}$ is last base recommendation's ranked item list, $\mathcal{K}_{\mathrm{Refl}_s}$ is the re-recommendation's ranked item list with perspective $s$ reflection, $\mathrm{Metric}(\cdot)$ is the metric evaluation function used to evaluate the recommend performance (e.g. the top-$k$ Normalize Discounted Cumulative Gain (NDCG@$k$)). If a reflection's $refl\_imp$ reaches a threshold $thresh > 0$, we call this reflection a \textit{"gold reflection"}.

% \xy{
% \subsubsection{Refining}
% Then, we set up three strategies for selecting reflection examples to optimize the effectiveness and personalization of reflection generation, which we refer to as ``refining." Specifically:

% \textbf{NEED TERM ALIGNMENT WITH FIGURE 1.}
% 1. The first strategy of example uses the reflection text content that has shown the greatest improvement effect within the current reflection perspective for all users, along with the sequence of previously recommended items and users.
% 2. The second strategy utilizes a collaborative filtering (CF) sub-model to construct embeddings for all users and then reasonably cluster users based on certain clustering rules. Reflection examples with the highest improvement effect within each user cluster are selected for different users.
% 3. The third strategy goes further by considering the individual characteristics of the current user and prioritizes selecting reflection examples that have demonstrated good improvement effects specifically for this user.

% Meanwhile, to avoid getting stuck in local optima during the refining iterations, we recommend probabilistic sampling based on the improvement effect of the reflections. This ensures the selection of high-effectiveness reflection (i.e. \textit{gold reflection}) examples in a reasonable manner. The sampling probability follows the formula:
% \begin{equation}
%     p_i^s=\frac{refl\_imp(u_i,\mathcal{S}_{u_i}^{l_i-1},s)}{\sum_t refl\_imp(u_t,\mathcal{S}_{u_t}^{l_t-1},s)}, \quad \sum_tp_t^s=1
% \end{equation}
% %其中，s类反思中，总计存在t个好反思，pis是s类反思中第i个好反思被选中的概率。
% where $s$ is current type of the reflection, and there are $t$ \textit{gold reflections}. $p_i^s$ is the probability of $i$-th \textit{gold reflection} being chosen. Note that amount of the \textit{gold reflection} may vary if we choose different refining strategies.


% \subsubsection{Iteration} After properly refining the reflection examples, we regenerate reflections for each user who has interacted with the system and continually evaluate the effectiveness of these reflections, which we call ``iteration." However, it's important to note that this entire process is conducted offline. After each iteration, if the use of new reflections generated through the iteration leads to a significant improvement in reflection effects when re-recommended, we store these new reflections along with their corresponding improvement effects for each user.%, which we refer to as \textit{exploitation}. 
% Alternatively, we may store the latest reflections at a certain probability without requiring a large improvement in reflection effects, avoiding overfitting of the reflection content. All these reflections and re-recommendation information are stored into the Meta-Reflector's Memory.%, which we call \textit{exploration}. This approach balances \textit{exploration} and \textit{exploitation}, avoiding overfitting of the reflection content.
% }
% \subsubsection{PPO Selector}
% \xy{
% After using refining iteration methods to collect various types of reflections for different users, it is necessary to select appropriate perspectives of reflection for each user to achieve the best recommendation effect after adding reflections. Considering that not every type of reflection improves the recommendation quality during the user interaction process—some may even degrade the final recommendation quality—and given that not all users have stored reflections and improvement effects across all three perspectives (resulting in many missing samples), simple supervised learning methods cannot be used to select reflection perspectives. Here, we propose using the Proximal Policy Optimization (PPO) ~\nc{} algorithm from DRL methods to efficiently and effectively select reflection perspectives for different users. In the following sections, we will introduce the environment and specific method design corresponding to the entire PPO algorithm.

% \textit{Multi-arm Contextual Bandit (MACB).} To outline the basics of our DRL environment, we define MACB as the tuple $MACB = (\mathcal{Z}, \mathcal{A}, R)$, where $\mathcal{Z}$, $\mathcal{A}$, and $R$ denote the state space, action (arm) space, and reward function, respectively. 
% \begin{itemize}
%     \item \textbf{State.} To model the session-based context information for our selector, we concatenate user, item list's average embedding into a single text string and convert it into a longer embedding for semantic extraction. We use a sub-model (a CF model) as user's and item's embedding generator since it has strong CF information about users and items. The state can be denoted as $\bm{z}= [emb_u,emb_i]$, where $\bm{z} \in \mathcal{Z}$ is $(d_u+d_i)$-dimensional concatenated embedding vector of the sub-model embedding generator.
%     \item \textbf{Action.} To select proper perspective reflection for different user, we define a discrete action space for selector, represented as $\bm{a} \in\mathcal{A}$, which is a $(|s|)$-dimensional vector. Here, $(|s|)$ is the size of total $s$ perspectives, and an action $\bm{a}$ corresponds to choosing a specific perspective. 
%     \item \textbf{Reward.} To direct the selector accurately select the proper perspective, we use the similar definition with $refl\_imp$ in Eq.\eqref{eq:refl:imp}, but for PPO training, we not only need the improvement above threshold, but also taking non-positive improvement into account. Thus, we denote the final reward of state $\bm{z}$ and action $\bm{a}$ as $ R(\bm{z, a}) = refl\_imp,\ refl\_imp \in [-1, 1]$. This technique significantly accelerates the PPO selector's training as the LLM is relatively slow for inference and producing reward, since we reuse $refl\_imp$ metric and do not need to access LLM again for reward signals.
%     %\item \textbf{Transition \& Reset.} To achieve better adaptation of environmental rewards, the selector observes the current user and their interaction sequence as state $\bm{z}$, then takes an action to choose a perspective $\bm{a}$ and receives a reward $r$ from the environment. Following this, the environment transitions to the next user and their sequence state $\bm{z}'$. We denote this transition as $T(\bm{z}, \bm{a}) = (r, \bm{z'})$.
%     %The reset operation is defined as shuffling the users and their sequences (i.e. the state) after all states are traversed for once, and then passing the new shuffled states set to PPO selector to step from the new initial state. This operation is used to make the whole states' transition.%in the shuffled order to perform the operation again.
%     \item \textbf{Replay Buffer.} To facilitate efficiency in policy optimization, we maintain a replay buffer $D = (\bm{z}, \bm{a}, r, \bm{z}')$ to store the tuples of observation state, action, reward, and next observation state. With the records in the replay buffer, the selector  can refine successful policies and learn from erroneous trials. 
% \end{itemize}

% \textit{PPO training.}
% \begin{itemize}
%     \item \textbf{Actor \& Critic Definition.} To model the actions of the selector and evaluate the value of the states, we implement a policy network parameterized by MLPs to define our selector’s Actor $\pi_{\bm{{\theta}}}$ and Critic $V_{\bm\psi}$, which maps the environmental space $\mathcal{Z}$ to the action space $\mathcal{A}$ and reward function $R$ respectively:
%         \begin{equation}
%         \label{eq:ac}
%         \begin{aligned}
%         \mathrm{Actor\ } \pi_{\bm\theta}(\bm{z}): \bm{a} &= softmax(\bm {\theta}\cdot \bm{z}) \\
%         \mathrm{Critic\ } V_{\bm\psi}(\bm{z}): r &= \bm{\psi}\cdot \bm{z}
%         \end{aligned}
%         \end{equation}
%     where $\bm{\theta} \in\mathbb{R}^{(|s|)\times (d_u + d_i)}$ is Actor's learnable weight matrix, and $\bm{z} \in \mathbb{R}^{(d_u + d_i)}$ denotes the state. The selector choose the largest value among the softmax logits of $\bm{a}$. $\bm{\psi} \in \mathbb{R}^{1\times(d_u+d_i)}$ is Critic's weight matrix. 
%     \item \textbf{Clip Objective.} During the training process, the selector's Actor uses the $\epsilon$-greedy ($\epsilon = 0.1$) strategy to explore the environment, with probability $\epsilon$ to take a random action while with probability ($1-\epsilon$) to exploit the learned policy $\pi_{\bm{\theta}}$. We adopts the clip objective function for PPO training to maximize the reward selection as follows:
%     \begin{equation}
%     \label{eq:ppo:train}
%     \begin{aligned}
%         \mathcal{L} = \mathrm{min} \left(\frac{\pi_{\bm{\theta}}}{\pi_{\mathrm{old}}}A(\bm{z,a}), clip(\frac{\pi_{\bm{\theta}}}{\pi_{\mathrm{old}}}, 1-\delta,1 + \delta)A (\bm{z,a}) \right), 
%     \end{aligned}
%     \end{equation}
%     where $A(\bm{z,a}) = \mathbb{E}(R(\bm{z} ,\bm{a})) - V_{\bm\psi}(\bm{z})$ is advantage function used to evaluate $\bm{z}$'s cumulative rewards $\mathbb{E}(R(\bm{z} ,\bm{a}))$ and current value $V_{\bm\psi}(\bm{z})$. $\delta$ is clip threshold ($\delta=0.05$).
% \end{itemize}

% \textit{Final Reflection Select.} With the trained PPO selector, the selection of reflection perspective and its results can be shown as follows:
% \begin{equation}
%     \label{eq:refl:ppo}
%     \begin{aligned}
%         \mathcal{K}_{\mathrm{Refl}_s} (u, \mathcal{S}_u^{l-1})&=\mathrm{LLMgen}(P_{\mathrm{Refl}_s}, \{\mathcal{C}_u, u, \mathcal{S}_u^{l-1}\})\\
%         s &= \pi_{\bm{\theta}}(\bm{z})
%     \end{aligned}
% \end{equation}
% where $\bm{z}$ is the state of current user $u$ and their sequential session $\mathcal{S}_u^{l-1}$.
% }

\subsection{Reflection Selection}
\label{sec:meta:selection}
The second objective of the meta-reflector is to model preference shifts in SeqRec. Since we have designed three memory banks for each user to collect effective reflections from three different perspectives, we require the meta-reflector to select one of these reflections for recommendation to achieve this goal.
We formulate the decision-making process as a Multi-Armed Contextual Bandit (MACB) problem~\cite{Li2010Contextual}, and adopt the Proximal Policy Optimization (PPO) algorithm~\cite{schulman2017proximal} to efficiently learn to select the reflections. Formally,
we define MACB as a tuple $(\mathcal{Z}, \mathcal{A}, \mathcal{R})$, where $\mathcal{Z}, \mathcal{A}, \mathcal{R}$ denote the state space, action (arm) space, and reward function, respectively.
% The corresponding  state, action, and re 
% Our MACB is defined as follows:
\begin{itemize}
    \item \textbf{State} $\bm{z} \in \mathcal{Z}$ is defined as the recommendation context. We represent it by concatenating the embedding of  user $u$ and the interaction sequence $\mathcal{S}_u$, i.e., $\bm{z}= [emb_u,emb_v]$, where the embeddings are derived from a CF model, and $emb_v$ denotes the average embedding for $\mathcal{S}_u$. 
    % To model the session-based context information for our selector, we concatenate user, item list's average embedding into a single text string and convert it into a longer embedding for semantic extraction. We use a sub-model (a CF model) as user's and item's embedding generator since it has strong CF information about users and items. The state can be denoted as $\bm{z}= [emb_u,emb_i]$, where $\bm{z} \in \mathcal{Z}$ is $(d_u+d_i)$-dimensional concatenated embedding vector of the sub-model embedding generator.
    \item \textbf{Action} $\bm{a} \in\mathcal{A}$ is defined as the selection of a reflection from three memory banks. We represent $\bm{a}$ as a 3-dimensional vector, with each dimension corresponding to an arm, each arm representing a reflection memory.
    % To select proper perspective reflection for different user, we define a discrete action space for selector, represented as $\bm{a} \in\mathcal{A}$, which is a $(|s|)$-dimensional vector. Here, $(|s|)$ is the size of total $s$ perspectives, and an action $\bm{a}$ corresponds to choosing a specific perspective. 
    \item \textbf{Reward} is defined to assess the recommendation improvement brought by the reflections. 
    We reuse the measure in Eq.\eqref{eq:refl:imp} and represent the reward as $R(\bm{z, a})=Imp$. 
    Since the reflection has been assessed in Sec.~\ref{sec:multi:perspective} we do not need to call the LLM here. Additionally, due to the sampling discussed in Sec.~\ref{sec:meta:main}, $R(\bm{z, a})$ can be both positive and negative, ensuring training efficiency.
    % reuse the measure in Eq.\eqref{eq:refl:imp}, and adopt
    %  $R(\bm{z, a})=Imp$ to 
    
    % To direct the selector accurately select the proper perspective, we use the similar definition with $refl\_imp$ in Eq.\eqref{eq:refl:imp} of Sec.~\ref{sec:meta:main}, but for PPO training, we not only need the improvement above threshold, but also taking non-positive improvement into account. Thus, we denote the final reward of state $\bm{z}$ and action $\bm{a}$ as $ R(\bm{z, a}) = refl\_imp,\ refl\_imp \in [-1, 1]$. This technique significantly accelerates the PPO selector's training as the LLM is relatively slow for inference and producing reward, since we reuse $refl\_imp$ metric and do not need to access LLM again for reward signals.
    \item \textbf{Replay Buffer} is designed to facilitate efficiency in policy optimization. We represent it as $D = (\bm{z}, \bm{a}, R(\bm{z},\bm{a}), \bm{z}')$ to store the tuples of observed state, action, reward, and next state. With the records in the replay buffer, we can refine successful policies and learn from erroneous trials. 
\end{itemize}
% \textbf{Multi-Arm Contextual Bandit} is 
\label{sec:meta:ppo}
% \subsubsection{PPO Selector}
% \xy{
% After using refining iteration methods to collect various types of reflections for different users in the memory, it is necessary to select appropriate perspectives of reflection for each user to achieve the best recommendation effect after adding reflections. Considering that not every type of reflection improves the recommendation quality during the user interaction process—some may even degrade the final recommendation quality—and given that not all users have stored reflections and improvement effects across all three perspectives (resulting in many missing samples), simple supervised learning methods cannot be used to select reflection perspectives. Here, we propose using the Proximal Policy Optimization (PPO)~\cite{schulman2017proximal} algorithm from DRL methods to efficiently and effectively select reflection perspectives for different users. In the following sections, we will introduce the environment and specific method design corresponding to the entire PPO algorithm.
% \subsubsection{Multi-arm Contextual Bandit (MACB)} To outline the basics of our DRL environment, we define MACB as the tuple $MACB = (\mathcal{Z}, \mathcal{A}, R)$, where $\mathcal{Z}$, $\mathcal{A}$, and $R$ denote the state space, action (arm) space, and reward function, respectively. 
% \begin{itemize}
%     \item \textbf{State.} To model the session-based context information for our selector, we concatenate user, item list's average embedding into a single text string and convert it into a longer embedding for semantic extraction. We use a sub-model (a CF model) as user's and item's embedding generator since it has strong CF information about users and items. The state can be denoted as $\bm{z}= [emb_u,emb_i]$, where $\bm{z} \in \mathcal{Z}$ is $(d_u+d_i)$-dimensional concatenated embedding vector of the sub-model embedding generator.
%     \item \textbf{Action.} To select proper perspective reflection for different user, we define a discrete action space for selector, represented as $\bm{a} \in\mathcal{A}$, which is a $(|s|)$-dimensional vector. Here, $(|s|)$ is the size of total $s$ perspectives, and an action $\bm{a}$ corresponds to choosing a specific perspective. 
%     \item \textbf{Reward.} To direct the selector accurately select the proper perspective, we use the similar definition with $refl\_imp$ in Eq.\eqref{eq:refl:imp} of Sec.~\ref{sec:meta:main}, but for PPO training, we not only need the improvement above threshold, but also taking non-positive improvement into account. Thus, we denote the final reward of state $\bm{z}$ and action $\bm{a}$ as $ R(\bm{z, a}) = refl\_imp,\ refl\_imp \in [-1, 1]$. This technique significantly accelerates the PPO selector's training as the LLM is relatively slow for inference and producing reward, since we reuse $refl\_imp$ metric and do not need to access LLM again for reward signals.
%     %\item \textbf{Transition \& Reset.} To achieve better adaptation of environmental rewards, the selector observes the current user and their interaction sequence as state $\bm{z}$, then takes an action to choose a perspective $\bm{a}$ and receives a reward $r$ from the environment. Following this, the environment transitions to the next user and their sequence state $\bm{z}'$. We denote this transition as $T(\bm{z}, \bm{a}) = (r, \bm{z'})$.
%     %The reset operation is defined as shuffling the users and their sequences (i.e. the state) after all states are traversed for once, and then passing the new shuffled states set to PPO selector to step from the new initial state. This operation is used to make the whole states' transition.%in the shuffled order to perform the operation again.
%     \item \textbf{Replay Buffer.} To facilitate efficiency in policy optimization, we maintain a replay buffer $D = (\bm{z}, \bm{a}, r, \bm{z}')$ to store the tuples of observation state, action, reward, and next observation state. With the records in the replay buffer, the selector  can refine successful policies and learn from erroneous trials. 
% \end{itemize}
\subsubsection{Training}
% \textbf{Training.}
We apply the PPO algorithm~\cite{schulman2017proximal} with an Actor \& Critic networks and a Clip objective function to efficiently learn our MACB.
% \subsubsection{PPO training}
% In order to solve the MACB problem mentioned above, we propose using PPO algorithm as our selector's backbone in the following part, which uses Actor \& Critic networks and Clip objective function.
\begin{itemize}
    \item \textbf{Actor \& Critic Definition.} To model the selection of reflections and evaluate the value of the states, we implement a policy network parameterized by MLPs to define our selector’s Actor $\pi_{\bm{{\theta}}}$ and Critic $V_{\bm\psi}$, which maps the environmental space $\mathcal{Z}$ to the action space $\mathcal{A}$ and reward function $R$ respectively:
        \begin{equation}
        \label{eq:ac}
        \begin{aligned}
        \mathrm{Actor\ } \pi_{\bm\theta}(\bm{z}): \bm{a} &= \mathrm{softmax}(\bm{\theta}\cdot \bm{z}) \\
        \mathrm{Critic\ } V_{\bm\psi}(\bm{z}): r &= \bm{\psi}\cdot \bm{z}
        \end{aligned}
        \end{equation}
    where $\bm{\theta}$ and $\bm{\psi}$ are the learnable weights of Actor and Critic respectively. 
    % where $\bm{\theta} \in\mathbb{R}^{(|s|)\times (d_u + d_i)}$ is Actor's learnable weight matrix, and $\bm{z} \in \mathbb{R}^{(d_u + d_i)}$ denotes the state. The selector choose the largest value among the softmax logits of $\bm{a}$. $\bm{\psi} \in \mathbb{R}^{1\times(d_u+d_i)}$ is Critic's weight matrix. 
    \item \textbf{Clip Objective.} During the training process, the selector's Actor uses the $\epsilon$-greedy ($\epsilon = 0.1$) strategy to explore the environment, with probability $\epsilon$ to take a random action while with probability ($1-\epsilon$) to exploit the learned policy $\pi_{\bm{\theta}}$. We adopt the clip objective function for PPO training to maximize the reward selection as follows:
    \begin{equation}
    \label{eq:ppo:train}
    \begin{aligned}
        \mathcal{L} = \mathrm{min} \left(\frac{\pi_{\bm{\theta}}}{\pi_{\mathrm{old}}}A(\bm{z,a}), clip(\frac{\pi_{\bm{\theta}}}{\pi_{\mathrm{old}}}, 1-\delta,1 + \delta)A (\bm{z,a}) \right), 
    \end{aligned}
    \end{equation}
    where $A(\bm{z,a}) = \mathbb{E}(R(\bm{z} ,\bm{a})) - V_{\bm\psi}(\bm{z})$ is advantage function used to evaluate $\bm{z}$'s cumulative rewards $\mathbb{E}(R(\bm{z} ,\bm{a}))$ and current value $V_{\bm\psi}(\bm{z})$. $\delta$ is clip threshold.% ($\delta=0.05$).
\end{itemize}

\subsubsection{Inference} 
During inference, we select the reflection memories with the highest confidence from the Actor, exploit the reflection  $Ref_i$ with the highest $Imp$ score in the memory, and make a recommendation according to Eq.~\ref{eq:llm4rec} by replacing the prompt $P$ with the reflection $Ref_i$.
% \subsubsection{Reflection Selection} With the trained PPO selector, the selection of reflection perspective and its results can be shown as follows:
% \begin{equation}
%     \label{eq:refl:ppo}
%     \begin{aligned}
%         \mathcal{K}_{\mathrm{Refl}_s} (u, \mathcal{S}_u^{l-1})&=\mathrm{LLMgen}(P_{\mathrm{Refl}_s}, \{\mathcal{C}_u, u, \mathcal{S}_u^{l-1}\})\\
%         s &= \pi_{\bm{\theta}}(\bm{z})
%     \end{aligned}
% \end{equation}
% where $\bm{z}$ is the state of current user $u$ and their sequential session $\mathcal{S}_u^{l-1}$.


\begin{table*}[!htbp]
\setlength{\belowcaptionskip}{5pt}
\centering
\small
\setlength{\tabcolsep}{2.2pt}
\begin{tabular}{@{}lcccccccccccc@{}}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{Methods}} & \multicolumn{4}{c|}{Arts}                                                                                 & \multicolumn{4}{c|}{Games}                                                                                & \multicolumn{4}{c}{Instruments}                                                           \\ \cmidrule(l){2-13} 
\multicolumn{1}{c|}{}                         & HR@5                 & HR@10                & N@5               & \multicolumn{1}{c|}{N@10}         & HR@5                 & HR@10                & N@5               & \multicolumn{1}{c|}{N@10}         & HR@5                 & HR@10                & N@5               & N@10              \\ \midrule
\multicolumn{13}{c}{\textit{Traditional Deep Recommendations Methods}}  \\ \midrule
\multicolumn{1}{l|}{Caser}    & 0.2555                                            & 0.3603                                            & 0.1823                                            & \multicolumn{1}{c|}{0.2161}                                             & 0.3024 & 0.4397 & 0.1997 & \multicolumn{1}{c|}{0.2440}  & 0.2931                                            & 0.3968                                            & 0.2193                                            & 0.2527                                            \\
\multicolumn{1}{l|}{FDSA}     & 0.2536                                            & 0.3670                                             & 0.1875                                            & \multicolumn{1}{c|}{0.2241}                                             & 0.3073 & 0.4466 & 0.2150  & \multicolumn{1}{c|}{0.2597} & 0.2842                                            & 0.3905                                            & 0.2157                                            & 0.2497                                            \\
\multicolumn{1}{l|}{BERT4Rec} & 0.2402                                            & 0.3613                                            & 0.1680                                             & \multicolumn{1}{c|}{0.2072}                                             & 0.2796 & 0.4160  & 0.1861 & \multicolumn{1}{c|}{0.2299} & 0.2618                                            & 0.3789                                            & 0.1954                                            & 0.2326                                            \\
\multicolumn{1}{l|}{GRU4Rec}  & 0.2431                                            & 0.3708                                            & 0.1722                                            & \multicolumn{1}{c|}{0.2129}                                             & 0.3192 & 0.4644 & 0.2083 & \multicolumn{1}{c|}{0.2554} & 0.3021                                            & 0.4021                                            & 0.2201                                            & 0.2520                                             \\

\multicolumn{1}{l|}{SASRec}                   & 0.3570               & 0.4280               & 0.2788               & \multicolumn{1}{c|}{0.3016}          & 0.2915               & 0.4348               & 0.1898               & \multicolumn{1}{c|}{0.2369}          & 0.3450               & 0.3890               & 0.2755               & 0.2896               \\ \midrule
\multicolumn{13}{c}{\textit{Training-Free LLM-based Methods}}    \\ \midrule
\multicolumn{1}{l|}{LLM4RS}                   & 0.1087               & 0.1277               & 0.0826               & \multicolumn{1}{c|}{0.0887}          & 0.1976               & 0.2233               & 0.1338               & \multicolumn{1}{c|}{0.1421}          & 0.0900               & 0.1188               & 0.0624               & 0.0717               \\
\multicolumn{1}{l|}{LLMRank(CoT)}                  & 0.3337			              & 0.4061              & 0.2595         & \multicolumn{1}{c|}{0.2828}    & 0.3508	  & 0.4496      & 0.2607    & \multicolumn{1}{c|}{0.2925}          & 0.2904		        & 0.3709              & 0.2202	                   & 0.2461              \\ \midrule
\multicolumn{13}{c}{\textit{Training-Required LLM-based Methods}}    \\ \midrule
\multicolumn{1}{l|}{LC-Rec}                   & 0.3768               & 0.4309               & 0.3006               & \multicolumn{1}{c|}{0.3181}          & 0.4140               & 0.4646               & \underline{0.3426}         & \multicolumn{1}{c|}{\underline{0.3593}}    & 0.3296               & 0.3920               & 0.2486               & 0.2691               \\
\multicolumn{1}{l|}{BinLLM}                   &         0.2422           &          0.2896           &        0.1786           & \multicolumn{1}{c|}{0.2126}                &            0.2701        &         0.3087           &        0.2119            & \multicolumn{1}{c|}{0.2523}                &   0.2386                 &            0.2799         &      0.1958               &           0.2442          \\
\multicolumn{1}{l|}{Re2LLM}                   & \underline{0.4252}         & \underline{0.4938}         & \underline{0.3535}               & \multicolumn{1}{c|}{\underline{0.3757}}          & \underline{0.4180}         & \underline{0.5198}         & 0.3231               & \multicolumn{1}{c|}{0.3559}          & \underline{0.3521}         & \underline{0.4424}         & \underline{0.2787}         & \underline{0.3074}         \\
\midrule
\multicolumn{1}{l|}{\textbf{\texttt{MoRE}}}            & \textbf{0.4376}      & \textbf{0.5043}      & \textbf{0.3705}      & \multicolumn{1}{c|}{\textbf{0.3922}} & \textbf{0.4773}      & \textbf{0.5731}      & \textbf{0.3647}      & \multicolumn{1}{c|}{\textbf{0.3957}} & \textbf{0.3824}      & \textbf{0.4674}      & \textbf{0.2981}      & \textbf{0.3251}      \\ \midrule
\multicolumn{1}{l|}{\textbf{Imp.}}            & \multicolumn{1}{c}{2.92\%$^\dagger$} & \multicolumn{1}{c}{2.13\%$^\dagger$} & \multicolumn{1}{c}{4.81\%$^\dagger$} & \multicolumn{1}{c|}{4.39\%$^\dagger$}                & \multicolumn{1}{c}{14.19\%$^\dagger$} & \multicolumn{1}{c}{10.25\%$^\dagger$} & \multicolumn{1}{c}{6.45\%$^\dagger$} & \multicolumn{1}{c|}{10.13\%$^\dagger$}                & \multicolumn{1}{c}{8.61\%$^\dagger$} & \multicolumn{1}{c}{5.65\%$^\dagger$} & \multicolumn{1}{c}{6.96\%$^\dagger$} & \multicolumn{1}{c}{5.76\%$^\dagger$} \\ \bottomrule
\end{tabular}
\caption{
% Overall recommendation performance comparison on different datasets. 
% It demonstrates that \texttt{MoRE} achieves state-of-the-art results on all metrics across the three datasets. 
Recommendation performance comparison.
The best and the second-best performances are denoted in \textbf{bold} and \underline{underlined} fonts, respectively. ``N@K'' is short for ``NDCG@K''. The ``Imp.'' indicates the percentage improvement of \texttt{MoRE} over the best performances from baselines. $^\dagger$ denotes \texttt{MoRE} performs significantly better than baselines based on two-tailed paired t-test with Bonferroni correction ($p < 0.05$).}
\label{tab:exp:big}
\end{table*}

\section{Experiment}

In this section, we conduct extensive experiments to answer the following research questions: 
\begin{itemize}
\item \textbf{RQ1:} How does \texttt{MoRE} compare to various existing baselines in terms of recommendation performance?
\item \textbf{RQ2:}
% Are 
% \texttt{MoRE}'s multi-perspective reflections and reflection selection effective?
How effective are the multi-perspective reflections and reflection selection in \texttt{MoRE}?
\item \textbf{RQ3:} For reflection memory maintenance, how effective are the refining and iteration strategies?
% how much contribution does the refining iteration provide? 
% How effective is the personalized cluster method?
\item \textbf{RQ4:} Does \texttt{MoRE} have an advantage in terms of training time overhead and GPU memory usage?
% \item \textbf{RQ5:} How interpretable is our method? 
\end{itemize}

\subsection{Experiment Settings}
\textbf{Dataset.} We conduct our experiments on three product categories from the Amazon dataset~\cite{ni2019justifying}: ``Arts", ``Video", and ``Instruments". Each item in these categories has attributes that reflect both explicit user preferences (e.g., titles) and implicit preferences (e.g., brands). To provide sequential recommendations, we follow the approach in~\cite{zheng2024adapting} and filter out unpopular users and items with fewer than five interactions. The statistics of the pre-processed datasets can be found in App.~\ref{app:dataset}.\\
% \xy{We evaluate our proposed method using three subsets of the Amazon review dataset~\cite{ni2019justifying}:  ``Arts, Crafts and Sewin'', ``Video Games'', and ``Musical Instruments''. 
% In the following text, we will concisely refer to them as ``Arts'', ``Games'', and ``Instruments'', respectively. These datasets contains user reviews from May 1996 to Oct 2018. Each item in the datasets includes a title and a description with side information (e.g. brands, categories). Following previous work~\cite{zheng2024adapting}, we exclude users and items that have fewer than 5 interactions. Subsequently, we construct user behavior sequences based on chronological order. %We evaluated our proposed approach on three subsets of Amazon review data~\cite{ni2019justifying}, including “Musical Instruments”, “Arts, Crafts and Sewing”, and “Video Games”. All three datasets contain user review data from May 1996 to October 2018. Each item in the dataset is associated with a title and a description. Following previous work~\cite{zheng2024adapting}, we filtered out unpopular users and items with less than 5 interactions. Then, we create user behavior sequences based on the chronological order.
% Details of the pre-processed datasets statistics can be found in App.~\ref{app:dataset}}
\textbf{Baselines.}
We adopt three categories of baselines: traditional deep recommendation methods (e.g., SASRec~\cite{kang2018self}, etc.), training-free LLM-based methods (e.g., LLM4RS~\cite{dai2023uncovering}, etc.), and training-required LLM-based methods (e.g., Re2LLM~\cite{wang2024re2llm}, etc.). See App.~\ref{app:details:Baselines} for details. 
\\
% We adopt the following representative SeqRec models as baselines for comparison with our \texttt{MoRE}:
% \textbf{Caser}~\cite{tang2018personalized} is a CNN-based method that models user-item interactions as sequences to capture both local and global patterns.
% \textbf{GRU4Rec}~\cite{hidasi2015session} is an RNN-based SeqRec model with GRU modeling the user behavior sequences.
% \textbf{BERT4Rec}~\cite{sun2019bert4rec} adopts a bidirectional Transformer model and incorporates a masked prediction approach to capture the patterns in item sequences. 
% \textbf{SASRec}~\cite{kang2018self} exploits a unidirectional Transformer-based neural network to model the item sequences and predict the next item. 
% \textbf{FDSA}~\cite{zhang2019feature}  models both item-level and feature-level transition patterns through a dual self-attention mechanism. \textbf{LLM4RS}~\cite{dai2023uncovering} investigates the potential of LLMs in enhancing recommendation capabilities by aligning it with traditional information retrieval (IR) ranking techniques, specifically point-wise, pair-wise, and list-wise ranking. 
% \textbf{LLMRank}~\cite{hou2024large} leverages LLMs for zero-shot ranking in recommendation tasks, addressing challenges related to interaction order and bias through specialized prompting techniques.
% \textbf{LC-Rec}\footnote{To ensure a fair comparison, we ensured that each model's recommendation process for each user was based on the same item candidate set of size 50. However, since LC-Rec's training is based on the full item set as the shared candidate set, it is challenging to guarantee that the model does not output items outside the size 50 candidate set for a user solely through the prompt. To address this, we implemented output constraints for the generation process of LC-Rec, ensuring that it outputs only the permitted 50 items for each user}~\cite{zheng2024adapting} is  a fine-tuning LLMREC method that incorporates collaborative filtering information by expanding the vocabulary space with special token embeddings. It is currently the state-of-the-art method for LLMREC in the full-candidate SeqRec setting.
% % is a large language model recommendation method that incorporates collaborative filtering information. LC-Rec expands the vocabulary space of the large language model backbone by introducing learnable item IDs and special token embeddings for training. LC-Rec designs various recommendation question-answering tasks involving item IDs, enabling the model to understand the relationship between special tokens and text tokens but incurring significant training costs. It is currently the state-of-the-art method for large model recommendations in the full candidate set setting.
% \textbf{BinLLM}\footnote{BinLLM introduces collaborative filtering knowledge to LLMs from the perspective of input text. However, it can only predict the relationship between one user and one item at a time, necessitating multiple inferences to provide recommendations for a user. To ensure a fair comparison, we modified the format of its prompt and reproduced it to make it output a list.}~\cite{zhang2024text} is a fine-tuning LLMREC method that incorporates collaborative filtering information by injecting user and item embeddings as binary text sequences into the LLM's input, without modifying the model's vocabulary space. It is currently the state-of-the-art method for LLMREC conditioned on the given user-item pair.
% % is a LLMREC method that incorporates collaborative filtering information without modifying the vocabulary space. Researchers of BinLLM believe that altering the model's vocabulary space would compromise the original generation capabilities of LLMs, leading to a loss in performance. They propose a fine-tuning method that injects user and item embeddings as binary text sequences into the LLM's input, attempting to leverage the implicit "logical AND" capability of the LLM to understand and capture the relationship between the given user and the target item.
%  \textbf{Re2LLM}~\cite{wang2024re2llm} is a reflection-based LLMREC method. It first constructs a reflection knowledge base (KB) with domain knowledge, and then retrieves suitable text in the fixed KB to insert into the LLM's input, adapting the LLM to session-based recommendation.
\textbf{Evaluation Metrics.} 
To evaluate the performance of
our \texttt{MoRE} and other baselines, we adopt two widely used metrics, top-$k$ Hit Ratio (HR@$k$) and Normalized Discounted Cumulative Gain (NDCG@$k$), with $k\in\{5, 10\}$. Following~\cite{zheng2024adapting, zhou2022filter}, we employ the leave-one-out strategy for the obtaining of training, validation, and test data. Specifically, for each user behavior sequence, the last item is used as the test data, the penultimate item is used as the validation data, and the remaining interaction records are used for training. Following previous work~\cite{wang2024re2llm}, we set every user's candidate set size $|\mathcal{C}_u|$ to 50, where we sample 49 negative items (i.e. items which users do not interact with) from the whole item set for each positive item (i.e. the target item). We perform a ranking evaluation over the candidate set. \texttt{MoRE} and all baselines are required to give a top-10 ranked list for each user.\\
%\scl{this is an example of text}
\textbf{Implementation Details.}
We use LLaMa-3\footnote{https://huggingface.co/gradientai/Meta-Llama-3-8B-bf16. }~\cite{dubey2024llama} as the LLM backbone for \texttt{MoRE} and LLM-based baselines.   Implementation details can be found in App.~\ref{app:details:imp}.
% \xy{We use LLaMa-3-8B-Instruct~\cite{dubey2024llama} as the LLM backbone for our \texttt{MoRE} and LLM-based baselines.

% Considering the cost and efficiency of LLMs, we perform random sampling from three datasets respectively. The principle for sampling users is to exclude those with excessively long interaction sequences before performing random sampling. For each dataset, we sample 1,000 users. Note that items are kept same as the pre-processed datasets.

% For a fair comparison, we use RecBole~\cite{zhao2021recbole} to implement all traditional SeqRec baselines (e.g. SASRec). All these baselines are optimized with Adam optimizer, and we use the grid search method to find the best hyper parameter for each of them. Grid search space was set as: \textit{embedding size} : \{32, 64, 128\}, \textit{learning rate} : \{$1e^{-2}, 1e^{-3},1e^{-4}$\} and \textit{batch size} : \{1024, 2048, 4096\}. For LLMREC baselines which need training, we follow their origin setting and make proper adaption to our datasets. All experiments are run on a 4$\times$A800-PCIE-80GB GPUs server.

% For our \texttt{MoRE} method, we train a DMF~\cite{xue2017deep} model as the source of CF Reflection Expert's CF score (Sec.~\ref{sec:multi:perspective}). Embedding size of this DMF model is 64 for both users and items. This DMF model is also used to implement the user clustering mentioned in the Refining process in Sec.~\ref{sec:meta:main}. DMF model provides embedding vectors for users in the three datasets, and these embeddings are used to cluster the users in each dataset. We define 20 clusters for each dataset, with the cluster ID being an integer in $[0, 19]$, inclusive. For Iteration process in Sec.~\ref{sec:meta:main}, we set the total iteration to 15, and impacts of Refining and Iteration can be found in Sec.~\ref{sec:exp:ri}.
% }


\subsection{Recommendation Performance}
To answer \textbf{RQ1}, we compare the SeqRec performance of \texttt{MoRE} against baselines for 10 trials, with the average results presented in Tab.~\ref{tab:exp:big}. We can observe the following:
% \begin{enumerate}

    (1) \texttt{MoRE} outperforms all other baselines across each metric on each dataset. On all metrics across three datasets, \texttt{MoRE} outperforms the best baseline by average improvements of 3.56\%, 10.25\%, and 6.75\%, respectively. We attribute this to our proposed LLM-based reflection framework which leverages the reflection capabilities of LLMs to understand both users' explicit and implicit preferences. Additionally, it enables LLMs to grasp the CF knowledge in a straightforward and comprehensible manner, leading to improved performance in SeqRec.
    
    (2) In general, LLM-based methods demonstrate performance comparable to the traditional methods, which validates the potential of LLMs in SeqRec.  Additionally, LLMRank with CoT~\cite{feng2024towards} significantly outperforms LLM4RS, indicating that prompt engineering strategies like CoT~\cite{wei2022chain} can substantially enhance performance without fine-tuning.
    
    (3) Typically, trained methods demonstrate superior performance compared to their untrained counterparts. Surprisingly, BinLLM delivers relatively underwhelming outcomes. Designed to leverage binary sequences in prompts to capture the correlation between a user-item pair, BinLLM struggles with the nature of SeqRec, which involves a user and multiple candidate items. The insertion of such sequences leads to excessively long prompts, hindering LLMs' capacity to accurately identify user-item associations.


In summary, \texttt{MoRE} exhibits superior performance in SeqRec, thereby validating the efficacy of our approach.


\subsection{Analysis of Multi-Perspective Reflection and Selection}
\label{sec:exp:selection}
% Intuitively, the reflection from one single perspective cannot address all issues. 
To validate the effectiveness of each perspective of reflection and answer \textbf{RQ2}, we conduct an analytical experiment on Amazon Arts. The results are presented in Tab.~\ref{tab:exp:ablation}.

We find that \texttt{MoRE}, equipped with the reflection selection, outperforms alternatives, demonstrating the effectiveness of the multi-perspective reflections and the corresponding perspective selection. Specifically, \texttt{MoRE} outperforms the variants with not only the single reflection perspective but also the dual or triple perspectives simultaneously. This underscores that no single perspective of reflection is universally optimal for all users, thereby confirming the necessity for selective choice among perspectives.

Moreover, \texttt{MoRE}'s selection strategy surpasses both the Random and Greedy selection approaches which respectively denote a random reflection selection from the three memory banks and the selection solely based on downstream recommendation performance.
This highlights the effectiveness of our contextual bandit modeling, enabling \texttt{MoRE} to judiciously choose the most suitable reflection for each user.
% , thereby catering to the diverse needs of different user types.
% To further assess the reflection generated by \texttt{MoRE}, we also make a \textbf{case study} in App.~\ref{app:details:case} to check whether \texttt{MoRE} can give the interpretable answers based on specific cases, compared to other alternative selection strategies.

We also conduct a \textbf{case study} in App.~\ref{app:details:case} to further assess the reflection selection of \texttt{MoRE} in comparison to other alternative selection strategies.

\begin{figure*}[!ht]
    %\centering
    \setlength{\belowcaptionskip}{-5pt}
    \begin{subfigure}[h]{0.3\textwidth}
        \centering
    \includegraphics[width=\textwidth]{fig_updated/Amazon_Arts_EP_reflect_refining_impact_v7_no_title.pdf}
    %\vspace{3.2ex}
        \caption{Arts}
        \label{fig:Arts:cluster:comp}
    \end{subfigure}
    \hfill
    \begin{subfigure}[h]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig_updated/Amazon_Games_EP_reflect_refining_impact_v7_no_title.pdf}
        \caption{Games}
        \label{fig:Games:cluster:comp}
    \end{subfigure}
    \hfill
    \begin{subfigure}[h]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig_updated/Amazon_Instruments_EP_reflect_refining_impact_v7_no_title.pdf}
        \caption{Instruments}
        \label{fig:Instruments:cluster:comp}
    \end{subfigure}
    % \centering
    % \includegraphics[width=0.45\textwidth]{LaTeX/fig/Amazon_Arts_cluster_explicit_reflect_iteration_trend_v1.pdf}
    \caption{
    Impact of refining and iteration strategies on recommendation performance. 
    We repeated the experiment 5 times, with the mean value for each method represented by the line and the shaded area indicating the standard deviation.
     % Impact of using different refining strategies %personalized cluster method for Refining the selected examples in Iteration period 
     % for giving EP reflector demonstrations in 3 datasets. ``Global'' means demonstrations are sampled from the best improved reflections among the whole dataset. ``Group'' means demonstrations are sampled from the best improved reflections from current user's own cluster. ``Individual'' means demonstrations are firstly selected from user's self good improved reflections, and then sampled from user's own cluster's other reflections. All of the methods are run for 5 times on 3 datasets. Mean value and standard deviation of each method is shown as the line and the shadow area.
     }
    % %\label{fig:diff:IL:IBCB}
    \label{fig:cluster:comp}

\end{figure*}

\begin{table*}[htbp]
\setlength{\belowcaptionskip}{5pt}
\centering
\small
\begin{tabular}{l|cc|cc|cc}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{Methods}} & \multicolumn{2}{c|}{Arts}              & \multicolumn{2}{c|}{Games}            & \multicolumn{2}{c}{Instruments}       \\ \cmidrule(l){2-7} 
\multicolumn{1}{c|}{}                         & Time/h                & GRAM/GB        & Time/h                & GRAM/GB       & Time/h                & GRAM/GB       \\ \midrule
LC-Rec (Fine-Tune)                            & 20.382(±0.670)          & 206.37          & 21.361(±0.678)          & 201.35        & 13.720(±0.436)          & 199.93        \\
BinLLM (Fine-Tune)                                 &         10.209(±0.090)              & 124.67          &                 11.468(±0.072)      & 120.57         &   10.435(±0.094)                    & 115.48         \\
Re2LLM (RL)                                   & 4.007(±0.007)          & 2.77          & 3.894(±0.005)          & 1.99          & 4.152(±0.008)          & 1.13          \\ \midrule
\textbf{\texttt{MoRE} (RL)}                            & \textbf{3.982(±0.001)} & \textbf{2.77} & \textbf{3.854(±0.002)} & \textbf{1.99} & \textbf{4.093(±0.003)} & \textbf{1.13} \\ \bottomrule
\end{tabular}
\caption{
% Comparison of training cost for LLM methods that involve training. 
% ``Time/h'' denotes the training time, presented as the mean and standard deviation (SD). ``GRAM/GB'' denotes the maximum memory consumption. We perform five repetitions on 4 A800 GPUs.
Training cost comparisons among LLM-based methods on four A800 GPUs. "Time/h" represents the training time, shown as the mean and standard deviation (SD). "GRAM/GB" indicates the maximum memory consumption.
}
\label{tab:exp:cost}
\end{table*}

\begin{table}[!t]
\setlength{\belowcaptionskip}{5pt}
\centering
\small
\begin{tabular}{l|cc}
\toprule
Methods                  & N@5             & N@10            \\ \midrule
\textbf{\texttt{MoRE}}                     & \textbf{0.3705} & \textbf{0.3922} \\ \midrule
- Random                & 0.3421          & 0.3701          \\
- Greedy                 & 0.3528          & 0.3786          \\ \midrule
- $Ref_\mathrm{EP}$ only          & 0.3670          & 0.3881          \\
- $Ref_\mathrm{IP}$ only          & 0.3571          & 0.3788          \\
- $Ref_\mathrm{CF}$ only          & 0.3572          & 0.3788          \\
- $Ref_\mathrm{EP}+Ref_\mathrm{IP}$        & 0.3443          & 0.3651          \\
- $Ref_\mathrm{EP}+Ref_\mathrm{CF}$        & 0.3311          & 0.3533          \\
- $Ref_\mathrm{IP}+Ref_\mathrm{CF}$        & 0.3033          & 0.3217          \\
- $Ref_\mathrm{EP}+Ref_\mathrm{IP}+Ref_\mathrm{CF}$ & 0.3051          & 0.3268          \\ \bottomrule
\end{tabular}
\caption{Ablation studies on Amazon Arts. ``Random'' indicates a random reflection selection from the three memory banks, while ``Greedy'' denotes that reflection selection is based solely on downstream SeqRec on the validation set.
% It illustrates \texttt{MoRE} selects the most suitable reflection direction for each user through Reflection Selection, achieving the best performance.
% The best performances are denoted in bold fonts. 
% ``Random'' indicates a random selection of directions, while ``Greedy'' means that the selection of directions depends solely on the performance on the validation set. ``N@K'' is short for ``NDCG@K''. $^\dagger$ denotes \texttt{MoRE} performs significantly better than others based on two-tailed paired t-test with Bonferroni correction ($p < 0.05$). 
}
\label{tab:exp:ablation}
\end{table}
\subsection{Analysis of the Refining and Iteration}
\label{exp:refine}
To answer \textbf{RQ3}, we test the impact of three refining strategies on SeqRec under different iteration rounds, taking reflections on explicit user preferences as an example. 
% (i.e., selecting LLM reflections based on the user's interaction history from the perspective of explicit preferences). 
From the Fig.~\ref{fig:cluster:comp}, we observed that:
% we test the effectiveness of refining and iteration within the reflection memory maintenance over 5 trials. As shown in Fig.~\ref{fig:cluster:comp}, we observe that:

(1) \textbf{Iteration}: 
Overall, as the number of iterations increases, the recommendation performance gradually improves. This indicates that iteration can enhance the quality of reflections, thereby improving the recommendation.
% As the number of iterations increases, the recommendation performance gradually improves across {\color{red}different perspectives}, validating the effectiveness of the iterations.

% (1) For different perspectives, the refining iteration method effectively improve the re-recommendation performance of reflections from those perspectives.

(2) \textbf{Refining}: Refining at group and individual levels shows a significantly better trend over that at the global level during iterations, particularly on Arts (Fig.~\ref{fig:cluster:comp}(a)).  
This improvement may be due to the global-level reflections introducing noise from other users, whereas group- and individual-level demonstrations more effectively elicit personalized reflective capabilities from the reflectors.

% In summary, the refining and iteration strategies collectively facilitate a self-improving mechanism for reflection without the need for fine-tuning.
% In summary, the refining and iteration strategies work together to enable a fine-tuning-free process that allows reflections to self-improve.
Additionally, we found that the refining and iteration strategies are most effective for reflections on explicit preferences, compared to reflections on implicit preferences and collaborative filtering. Detailed experiments and discussions are presented in App.~\ref{app:perspect:details}.




% The refining method using clustering and personalized example sampling shows a significantly better trend over iterations compare to using `Share', which represents the globally optimal example sampling method. Specifically, in the iteration graph for EP reflection on Arts (left figure in Fig.1), the re-recommendation performance with the `Personalized' and `Cluster' methods improves noticeably as the number of iterations increases, with a clear improvement in performance by the later stages of iteration compare to the non-iterated version. In contrast, the method using `Share' experiences a continuous decline in performance due to iteration, possibly because the globally optimal approach can sometimes lead to all generated reflections being skewed by examples from certain specific users. This further supports our conclusion that the use of clustering and personalized refining iteration method can effectively enhance the personalized reflection effects for different users.

\label{sec:exp:ri}
% \begin{figure*}
%     %\centering
%     \setlength{\belowcaptionskip}{-5pt}
%     \begin{subfigure}[h]{0.33\textwidth}
%         \centering
%     \includegraphics[width=\textwidth]{LaTeX/fig_updated/Amazon_Games_EP_reflect_iteration_trend_v1.pdf}
%     %\vspace{3.2ex}
%         \caption{Explicit Preference (EP) Reflect}
%         \label{fig:Games:explicit:iter}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[h]{0.33\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{LaTeX/fig_updated/Amazon_Games_IP_reflect_iteration_trend_v1.pdf}
%         \caption{Implicit Preference (IP) Reflect}
%         \label{fig:Games:implicit:iter}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[h]{0.33\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{LaTeX/fig_updated/Amazon_Games_CF_reflect_iteration_trend_v1.pdf}
%         \caption{Collaborative Filtering (CF) Reflect}
%         \label{fig:Games:CF:iter}
%     \end{subfigure}
%     % \centering
%     % \includegraphics[width=0.45\textwidth]{LaTeX/fig/Amazon_Arts_cluster_explicit_reflect_iteration_trend_v1.pdf}
%     \caption{
%     Different types of reflections' iteration trend comparison.}
%     % %\label{fig:diff:IL:IBCB}
%     \label{fig:type:iter:comp}

% \end{figure*}

% \subsection{Analysis of PPO Selector}




\subsection{Analysis of LLM Training Cost}
% \begin{table*}[tb]
% \centering
% \small
% \begin{tabular}{l|cc|cc|cc}
% \toprule
% \multicolumn{1}{c|}{\multirow{2}{*}{Methods}} & \multicolumn{2}{c|}{Arts}              & \multicolumn{2}{c|}{Games}            & \multicolumn{2}{c}{Instruments}       \\ \cmidrule(l){2-7} 
% \multicolumn{1}{c|}{}                         & Time/h                & GRAM/GB        & Time/h                & GRAM/GB       & Time/h                & GRAM/GB       \\ \midrule
% LC-Rec (Fine-Tune)                            & 20.382(±0.670)          & 206.37          & 21.361(±0.678)          & 201.35        & 13.720(±0.436)          & 199.93        \\
% BinLLM (Fine-Tune)                                 &         10.209(±0.090)              & 124.67          &                 11.468(±0.072)      & 120.57         &   10.435(±0.094)                    & 115.48         \\
% Re2LLM (RL)                                   & 4.007(±0.007)          & 2.77          & 3.894(±0.005)          & 1.99          & 4.152(±0.008)          & 1.13          \\ \midrule
% \textbf{\texttt{MoRE} (RL)}                            & \textbf{3.982(±0.001)} & \textbf{2.77} & \textbf{3.854(±0.002)} & \textbf{1.99} & \textbf{4.093(±0.003)} & \textbf{1.13} \\ \bottomrule
% \end{tabular}
% \caption{
% % Comparison of training cost for LLM methods that involve training. 
% % ``Time/h'' denotes the training time, presented as the mean and standard deviation (SD). ``GRAM/GB'' denotes the maximum memory consumption. We perform five repetitions on 4 A800 GPUs.
% Training cost comparisons among LLM-based methods on four A800 GPUs. "Time/h" represents the training time, shown as the mean and standard deviation (SD). "GRAM/GB" indicates the maximum memory consumption.
% }
% \label{tab:exp:cost}
% \end{table*}

To address \textbf{RQ4}, we conduct 5 repeat experiments to compare the training time and maximum memory consumption associated with all the LLM-based baselines that require training. 
To mitigate the effects of experimental randomness, we perform 5 repetitions of the experiments and report the results as the mean and standard deviation (SD), as shown in Tab.~\ref{tab:exp:cost}. Our findings are as follows: 

 (1) The training cost of reflection-based methods is lower than fine-tuning methods. This is because the reflection-based methods do not require fine-tuning, thus avoiding significant training time and memory costs. 

 (2) Under reflection-based setup, \texttt{MoRE} has lower training time and memory consumption compared to Re2LLM. We attribute this to the larger action space of Re2LLM. Specifically, \texttt{MoRE}'s Meta-Reflector does not require selecting specific reflections but only needs to choose among three directions of reflection. 
 % Furthermore, updates to the reflection text are confined to the corresponding directional reflection library, ensuring consistency and coherence within the type of reflection. Even if a new, better reflection text replaces an old one, it still belongs to the same direction, and Meta-Reflector does not need retraining. 
 In contrast, Re2LLM must first acquire a knowledge base of reflection and, once fixed, conduct PPO training of the retrieval agent within that knowledge base. This means it selects specific reflections from the entire knowledge base, with a larger action space. 
 % Additionally, if its knowledge base changes after PPO training, its retrieval  must be retrained, which would consume more time in practical scenarios. 
 
 In summary, \texttt{MoRE} has the lowest training costs including time overhead and GPU memory usage among all the LLM-based baselines, demonstrating its training efficiency.



% \subsection{Case Study}

\definecolor{myboxcolor}{RGB}{0,100,0} 
\definecolor{myboxcolor2}{RGB}{100,0,0} 
\newtcolorbox{mybox_case}[1]{
  colback=myboxcolor!5!white,
  colframe=myboxcolor!75!black,
  fonttitle=\bfseries,
  title=#1,
  halign title=center, 
  halign=flush left,   
  left=0mm,
  right=0mm
}
\newtcolorbox{mybox_random}[1]{
  colback=myboxcolor2!5!white,
  colframe=myboxcolor2!75!black,
  fonttitle=\bfseries,
  title=#1,
  halign title=center, 
  halign=flush left,   
  left=0mm,
  right=0mm
}

\iffalse
\begin{mybox_case}{Case Study: \emph{\texttt{MoRE}'s Reflection Selector}}
\vspace{0pt}
\small{\textit{\textbf{Prompt}: I've purchased the following products in the past in order: \{Ben 10 Omniverse 2 - Nintendo Wii U;...\}. And after last previous recommendation (maybe a failed trial), you give the following reflects:\{\color{blue}$Ref_i$\color{black}\}. Now there are {\color{blue}{$|\mathcal{C}_u|$}} candidate products that I can consider to purchase next:\{\color{blue}$\mathcal{C}_u$\color{black}\}.Please rank these {\color{blue}{$|\mathcal{C}_u|$}} products by measuring the possibilities that I would like to purchase next most, according to the given purchasing records and reflects. Please think step by step. Please show me your top 10 ranking results with order numbers. Split your output with line break. You MUST rank the given candidates. You can not generate candidates that are not in the given candidate list.% Based on these interactions, recommend a movie for me to watch next from a candidate set: \{\color{blue}$\mathcal{C}$\color{black}\}. Please recommend from the candidate set. List the top 10 recommendations in numbered bullet points. Hint: \{\color{blue}$h$\color{black}\}.
% \newline 
% \textbf{Answer by recommendation w/o reflects}, where \color{blue} $Ref$ \color{black} = `':
% \newline  ``Final Fantasy Legend", ``2. Assassin's Creed Liberation HD [Download]", ``3. Spinido iPhone 7 Plus Desk Stand Holder Compatible with All Smartphone with Cases- Gold", ``4. Phineas and Ferb Ride Again - Nintendo DS", ``5. Shadow Warrior", ``6. Saints Row IV: National Treasure - Xbox 360", ``7. Cabela's African Adventures - Wii", ``8. The Sims 2: Double Deluxe - PC", ``9. Disney INFINITY (2.0 Edition) [Download]", ``10. Metal Gear Solid HD Collection"
\newline 
\textbf{Answer by \texttt{MoRE} perspective selector}, where \color{myboxcolor!75!black}{\textbf{selected reflection (CF reflection)}} \color{blue} $Ref_i = Ref_\mathrm{CF}$ \color{black} = `\textbf{\color{myboxcolor!75!black}{PREFERENCE: The user tends to prefer gaming-related items with high CF scores, particularly those from PlayStation 4 and Xbox 360 platforms, as well as items with high CF scores from previous interactions. ANALYSIS: Although the actor's previous recommendations are diverse, some items such as \{HORI Fighting Commander 4 Controller for PlayStation 4/3, ...\}, was not included in the actor's recommendations. This suggests that the actor may have overlooked strong CF signals in favor of more diverse recommendations. SUGGESTIONS: Prioritize gaming-related items with high CF scores, especially those from PlayStation 4 and Xbox 360 platforms, as well as items with high CF scores from previous interactions. Consider including items with CF scores above 0.5, such as \{...\}, to improve the accuracy of the recommendations.}}':
\newline \textbf{{1. Street Fighter V - PlayStation 4 Standard Edition (CF score: 0.83)}}, 2. Mass Effect 2 - PC (CF score: 0.78), 3. Assassin's Creed Liberation HD [Download] (CF score: 0.76), 4. Metal Gear Solid HD Collection (CF score: 0.75), 5. Call of Duty: Advanced Warfare Atlas Limited Edition - Xbox One (CF score: 0.74), 6. Spec Ops: The Line - Playstation 3 (CF score: 0.73), 7. Cities: Skylines [Online Game Code] (CF score: 0.72), 8. Final Fantasy Crystal Chronicles: Echoes of Time - Nintendo Wii (CF score: 0.71), 9. Fatal Fury: Mark of The Wolves (CF score: 0.7), 10. .hack, Part 3: Outbreak (CF score: 0.69)
% \newline 
% \textbf{Answer by Random perspective selector}, where \color{myboxcolor2!75!black}{\textbf{random hint}} \color{blue} $Ref$ \color{black} = `\textbf{\color{myboxcolor2!75!black}{Pay attention to actors who appear in multiple movies from the watched list and consider other films featuring these actors}}':
% \newline 1. The Day After Tomorrow; 2. Taken; 3. The Bourne Identity; 4. Last Man Standing; 5. The Last Castle; 6. The Wrestler; 7. Redbelt; 8. The Stepfather; 9. Kiss of the Dragon; 10. Courage Under Fire
% \newline 
% \textbf{Answer by \texttt{MoRE}}, where \color{myboxcolor2!75!black}{\textbf{random hint}} \color{blue} $Ref$ \color{black} = `\textbf{\color{myboxcolor2!75!black}{Pay attention to actors who appear in multiple movies from the watched list and consider other films featuring these actors}}':
% \newline 1. The Day After Tomorrow; 2. Taken; 3. The Bourne Identity; 4. Last Man Standing; 5. The Last Castle; 6. The Wrestler; 7. Redbelt; 8. The Stepfather; 9. Kiss of the Dragon; 10. Courage Under Fire
}}
\vspace{0pt}
\end{mybox_case} 
\vspace{0pt}
\begin{mybox_random}{Case Study: \emph{Other Reflection Selectors}}
\vspace{0pt}
\small{\textit{\textbf{Prompt}: (same form as former prompt)%I've purchased the following products in the past in order: \{Ben 10 Omniverse 2 - Nintendo Wii U;...\}. And after last previous recommendation (maybe a failed trial), you give the following reflects:\{\color{blue}$Ref$\color{black}\}. Now there are 50 candidate products that I can consider to purchase next:\{\color{blue}$\mathcal{C}$\color{black}\}.Please rank these 50 products by measuring the possibilities that I would like to purchase next most, according to the given purchasing records and reflects. Please think step by step. Please show me your top 10 ranking results with order numbers. Split your output with line break. You MUST rank the given candidates. You can not generate candidates that are not in the given candidate list.Based on these interactions, recommend a movie for me to watch next from a candidate set: \{\color{blue}$\mathcal{C}$\color{black}\}. Please recommend from the candidate set. List the top 10 recommendations in numbered bullet points. Hint: \{\color{blue}$h$\color{black}\}.
% \newline 
% \textbf{Answer by recommendation w/o reflects}, where \color{blue} $Ref$ \color{black} = `':
% \newline  ``Final Fantasy Legend", ``2. Assassin's Creed Liberation HD [Download]", ``3. Spinido iPhone 7 Plus Desk Stand Holder Compatible with All Smartphone with Cases- Gold", ``4. Phineas and Ferb Ride Again - Nintendo DS", ``5. Shadow Warrior", ``6. Saints Row IV: National Treasure - Xbox 360", ``7. Cabela's African Adventures - Wii", ``8. The Sims 2: Double Deluxe - PC", ``9. Disney INFINITY (2.0 Edition) [Download]", ``10. Metal Gear Solid HD Collection"
\newline 
\textbf{Answer by recommendation w/o reflection}, where \color{myboxcolor2!75!black}{\textbf{selected reflection (EP reflection)}} \color{blue} $Ref_i$ \color{black} = `':
\newline  1. Final Fantasy Legend, 2. Assassin's Creed Liberation HD [Download], 3. Spinido iPhone 7 Plus Desk Stand Holder Compatible with All Smartphone with Cases- Gold, 4. Phineas and Ferb Ride Again - Nintendo DS, 5. Shadow Warrior, 6. Saints Row IV: National Treasure - Xbox 360, 7. Cabela's African Adventures - Wii, 8. The Sims 2: Double Deluxe - PC, 9. Disney INFINITY (2.0 Edition) [Download], 10. Metal Gear Solid HD Collection
\newline 
\textbf{Answer by Greedy perspective selector}, where \color{myboxcolor2!75!black}{\textbf{selected reflection (EP reflection)}} \color{blue} $Ref_i = Ref_\mathrm{EP}$ \color{black} = `\textbf{\color{myboxcolor2!75!black}{ PREFERENCE: The user has shown a strong interest in fighting games, particularly those with a classic or retro feel, as well as console-based games. ANALYSIS: The actor's recommendations did not fully capitalize on the user's preferences for fighting games and console-based games. The recommended games did not show a strong focus on gameplay and mechanics, and did not prioritize the most engaging and popular titles in the fighting game genre. SUGGESTIONS: Prioritize recommending fighting games, particularly those with a classic or retro feel, and consider suggesting console-based games that cater to the user's interest in gameplay and mechanics.}}':
\newline  1. Fatal Fury: Mark of The Wolves, 2. Final Fantasy Crystal Chronicles: Echoes of Time - Nintendo Wii, 3. .hack, Part 3: Outbreak, 4. Capcom Classics Collection, 5. Bad News Baseball - Nintendo NES, 6. Teenage Mutant Ninja Turtles IV: Turtles in Time, \textbf{7. Street Fighter V - PlayStation 4 Standard Edition}, 8. Metal Gear Solid HD Collection, 9. Final Fantasy Legend, 10. Urban Champion
\newline 
\textbf{Answer by Random perspective selector}, where \color{myboxcolor2!75!black}{\textbf{selected reflection (IP reflection)}} \color{blue} $Ref_i = Ref_\mathrm{IP}$ \color{black} = `\textbf{\color{myboxcolor2!75!black}{ PREFERENCE: Based on the user's interaction history, it appears that they have a strong preference for games from Nintendo and PlayStation platforms, particularly games from the Wii and Wii U console platforms. The user also shows interest in games with multiplayer features, as evidenced by the inclusion of games like \{...\}. ANALYSIS: To improve the actor's recommendations, I suggest prioritizing games from Nintendo and PlayStation platforms, particularly games from the Wii and Wii U console platforms. The actor should also focus on games with multiplayer features, as this seems to be an area of interest for the user. Additionally, consider recommending games that offer unique gameplay mechanics, such as \{...\}, which the user has interacted with previously.}}':
\newline  1. Final Fantasy Crystal Chronicles: Echoes of Time - Nintendo Wii, 2. Mike Tyson's Punch-Out!! - Nintendo NES, 3. Bad News Baseball - Nintendo NES, 4. Urban Champion - Nintendo NES, 5. Super Mario 64 DS - Nintendo DS, 6. Moshi Monsters - Nintendo DS, 7. LEGO Pirates of the Caribbean - Nintendo DS, 8. Phineas and Ferb Ride Again - Nintendo DS, 9. Cabela's African Adventures - Wii, 10. Disney Magical World - Nintendo 3DS
% \newline 
% \textbf{Answer by Random perspective selector}, where \color{myboxcolor2!75!black}{\textbf{random hint}} \color{blue} $Ref$ \color{black} = `\textbf{\color{myboxcolor2!75!black}{Pay attention to actors who appear in multiple movies from the watched list and consider other films featuring these actors}}':
% \newline 1. The Day After Tomorrow; 2. Taken; 3. The Bourne Identity; 4. Last Man Standing; 5. The Last Castle; 6. The Wrestler; 7. Redbelt; 8. The Stepfather; 9. Kiss of the Dragon; 10. Courage Under Fire
% \newline 
% \textbf{Answer by \texttt{MoRE}}, where \color{myboxcolor2!75!black}{\textbf{random hint}} \color{blue} $Ref$ \color{black} = `\textbf{\color{myboxcolor2!75!black}{Pay attention to actors who appear in multiple movies from the watched list and consider other films featuring these actors}}':
% \newline 1. The Day After Tomorrow; 2. Taken; 3. The Bourne Identity; 4. Last Man Standing; 5. The Last Castle; 6. The Wrestler; 7. Redbelt; 8. The Stepfather; 9. Kiss of the Dragon; 10. Courage Under Fire
}}
\vspace{0pt}
\end{mybox_random} 
\fi




\section{Conclusion}
In this paper, we propose a mixture of reflectors framework, namely \texttt{MoRE}, for modeling and learning the dynamic user preferences in SeqRec.  
We first introduce three reflectors for each user to generate LLMs’ reflections from the perspectives of explicit user preferences, implicit user preferences, and collaborative signals. 
Building on these reflectors, we introduce a meta-reflector that evaluates and updates the generated reflections using a self-improving strategy. It selects the most appropriate perspective and corresponding reflections for each user's current recommendation using a contextual bandit algorithm.
Extensive experiments conducted on three benchmark datasets demonstrate that \texttt{MoRE} consistently outperforms traditional recommendation methods and LLM-based recommendation methods with minimal GPU memory usage and training time overhead. 



% Traditional imitation learning (IL) focuses on learning the decision-making policy of an experienced and fixed expert by using its historical behaviors. IL utilizes experts' demonstrations for policy fitting and aims to extract knowledge from experts' demonstrations to replicate their behaviors or environments. It can be divided into two main categories: Behavior Cloning (BC)~\citep{Bain1995Framework} and Inverse Reinforcement Learning (IRL)~\citep{Russell1998Learning}. BC approaches aim to learn a policy that directly maps states to actions, while IRL approaches focus on recovering the reward parameters from demonstrations to recover the experts' policy~\citep{Zheng2022Imitation}. 

% A major challenge in imitation learning (IL) is the substantial requirement of expert demonstration data~\citep{Abbeel2004Apprenticeship, Hussein2017Imitation}. There is a common assumption that the experts are always experienced (see Fig.~\ref{fig:IL:mechanism}). However, in real-world streaming scenarios, the behavior policy of the expert constantly evolves over time, transitioning from a novice expert to an experienced one. Throughout this process, we accumulate a significant amount of expert's \emph{behavioral evolution history}.
%  Taking streaming recommender systems as an example~\citep{Zhang2021Counterfactual, Zhang2022Counteracting}, the  in streaming recommendation needs to make a trade-off between exploitation and exploration during the recommendation process, and continuously and incrementally update its recommendation policy~\citep{Chandramouli2011Streamrec, Chang2017Streaming, Jakomin2020Simultaneous}. 

% \begin{figure}
%     \centering
%     \setlength{\belowcaptionskip}{-10pt}
%     \includegraphics[width=.43\textwidth]{fig/IL mechanism.png}
%     \caption{Imitation Learning (IL) approaches often hold the view that interactions made by experts are experienced, which may not conform to streaming scenarios since even the expert has to evolve from novice to experienced.}
%     \label{fig:IL:mechanism}
% \end{figure}

% In the behavioral evolution history, there exist a significant amount of contradictory data where an expert may take different actions when facing the same context at different time periods. This contradicts the assumption made by traditional imitation learning (IL) approaches regarding the consistency of expert behavior data. Therefore, directly applying existing IL methods to recover the behavior policy from the expert's behavioral evolution history is not reasonable. For example, behavior cloning (BC) approaches are highly sensitive to distribution drift and contradictory data, and inconsistencies in the expert's evolution history can lead to a sharp decline in the final recovery performance.
% Furthermore, some IL approaches rely on large-scale iterations of Metropolis-Hastings sampling to achieve accurate estimation in universal scenarios~\citep{Ramachandran2007Bayesian, Choi2011MAP}. However, these approaches overlook the exploitation-exploration mechanism in expert interactions and demonstrate low sample efficiency when dealing with large-scale interaction data. While recent work by ~\citet{Huyuk2022Inverse} focused on contextual bandits, it cannot be adapted to the batched bandit setting as it assumes the expert updates the policy in a fully-online manner. Additionally, existing inverse bandit approaches typically employ sampling techniques to estimate the likelihood, resulting in low training efficiency. 
% There is an urgent need to develop inverse bandit methods specifically designed for the more general batched bandit setting and to devise novel techniques for recovering parameters tailored for bandit polices.
% \iffalse
% % This document details the formatting requirements for anonymous submissions. The requirements are the same as for camera ready papers but with a few notable differences:

% % \begin{itemize}
% %     \item Anonymous submissions must not include the author names and affiliations. Write ``Anonymous Submission'' as the ``sole author'' and leave the affiliations empty.
% %     \item The PDF document's metadata should be cleared with a metadata-cleaning tool before submitting it. This is to prevent leaked information from revealing your identity.
% %     \item References must be anonymized whenever the reader can infer that they are to the authors' previous work.
% %     \item anonymous's copyright notice should not be included as a footer in the first page.
% %     \item Only the PDF version is required at this stage. No source versions will be requested, nor any copyright transfer form.
% % \end{itemize}

% % You can remove the copyright notice and ensure that your names aren't shown by including \texttt{submission} option when loading the \texttt{anonymous25} package:

% % \begin{quote}\begin{scriptsize}\begin{verbatim}
% % \documentclass[letterpaper]{article}
% % \usepackage[submission]{anonymous25}
% % \end{verbatim}\end{scriptsize}\end{quote}

% % The remainder of this document are the original camera-
% % ready instructions. Any contradiction of the above points
% % ought to be ignored while preparing anonymous submis-
% % sions.


% \section{Camera-Ready Guidelines}

% Congratulations on having a paper selected for inclusion in an anonymous Press proceedings or technical report! This document details the requirements necessary to get your accepted paper published using PDF\LaTeX{}. If you are using Microsoft Word, instructions are provided in a different document. anonymous Press does not support any other formatting software.

% The instructions herein are provided as a general guide for experienced \LaTeX{} users. If you do not know how to use \LaTeX{}, please obtain assistance locally. anonymous cannot provide you with support and the accompanying style files are \textbf{not} guaranteed to work. If the results you obtain are not in accordance with the specifications you received, you must correct your source file to achieve the correct result.

% These instructions are generic. Consequently, they do not include specific dates, page charges, and so forth. Please consult your specific written conference instructions for details regarding your submission. Please review the entire document for specific instructions that might apply to your particular situation. All authors must comply with the following:

% \begin{itemize}
% \item You must use the 2025 anonymous Press \LaTeX{} style file and the anonymous25.bst bibliography style files, which are located in the 2025 anonymous Author Kit (anonymous25.sty, anonymous25.bst).
% \item You must complete, sign, and return by the deadline the anonymous copyright form (unless directed by anonymous Press to use the anonymous Distribution License instead).
% \item You must read and format your paper source and PDF according to the formatting instructions for authors.
% \item You must submit your electronic files and abstract using our electronic submission form \textbf{on time.}
% \item You must pay any required page or formatting charges to anonymous Press so that they are received by the deadline.
% \item You must check your paper before submitting it, ensuring that it compiles without error, and complies with the guidelines found in the anonymous Author Kit.
% \end{itemize}

% \section{Copyright}
% All papers submitted for publication by anonymous Press must be accompanied by a valid signed copyright form. They must also contain the anonymous copyright notice at the bottom of the first page of the paper. There are no exceptions to these requirements. If you fail to provide us with a signed copyright form or disable the copyright notice, we will be unable to publish your paper. There are \textbf{no exceptions} to this policy. You will find a PDF version of the anonymous copyright form in the anonymous AuthorKit. Please see the specific instructions for your conference for submission details.

% \section{Formatting Requirements in Brief}
% We need source and PDF files that can be used in a variety of ways and can be output on a variety of devices. The design and appearance of the paper is strictly governed by the anonymous style file (anonymous25.sty).
% \textbf{You must not make any changes to the anonymous style file, nor use any commands, packages, style files, or macros within your own paper that alter that design, including, but not limited to spacing, floats, margins, fonts, font size, and appearance.} anonymous imposes requirements on your source and PDF files that must be followed. Most of these requirements are based on our efforts to standardize conference manuscript properties and layout. All papers submitted to anonymous for publication will be recompiled for standardization purposes. Consequently, every paper submission must comply with the following requirements:

% \begin{itemize}
% \item Your .tex file must compile in PDF\LaTeX{} --- (you may not include .ps or .eps figure files.)
% \item All fonts must be embedded in the PDF file --- including your figures.
% \item Modifications to the style file, whether directly or via commands in your document may not ever be made, most especially when made in an effort to avoid extra page charges or make your paper fit in a specific number of pages.
% \item No type 3 fonts may be used (even in illustrations).
% \item You may not alter the spacing above and below captions, figures, headings, and subheadings.
% \item You may not alter the font sizes of text elements, footnotes, heading elements, captions, or title information (for references and mathematics, please see the limited exceptions provided herein).
% \item You may not alter the line spacing of text.
% \item Your title must follow Title Case capitalization rules (not sentence case).
% \item \LaTeX{} documents must use the Times or Nimbus font package (you may not use Computer Modern for the text of your paper).
% \item No \LaTeX{} 209 documents may be used or submitted.
% \item Your source must not require use of fonts for non-Roman alphabets within the text itself. If your paper includes symbols in other languages (such as, but not limited to, Arabic, Chinese, Hebrew, Japanese, Thai, Russian and other Cyrillic languages), you must restrict their use to bit-mapped figures. Fonts that require non-English language support (CID and Identity-H) must be converted to outlines or 300 dpi bitmap or removed from the document (even if they are in a graphics file embedded in the document).
% \item Two-column format in anonymous style is required for all papers.
% \item The paper size for final submission must be US letter without exception.
% \item The source file must exactly match the PDF.
% \item The document margins may not be exceeded (no overfull boxes).
% \item The number of pages and the file size must be as specified for your event.
% \item No document may be password protected.
% \item Neither the PDFs nor the source may contain any embedded links or bookmarks (no hyperref or navigator packages).
% \item Your source and PDF must not have any page numbers, footers, or headers (no pagestyle commands).
% \item Your PDF must be compatible with Acrobat 5 or higher.
% \item Your \LaTeX{} source file (excluding references) must consist of a \textbf{single} file (use of the ``input" command is not allowed.
% \item Your graphics must be sized appropriately outside of \LaTeX{} (do not use the ``clip" or ``trim'' command) .
% \end{itemize}

% If you do not follow these requirements, your paper will be returned to you to correct the deficiencies.

% \section{What Files to Submit}
% You must submit the following items to ensure that your paper is published:
% \begin{itemize}
% \item A fully-compliant PDF file.
% \item Your \LaTeX{} source file submitted as a \textbf{single} .tex file (do not use the ``input" command to include sections of your paper --- every section must be in the single source file). (The only allowable exception is .bib file, which should be included separately).
% \item The bibliography (.bib) file(s).
% \item Your source must compile on our system, which includes only standard \LaTeX{} 2020 TeXLive support files.
% \item Only the graphics files used in compiling paper.
% \item The \LaTeX{}-generated files (e.g. .aux,  .bbl file, PDF, etc.).
% \end{itemize}

% Your \LaTeX{} source will be reviewed and recompiled on our system (if it does not compile, your paper will be returned to you. \textbf{Do not submit your source in multiple text files.} Your single \LaTeX{} source file must include all your text, your bibliography (formatted using anonymous25.bst), and any custom macros.

% Your files should work without any supporting files (other than the program itself) on any computer with a standard \LaTeX{} distribution.

% \textbf{Do not send files that are not actually used in the paper.} Avoid including any files not needed for compiling your paper, including, for example, this instructions file, unused graphics files, style files, additional material sent for the purpose of the paper review, intermediate build files and so forth.

% \textbf{Obsolete style files.} The commands for some common packages (such as some used for algorithms), may have changed. Please be certain that you are not compiling your paper using old or obsolete style files.

% \textbf{Final Archive.} Place your source files in a single archive which should be compressed using .zip. The final file size may not exceed 10 MB.
% Name your source file with the last (family) name of the first author, even if that is not you.


% \section{Using \LaTeX{} to Format Your Paper}

% The latest version of the anonymous style file is available on anonymous's website. Download this file and place it in the \TeX\ search path. Placing it in the same directory as the paper should also work. You must download the latest version of the complete anonymous Author Kit so that you will have the latest instruction set and style file.

% \subsection{Document Preamble}

% In the \LaTeX{} source for your paper, you \textbf{must} place the following lines as shown in the example in this subsection. This command set-up is for three authors. Add or subtract author and address lines as necessary, and uncomment the portions that apply to you. In most instances, this is all you need to do to format your paper in the Times font. The helvet package will cause Helvetica to be used for sans serif. These files are part of the PSNFSS2e package, which is freely available from many Internet sites (and is often part of a standard installation).

% Leave the setcounter for section number depth commented out and set at 0 unless you want to add section numbers to your paper. If you do add section numbers, you must uncomment this line and change the number to 1 (for section numbers), or 2 (for section and subsection numbers). The style file will not work properly with numbering of subsubsections, so do not use a number higher than 2.

% \subsubsection{The Following Must Appear in Your Preamble}
% \begin{quote}
% \begin{scriptsize}\begin{verbatim}
% \documentclass[letterpaper]{article}
% % DO NOT CHANGE THIS
% \usepackage[submission]{anonymous25} % DO NOT CHANGE THIS
% \usepackage{times} % DO NOT CHANGE THIS
% \usepackage{helvet} % DO NOT CHANGE THIS
% \usepackage{courier} % DO NOT CHANGE THIS
% \usepackage[hyphens]{url} % DO NOT CHANGE THIS
% \usepackage{graphicx} % DO NOT CHANGE THIS
% \urlstyle{rm} % DO NOT CHANGE THIS
% \def\UrlFont{\rm} % DO NOT CHANGE THIS
% \usepackage{graphicx}  % DO NOT CHANGE THIS
% \usepackage{natbib}  % DO NOT CHANGE THIS
% \usepackage{caption}  % DO NOT CHANGE THIS
% \frenchspacing % DO NOT CHANGE THIS
% \setlength{\pdfpagewidth}{8.5in} % DO NOT CHANGE THIS
% \setlength{\pdfpageheight}{11in} % DO NOT CHANGE THIS
% %
% % Keep the \pdfinfo as shown here. There's no need
% % for you to add the /Title and /Author tags.
% \pdfinfo{
% /TemplateVersion (2025.1)
% }
% \end{verbatim}\end{scriptsize}
% \end{quote}

% \subsection{Preparing Your Paper}

% After the preamble above, you should prepare your paper as follows:
% \begin{quote}
% \begin{scriptsize}\begin{verbatim}
% \begin{document}
% \maketitle
% \begin{abstract}
% %...
% \end{abstract}\end{verbatim}\end{scriptsize}
% \end{quote}

% \noindent If you want to add links to the paper's code, dataset(s), and extended version or similar this is the place to add them, within a \emph{links} environment:
% \begin{quote}%
% \begin{scriptsize}\begin{verbatim}
% \begin{links}
%   \link{Code}{https://anonymous.org/example/guidelines}
%   \link{Datasets}{https://anonymous.org/example/datasets}
%   \link{Extended version}{https://anonymous.org/example}
% \end{links}\end{verbatim}\end{scriptsize}
% \end{quote}
% \noindent Make sure that you do not de-anonymize yourself with these links.

% \noindent You should then continue with the body of your paper. Your paper must conclude with the references, which should be inserted as follows:
% \begin{quote}
% \begin{scriptsize}\begin{verbatim}
% % References and End of Paper
% % These lines must be placed at the end of your paper
% \bibliography{Bibliography-File}
% \end{document}
% \end{verbatim}\end{scriptsize}
% \end{quote}

% \begin{quote}
% \begin{scriptsize}\begin{verbatim}
% \begin{document}\\
% \maketitle\\
% ...\\
% \bibliography{Bibliography-File}\\
% \end{document}\\
% \end{verbatim}\end{scriptsize}
% \end{quote}




% \subsection{Commands and Packages That May Not Be Used}
% \begin{table*}[t]
% \centering

% \begin{tabular}{l|l|l|l}
% \textbackslash abovecaption &
% \textbackslash abovedisplay &
% \textbackslash addevensidemargin &
% \textbackslash addsidemargin \\
% \textbackslash addtolength &
% \textbackslash baselinestretch &
% \textbackslash belowcaption &
% \textbackslash belowdisplay \\
% \textbackslash break &
% \textbackslash clearpage &
% \textbackslash clip &
% \textbackslash columnsep \\
% \textbackslash float &
% \textbackslash input &
% \textbackslash input &
% \textbackslash linespread \\
% \textbackslash newpage &
% \textbackslash pagebreak &
% \textbackslash renewcommand &
% \textbackslash setlength \\
% \textbackslash text height &
% \textbackslash tiny &
% \textbackslash top margin &
% \textbackslash trim \\
% \textbackslash vskip\{- &
% \textbackslash vspace\{- \\
% \end{tabular}
% %}
% \caption{Commands that must not be used}
% \label{table1}
% \end{table*}




% \begin{table}[t]
% \centering
% %\resizebox{.95\columnwidth}{!}{
% \begin{tabular}{l|l|l|l}
%     authblk & babel & cjk & dvips \\
%     epsf & epsfig & euler & float \\
%     fullpage & geometry & graphics & hyperref \\
%     layout & linespread & lmodern & maltepaper \\
%     navigator & pdfcomment & pgfplots & psfig \\
%     pstricks & t1enc & titlesec & tocbind \\
%     ulem
% \end{tabular}
% \caption{LaTeX style packages that must not be used.}
% \label{table2}
% \end{table}

% There are a number of packages, commands, scripts, and macros that are incompatable with anonymous25.sty. The common ones are listed in Tab.~\ref{table1} and Tab.~\ref{table2}. Generally, if a command, package, script, or macro alters floats, margins, fonts, sizing, linespacing, or the presentation of the references and citations, it is unacceptable. Note that negative vskip and vspace may not be used except in certain rare occurances, and may never be used around tables, figures, captions, sections, subsections, subsubsections, or references.


% \subsection{Page Breaks}
% For your final camera ready copy, you must not use any page break commands. References must flow directly after the text without breaks. Note that some conferences require references to be on a separate page during the review process. anonymous Press, however, does not require this condition for the final paper.


% \subsection{Paper Size, Margins, and Column Width}
% Papers must be formatted to print in two-column format on 8.5 x 11 inch US letter-sized paper. The margins must be exactly as follows:
% \begin{itemize}
% \item Top margin: 1.25 inches (first page), .75 inches (others)
% \item Left margin: .75 inches
% \item Right margin: .75 inches
% \item Bottom margin: 1.25 inches
% \end{itemize}


% The default paper size in most installations of \LaTeX{} is A4. However, because we require that your electronic paper be formatted in US letter size, the preamble we have provided includes commands that alter the default to US letter size. Please note that using any other package to alter page size (such as, but not limited to the Geometry package) will result in your final paper being returned to you for correction.


% \subsubsection{Column Width and Margins.}
% To ensure maximum readability, your paper must include two columns. Each column should be 3.3 inches wide (slightly more than 3.25 inches), with a .375 inch (.952 cm) gutter of white space between the two columns. The anonymous25.sty file will automatically create these columns for you.

% \subsection{Overlength Papers}
% If your paper is too long and you resort to formatting tricks to make it fit, it is quite likely that it will be returned to you. The best way to retain readability if the paper is overlength is to cut text, figures, or tables. There are a few acceptable ways to reduce paper size that don't affect readability. First, turn on \textbackslash frenchspacing, which will reduce the space after periods. Next, move all your figures and tables to the top of the page. Consider removing less important portions of a figure. If you use \textbackslash centering instead of \textbackslash begin\{center\} in your figure environment, you can also buy some space. For mathematical environments, you may reduce fontsize {\bf but not below 6.5 point}.


% Commands that alter page layout are forbidden. These include \textbackslash columnsep,  \textbackslash float, \textbackslash topmargin, \textbackslash topskip, \textbackslash textheight, \textbackslash textwidth, \textbackslash oddsidemargin, and \textbackslash evensizemargin (this list is not exhaustive). If you alter page layout, you will be required to pay the page fee. Other commands that are questionable and may cause your paper to be rejected include \textbackslash parindent, and \textbackslash parskip. Commands that alter the space between sections are forbidden. The title sec package is not allowed. Regardless of the above, if your paper is obviously ``squeezed" it is not going to to be accepted. Options for reducing the length of a paper include reducing the size of your graphics, cutting text, or paying the extra page charge (if it is offered).


% \subsection{Type Font and Size}
% Your paper must be formatted in Times Roman or Nimbus. We will not accept papers formatted using Computer Modern or Palatino or some other font as the text or heading typeface. Sans serif, when used, should be Courier. Use Symbol or Lucida or Computer Modern for \textit{mathematics only. }

% Do not use type 3 fonts for any portion of your paper, including graphics. Type 3 bitmapped fonts are designed for fixed resolution printers. Most print at 300 dpi even if the printer resolution is 1200 dpi or higher. They also often cause high resolution imagesetter devices to crash. Consequently, anonymous will not accept electronic files containing obsolete type 3 fonts. Files containing those fonts (even in graphics) will be rejected. (Authors using blackboard symbols must avoid packages that use type 3 fonts.)

% Fortunately, there are effective workarounds that will prevent your file from embedding type 3 bitmapped fonts. The easiest workaround is to use the required times, helvet, and courier packages with \LaTeX{}2e. (Note that papers formatted in this way will still use Computer Modern for the mathematics. To make the math look good, you'll either have to use Symbol or Lucida, or you will need to install type 1 Computer Modern fonts --- for more on these fonts, see the section ``Obtaining Type 1 Computer Modern.")

% If you are unsure if your paper contains type 3 fonts, view the PDF in Acrobat Reader. The Properties/Fonts window will display the font name, font type, and encoding properties of all the fonts in the document. If you are unsure if your graphics contain type 3 fonts (and they are PostScript or encapsulated PostScript documents), create PDF versions of them, and consult the properties window in Acrobat Reader.

% The default size for your type must be ten-point with twelve-point leading (line spacing). Start all pages (except the first) directly under the top margin. (See the next section for instructions on formatting the title page.) Indent ten points when beginning a new paragraph, unless the paragraph begins directly below a heading or subheading.


% \subsubsection{Obtaining Type 1 Computer Modern for \LaTeX{}.}

% If you use Computer Modern for the mathematics in your paper (you cannot use it for the text) you may need to download type 1 Computer fonts. They are available without charge from the American Mathematical Society:
% http://www.ams.org/tex/type1-fonts.html.

% \subsubsection{Nonroman Fonts.}
% If your paper includes symbols in other languages (such as, but not limited to, Arabic, Chinese, Hebrew, Japanese, Thai, Russian and other Cyrillic languages), you must restrict their use to bit-mapped figures.

% \subsection{Title and Authors}
% Your title must appear centered over both text columns in sixteen-point bold type (twenty-four point leading). The title must be written in Title Case according to the Chicago Manual of Style rules. The rules are a bit involved, but in general verbs (including short verbs like be, is, using, and go), nouns, adverbs, adjectives, and pronouns should be capitalized, (including both words in hyphenated terms), while articles, conjunctions, and prepositions are lower case unless they directly follow a colon or long dash. You can use the online tool \url{https://titlecaseconverter.com/} to double-check the proper capitalization (select the "Chicago" style and mark the "Show explanations" checkbox).

% Author's names should appear below the title of the paper, centered in twelve-point type (with fifteen point leading), along with affiliation(s) and complete address(es) (including electronic mail address if available) in nine-point roman type (the twelve point leading). You should begin the two-column format when you come to the abstract.

% \subsubsection{Formatting Author Information.}
% Author information has to be set according to the following specification depending if you have one or more than one affiliation. You may not use a table nor may you employ the \textbackslash authorblk.sty package. For one or several authors from the same institution, please separate them with commas and write all affiliation directly below (one affiliation per line) using the macros \textbackslash author and \textbackslash affiliations:

% \begin{quote}\begin{scriptsize}\begin{verbatim}
% \author{
%     Author 1, ..., Author n\\
% }
% \affiliations {
%     Address line\\
%     ... \\
%     Address line\\
% }
% \end{verbatim}\end{scriptsize}\end{quote}


% \noindent For authors from different institutions, use \textbackslash textsuperscript \{\textbackslash rm x \} to match authors and affiliations. Notice that there should not be any spaces between the author name (or comma following it) and the superscript.

% \begin{quote}\begin{scriptsize}\begin{verbatim}
% \author{
%     AuthorOne\equalcontrib\textsuperscript{\rm 1,\rm 2},
%     AuthorTwo\equalcontrib\textsuperscript{\rm 2},
%     AuthorThree\textsuperscript{\rm 3},\\
%     AuthorFour\textsuperscript{\rm 4},
%     AuthorFive \textsuperscript{\rm 5}}
% }
% \affiliations {
%     \textsuperscript{\rm 1}AffiliationOne,\\
%     \textsuperscript{\rm 2}AffiliationTwo,\\
%     \textsuperscript{\rm 3}AffiliationThree,\\
%     \textsuperscript{\rm 4}AffiliationFour,\\
%     \textsuperscript{\rm 5}AffiliationFive\\
%     \{email, email\}@affiliation.com,
%     email@affiliation.com,
%     email@affiliation.com,
%     email@affiliation.com
% }
% \end{verbatim}\end{scriptsize}\end{quote}

% You can indicate that some authors contributed equally using the \textbackslash equalcontrib command. This will add a marker after the author names and a footnote on the first page.

% Note that you may want to  break the author list for better visualization. You can achieve this using a simple line break (\textbackslash  \textbackslash).

% \subsection{\LaTeX{} Copyright Notice}
% The copyright notice automatically appears if you use anonymous25.sty. It has been hardcoded and may not be disabled.

% \subsection{Credits}
% Any credits to a sponsoring agency should appear in the acknowledgments section, unless the agency requires different placement. If it is necessary to include this information on the front page, use
% \textbackslash thanks in either the \textbackslash author or \textbackslash title commands.
% For example:
% \begin{quote}
% \begin{small}
% \textbackslash title\{Very Important Results in AI\textbackslash thanks\{This work is
%  supported by everybody.\}\}
% \end{small}
% \end{quote}
% Multiple \textbackslash thanks commands can be given. Each will result in a separate footnote indication in the author or title with the corresponding text at the botton of the first column of the document. Note that the \textbackslash thanks command is fragile. You will need to use \textbackslash protect.

% Please do not include \textbackslash pubnote commands in your document.

% \subsection{Abstract}
% Follow the example commands in this document for creation of your abstract. The command \textbackslash begin\{abstract\} will automatically indent the text block. Please do not indent it further. {Do not include references in your abstract!}

% \subsection{Page Numbers}

% Do not print any page numbers on your paper. The use of \textbackslash pagestyle is forbidden.

% \subsection{Text}
% The main body of the paper must be formatted in black, ten-point Times Roman with twelve-point leading (line spacing). You may not reduce font size or the linespacing. Commands that alter font size or line spacing (including, but not limited to baselinestretch, baselineshift, linespread, and others) are expressly forbidden. In addition, you may not use color in the text.

% \subsection{Citations}
% Citations within the text should include the author's last name and year, for example (Newell 1980). Append lower-case letters to the year in cases of ambiguity. Multiple authors should be treated as follows: (Feigenbaum and Engelmore 1988) or (Ford, Hayes, and Glymour 1992). In the case of four or more authors, list only the first author, followed by et al. (Ford et al. 1997).

% \subsection{Extracts}
% Long quotations and extracts should be indented ten points from the left and right margins.

% \begin{quote}
% This is an example of an extract or quotation. Note the indent on both sides. Quotation marks are not necessary if you offset the text in a block like this, and properly identify and cite the quotation in the text.

% \end{quote}

% \subsection{Footnotes}
% Use footnotes judiciously, taking into account that they interrupt the reading of the text. When required, they should be consecutively numbered throughout with superscript Arabic numbers. Footnotes should appear at the bottom of the page, separated from the text by a blank line space and a thin, half-point rule.

% \subsection{Headings and Sections}
% When necessary, headings should be used to separate major sections of your paper. Remember, you are writing a short paper, not a lengthy book! An overabundance of headings will tend to make your paper look more like an outline than a paper. The anonymous25.sty package will create headings for you. Do not alter their size nor their spacing above or below.

% \subsubsection{Section Numbers.}
% The use of section numbers in anonymous Press papers is optional. To use section numbers in \LaTeX{}, uncomment the setcounter line in your document preamble and change the 0 to a 1. Section numbers should not be used in short poster papers and/or extended abstracts.

% \subsubsection{Section Headings.}
% Sections should be arranged and headed as follows:
% \begin{enumerate}
% \item Main content sections
% \item Appendices (optional)
% \item Ethical Statement (optional, unnumbered)
% \item Acknowledgements (optional, unnumbered)
% \item References (unnumbered)
% \end{enumerate}

% \subsubsection{Appendices.}
% Any appendices must appear after the main content. If your main sections are numbered, appendix sections must use letters instead of arabic numerals. In \LaTeX{} you can use the \texttt{\textbackslash appendix} command to achieve this effect and then use \texttt{\textbackslash section\{Heading\}} normally for your appendix sections.

% \subsubsection{Ethical Statement.}
% You can write a statement about the potential ethical impact of your work, including its broad societal implications, both positive and negative. If included, such statement must be written in an unnumbered section titled \emph{Ethical Statement}.

% \subsubsection{Acknowledgments.}
% The acknowledgments section, if included, appears right before the references and is headed ``Acknowledgments". It must not be numbered even if other sections are (use \texttt{\textbackslash section*\{Acknowledgements\}} in \LaTeX{}). This section includes acknowledgments of help from associates and colleagues, credits to sponsoring agencies, financial support, and permission to publish. Please acknowledge other contributors, grant support, and so forth, in this section. Do not put acknowledgments in a footnote on the first page. If your grant agency requires acknowledgment of the grant on page 1, limit the footnote to the required statement, and put the remaining acknowledgments at the back. Please try to limit acknowledgments to no more than three sentences.

% \subsubsection{References.}
% The references section should be labeled ``References" and must appear at the very end of the paper (don't end the paper with references, and then put a figure by itself on the last page). A sample list of references is given later on in these instructions. Please use a consistent format for references. Poorly prepared or sloppy references reflect badly on the quality of your paper and your research. Please prepare complete and accurate citations.

% \subsection{Illustrations and  Figures}

% \begin{figure}[t]
% \centering
% \includegraphics[width=0.9\columnwidth]{figure1} % Reduce the figure size so that it is slightly narrower than the column. Don't use precise values for figure width.This setup will avoid overfull boxes.
% \caption{Using the trim and clip commands produces fragile layers that can result in disasters (like this one from an actual paper) when the color space is corrected or the PDF combined with others for the final proceedings. Crop your figures properly in a graphics program -- not in LaTeX.}
% \label{fig1}
% \end{figure}

% \begin{figure*}[t]
% \centering
% \includegraphics[width=0.8\textwidth]{figure2} % Reduce the figure size so that it is slightly narrower than the column.
% \caption{Adjusting the bounding box instead of actually removing the unwanted data resulted multiple layers in this paper. It also needlessly increased the PDF size. In this case, the size of the unwanted layer doubled the paper's size, and produced the following surprising results in final production. Crop your figures properly in a graphics program. Don't just alter the bounding box.}
% \label{fig2}
% \end{figure*}

% % Using the \centering command instead of \begin{center} ... \end{center} will save space
% % Positioning your figure at the top of the page will save space and make the paper more readable
% % Using 0.95\columnwidth in conjunction with the


% Your paper must compile in PDF\LaTeX{}. Consequently, all your figures must be .jpg, .png, or .pdf. You may not use the .gif (the resolution is too low), .ps, or .eps file format for your figures.

% Figures, drawings, tables, and photographs should be placed throughout the paper on the page (or the subsequent page) where they are first discussed. Do not group them together at the end of the paper. If placed at the top of the paper, illustrations may run across both columns. Figures must not invade the top, bottom, or side margin areas. Figures must be inserted using the \textbackslash usepackage\{graphicx\}. Number figures sequentially, for example, figure 1, and so on. Do not use minipage to group figures.

% If you normally create your figures using pgfplots, please create the figures first, and then import them as pdfs with proper bounding boxes, as the bounding and trim boxes created by pfgplots are fragile and not valid.

% When you include your figures, you must crop them \textbf{outside} of \LaTeX{}. The command \textbackslash includegraphics*[clip=true, viewport 0 0 10 10]{...} might result in a PDF that looks great, but the image is \textbf{not really cropped.} The full image can reappear (and obscure whatever it is overlapping) when page numbers are applied or color space is standardized. Fig.~\ref{fig1}, and Fig.~\ref{fig2} display some unwanted results that often occur.

% If your paper includes illustrations that are not compatible with PDF\TeX{} (such as .eps or .ps documents), you will need to convert them. The epstopdf package will usually work for eps files. You will need to convert your ps files to PDF in either case.

% \subsubsection {Figure Captions.}The illustration number and caption must appear \textit{under} the illustration. Labels and other text with the actual illustration must be at least nine-point type. However, the font and size of figure captions must be 10 point roman. Do not make them smaller, bold, or italic. (Individual words may be italicized if the context requires differentiation.)

% \subsection{Tables}

% \subsection{Tables}

% Tables should be presented in 10 point roman type. If necessary, they may be altered to 9 point type. You must not use \texttt{\textbackslash resizebox} or other commands that resize the entire table to make it smaller, because you can't control the final font size this way.
% If your table is too large you can use \texttt{\textbackslash setlength\{\textbackslash tabcolsep\}\{1mm\}} to compress the columns a bit or you can adapt the content (e.g.: reduce the decimal precision when presenting numbers, use shortened column titles, make some column duble-line to get it narrower).

% Tables that do not fit in a single column must be placed across double columns. If your table won't fit within the margins even when spanning both columns and using the above techniques, you must split it in two separate tables.

% \subsubsection {Table Captions.} The number and caption for your table must appear \textit{under} (not above) the table.  Additionally, the font and size of table captions must be 10 point roman and must be placed beneath the figure. Do not make them smaller, bold, or italic. (Individual words may be italicized if the context requires differentiation.)



% \subsubsection{Low-Resolution Bitmaps.}
% You may not use low-resolution (such as 72 dpi) screen-dumps and GIF files---these files contain so few pixels that they are always blurry, and illegible when printed. If they are color, they will become an indecipherable mess when converted to black and white. This is always the case with gif files, which should never be used. The resolution of screen dumps can be increased by reducing the print size of the original file while retaining the same number of pixels. You can also enlarge files by manipulating them in software such as PhotoShop. Your figures should be 300 dpi when incorporated into your document.

% \subsubsection{\LaTeX{} Overflow.}
% \LaTeX{} users please beware: \LaTeX{} will sometimes put portions of the figure or table or an equation in the margin. If this happens, you need to make the figure or table span both columns. If absolutely necessary, you may reduce the figure, or reformat the equation, or reconfigure the table.{ \bf Check your log file!} You must fix any overflow into the margin (that means no overfull boxes in \LaTeX{}). \textbf{Nothing is permitted to intrude into the margin or gutter.}


% \subsubsection{Using Color.}
% Use of color is restricted to figures only. It must be WACG 2.0 compliant. (That is, the contrast ratio must be greater than 4.5:1 no matter the font size.) It must be CMYK, NOT RGB. It may never be used for any portion of the text of your paper. The archival version of your paper will be printed in black and white and grayscale. The web version must be readable by persons with disabilities. Consequently, because conversion to grayscale can cause undesirable effects (red changes to black, yellow can disappear, and so forth), we strongly suggest you avoid placing color figures in your document. If you do include color figures, you must (1) use the CMYK (not RGB) colorspace and (2) be mindful of readers who may happen to have trouble distinguishing colors. Your paper must be decipherable without using color for distinction.

% \subsubsection{Drawings.}
% We suggest you use computer drawing software (such as Adobe Illustrator or, (if unavoidable), the drawing tools in Microsoft Word) to create your illustrations. Do not use Microsoft Publisher. These illustrations will look best if all line widths are uniform (half- to two-point in size), and you do not create labels over shaded areas. Shading should be 133 lines per inch if possible. Use Times Roman or Helvetica for all figure call-outs. \textbf{Do not use hairline width lines} --- be sure that the stroke width of all lines is at least .5 pt. Zero point lines will print on a laser printer, but will completely disappear on the high-resolution devices used by our printers.

% \subsubsection{Photographs and Images.}
% Photographs and other images should be in grayscale (color photographs will not reproduce well; for example, red tones will reproduce as black, yellow may turn to white, and so forth) and set to a minimum of 300 dpi. Do not prescreen images.

% \subsubsection{Resizing Graphics.}
% Resize your graphics \textbf{before} you include them with LaTeX. You may \textbf{not} use trim or clip options as part of your \textbackslash includegraphics command. Resize the media box of your PDF using a graphics program instead.

% \subsubsection{Fonts in Your Illustrations.}
% You must embed all fonts in your graphics before including them in your LaTeX document.

% \subsubsection{Algorithms.}
% Algorithms and/or programs are a special kind of figures. Like all illustrations, they should appear floated to the top (preferably) or bottom of the page. However, their caption should appear in the header, left-justified and enclosed between horizontal lines, as shown in Algorithm~\ref{alg:algorithm}. The algorithm body should be terminated with another horizontal line. It is up to the authors to decide whether to show line numbers or not, how to format comments, etc.

% In \LaTeX{} algorithms may be typeset using the {\tt algorithm} and {\tt algorithmic} packages, but you can also use one of the many other packages for the task.

% \begin{algorithm}[tb]
% \caption{Example algorithm}
% \label{alg:algorithm}
% \textbf{Input}: Your algorithm's input\\
% \textbf{Parameter}: Optional list of parameters\\
% \textbf{Output}: Your algorithm's output
% \begin{algorithmic}[1] %[1] enables line numbers
% \STATE Let $t=0$.
% \WHILE{condition}
% \STATE Do some action.
% \IF {conditional}
% \STATE Perform task A.
% \ELSE
% \STATE Perform task B.
% \ENDIF
% \ENDWHILE
% \STATE \textbf{return} solution
% \end{algorithmic}
% \end{algorithm}

% \subsubsection{Listings.}
% Listings are much like algorithms and programs. They should also appear floated to the top (preferably) or bottom of the page. Listing captions should appear in the header, left-justified and enclosed between horizontal lines as shown in Listing~\ref{lst:listing}. Terminate the body with another horizontal line and avoid any background color. Line numbers, if included, must appear within the text column.

% \begin{listing}[tb]%
% \caption{Example listing {\tt quicksort.hs}}%
% \label{lst:listing}%
% \begin{lstlisting}[language=Haskell]
% quicksort :: Ord a => [a] -> [a]
% quicksort []     = []
% quicksort (p:xs) = (quicksort lesser) ++ [p] ++ (quicksort greater)
% 	where
% 		lesser  = filter (< p) xs
% 		greater = filter (>= p) xs
% \end{lstlisting}
% \end{listing}

% \subsection{References}
% The anonymous style includes a set of definitions for use in formatting references with BibTeX. These definitions make the bibliography style fairly close to the ones  specified in the Reference Examples appendix below. To use these definitions, you also need the BibTeX style file ``anonymous25.bst," available in the anonymous Author Kit on the anonymous web site. Then, at the end of your paper but before \textbackslash end{document}, you need to put the following lines:

% \begin{quote}
% \begin{small}
% \textbackslash bibliography\{bibfile1,bibfile2,...\}
% \end{small}
% \end{quote}

% Please note that the anonymous25.sty class already sets the bibliographystyle for you, so you do not have to place any \textbackslash bibliographystyle command in the document yourselves. The anonymous25.sty file is incompatible with the hyperref and navigator packages. If you use either, your references will be garbled and your paper will be returned to you.

% References may be the same size as surrounding text.
% However, in this section (only), you may reduce the size to {\em \textbackslash small} (9pt) if your paper exceeds the allowable number of pages. Making it any smaller than 9 point with 10 point linespacing, however, is not allowed.

% The list of files in the \textbackslash bibliography command should be the names of your BibTeX source files (that is, the .bib files referenced in your paper).

% The following commands are available for your use in citing references:
% \begin{quote}
% {\em \textbackslash cite:} Cites the given reference(s) with a full citation. This appears as ``(Author Year)'' for one reference, or ``(Author Year; Author Year)'' for multiple references.\smallskip\\
% {\em \textbackslash shortcite:} Cites the given reference(s) with just the year. This appears as ``(Year)'' for one reference, or ``(Year; Year)'' for multiple references.\smallskip\\
% {\em \textbackslash citeauthor:} Cites the given reference(s) with just the author name(s) and no parentheses.\smallskip\\
% {\em \textbackslash citeyear:} Cites the given reference(s) with just the date(s) and no parentheses.
% \end{quote}
% You may also use any of the \emph{natbib} citation commands.


% \section{Proofreading Your PDF}
% Please check all the pages of your PDF file. The most commonly forgotten element is the acknowledgements --- especially the correct grant number. Authors also commonly forget to add the metadata to the source, use the wrong reference style file, or don't follow the capitalization rules or comma placement for their author-title information properly. A final common problem is text (expecially equations) that runs into the margin. You will need to fix these common errors before submitting your file.

% \section{Improperly Formatted Files }
% In the past, anonymous has corrected improperly formatted files submitted by the authors. Unfortunately, this has become an increasingly burdensome expense that we can no longer absorb). Consequently, if your file is improperly formatted, it will be returned to you for correction.

% \section{Naming Your Electronic File}
% We require that you name your \LaTeX{} source file with the last name (family name) of the first author so that it can easily be differentiated from other submissions. Complete file-naming instructions will be provided to you in the submission instructions.

% \section{Submitting Your Electronic Files to anonymous}
% Instructions on paper submittal will be provided to you in your acceptance letter.

% \section{Inquiries}
% If you have any questions about the preparation or submission of your paper as instructed in this document, please contact anonymous Press at the address given below. If you have technical questions about implementation of the anonymous style file, please contact an expert at your site. We do not provide technical support for \LaTeX{} or any other software package. To avoid problems, please keep your paper simple, and do not incorporate complicated macros and style files.

% \begin{quote}
% \noindent anonymous Press\\
% 1101 Pennsylvania Ave, NW Suite 300\\
% Washington, DC 20004 USA\\
% \textit{Telephone:} 1-202-360-4062\\
% \textit{E-mail:} See the submission instructions for your particular conference or event.
% \end{quote}

% \section{Additional Resources}
% \LaTeX{} is a difficult program to master. If you've used that software, and this document didn't help or some items were not explained clearly, we recommend you read Michael Shell's excellent document (testflow doc.txt V1.0a 2002/08/13) about obtaining correct PS/PDF output on \LaTeX{} systems. (It was written for another purpose, but it has general application as well). It is available at www.ctan.org in the tex-archive.

% \appendix
% \section{Reference Examples}
% \label{sec:reference_examples}

% \nobibliography*
% Formatted bibliographies should look like the following examples. You should use BibTeX to generate the references. Missing fields are unacceptable when compiling references, and usually indicate that you are using the wrong type of entry (BibTeX class).

% \paragraph{Book with multiple authors~\nocite{em:86}} Use the \texttt{@book} class.\\[.2em]
% \bibentry{em:86}.

% \paragraph{Journal and magazine articles~\nocite{r:80, hcr:83}} Use the \texttt{@article} class.\\[.2em]
% \bibentry{r:80}.\\[.2em]
% \bibentry{hcr:83}.

% \paragraph{Proceedings paper published by a society, press or publisher~\nocite{c:83, c:84}} Use the \texttt{@inproceedings} class. You may abbreviate the \emph{booktitle} field, but make sure that the conference edition is clear.\\[.2em]
% \bibentry{c:84}.\\[.2em]
% \bibentry{c:83}.

% \paragraph{University technical report~\nocite{r:86}} Use the \texttt{@techreport} class.\\[.2em]
% \bibentry{r:86}.

% \paragraph{Dissertation or thesis~\nocite{c:79}} Use the \texttt{@phdthesis} class.\\[.2em]
% \bibentry{c:79}.

% \paragraph{Forthcoming publication~\nocite{c:21}} Use the \texttt{@misc} class with a \texttt{note="Forthcoming"} annotation.
% \begin{quote}
% \begin{footnotesize}
% \begin{verbatim}
% @misc(key,
%   [...]
%   note="Forthcoming",
% )
% \end{verbatim}
% \end{footnotesize}
% \end{quote}
% \bibentry{c:21}.

% \paragraph{ArXiv paper~\nocite{c:22}} Fetch the BibTeX entry from the "Export Bibtex Citation" link in the arXiv website. Notice it uses the \texttt{@misc} class instead of the \texttt{@article} one, and that it includes the \texttt{eprint} and \texttt{archivePrefix} keys.
% \begin{quote}
% \begin{footnotesize}
% \begin{verbatim}
% @misc(key,
%   [...]
%   eprint="xxxx.yyyy",
%   archivePrefix="arXiv",
% )
% \end{verbatim}
% \end{footnotesize}
% \end{quote}
% \bibentry{c:22}.

% \paragraph{Website or online resource~\nocite{c:23}} Use the \texttt{@misc} class. Add the url in the \texttt{howpublished} field and the date of access in the \texttt{note} field:
% \begin{quote}
% \begin{footnotesize}
% \begin{verbatim}
% @misc(key,
%   [...]
%   howpublished="\url{http://...}",
%   note="Accessed: YYYY-mm-dd",
% )
% \end{verbatim}
% \end{footnotesize}
% \end{quote}
% \bibentry{c:23}.

% \vspace{.2em}
% For the most up to date version of the anonymous reference style, please consult the \textit{AI Magazine} Author Guidelines at \url{https://anonymous.org/ojs/index.php/aimagazine/about/submissions#authorGuidelines}

% \section{Acknowledgments}
% anonymous is especially grateful to Peter Patel Schneider for his work in implementing the original anonymous.sty file, liberally using the ideas of other style hackers, including Barbara Beeton. We also acknowledge with thanks the work of George Ferguson for his guide to using the style and BibTeX files --- which has been incorporated into this document --- and Hans Guesgen, who provided several timely modifications, as well as the many others who have, from time to time, sent in suggestions on improvements to the anonymous style. We are especially grateful to Francisco Cruz, Marc Pujol-Gonzalez, and Mico Loretan for the improvements to the Bib\TeX{} and \LaTeX{} files made in 2020.

% The preparation of the \LaTeX{} and Bib\TeX{} files that implement these instructions was supported by Schlumberger Palo Alto Research, AT\&T Bell Laboratories, Morgan Kaufmann Publishers, The Live Oak Press, LLC, and anonymous Press. Bibliography style changes were added by Sunil Issar. \verb+\+pubnote was added by J. Scott Penberthy. George Ferguson added support for printing the anonymous copyright slug. Additional changes to anonymous25.sty and anonymous25.bst have been made by Francisco Cruz and Marc Pujol-Gonzalez.

% \bigskip
% \noindent Thank you for reading these instructions carefully. We look forward to receiving your electronic files!
% \fi
% \bibliographystyle{abbrv}
\bibliographystyle{ACM-Reference-Format}
\bibliography{acmwww}
\newpage
\appendix
% \section{Appendix: xxx}
\section{Appendix: Experiment Details}
\subsection{Datasets Statistics}
\label{app:dataset}
\begin{table}[!htbp]
\centering
\setlength{\tabcolsep}{3.2pt}
\begin{tabular}{l|c|c|c}
\toprule
         & \textbf{Arts}    & \textbf{Games}   & \textbf{Instruments} \\ \midrule
\# Users & 55970   & 55145   & 27404       \\
\# Items & 22612   & 17287   & 10450       \\
Avg. len & 8.80    & 9.01    & 8.41        \\
Sparsity & 99.96\% & 99.95\% & 99.92\%     \\ \bottomrule
\end{tabular}
\caption{Statistics of the 3 pre-processed datasets. Avg. len represents the average length of interacted items per user.}
\label{tab:dataset}
\end{table}
The processed data statistics are summarized in Table~\ref{tab:dataset}.
Note that ``Arts'', ``Games'' and ``Instruments'' represent the abbreviations of ``Arts, Crafts and Sewing'', ``Video Games'' and ``Musical Instruments'' respectively in the Amazon dataset (Amazon Review Data (2018)), where all data include reviews in the range May 1996 - Oct 2018~\cite{ni2019justifying}.

\subsection{Baselines Details}
\label{app:details:Baselines}
We adopt three types of representative sequential recommendation methods as baselines to validate the effectiveness of our \texttt{MoRE}:
% We adopt the following representative SeqRec models as baselines for comparison with our \texttt{MoRE}:

Traditional deep learning recommendation models include:
\begin{itemize}
\item\textbf{Caser}~\cite{tang2018personalized} is a CNN-based method that models user-item interactions as sequences to capture both local and global patterns.
    \item \textbf{GRU4Rec}~\cite{hidasi2015session} is an RNN-based SeqRec model with GRU modeling the user behavior sequences.
    \item \textbf{BERT4Rec}~\cite{sun2019bert4rec} adopts a bidirectional Transformer model and incorporates a masked prediction approach to capture the patterns in item sequences. 
    \item \textbf{SASRec}~\cite{kang2018self} exploits a unidirectional Transformer-based neural network to model the item sequences and predict the next item.
    \item \textbf{FDSA}~\cite{zhang2019feature}  models both item-level and feature-level transition patterns through a dual self-attention mechanism. 
\end{itemize}
Training-free LLM-based methods, i.e.,
the prompt-based recommendation methods include:
\begin{itemize}
\item\textbf{LLM4RS}~\cite{dai2023uncovering} investigates the potential of LLMs in enhancing recommendation capabilities by aligning it with traditional information retrieval (IR) ranking techniques, specifically point-wise, pair-wise, and list-wise ranking. 
    \item \textbf{LLMRank}~\cite{hou2024large} leverages LLMs for zero-shot ranking in recommendation tasks, addressing challenges related to interaction order and bias through specialized prompting techniques.
\end{itemize}
Training-required LLM-based methods, i.e., fine-tuning and reflection-based recommendation methods include:
\begin{itemize}
    \item \textbf{LC-Rec}\footnote{To ensure a fair comparison, we ensured that each model's recommendation process for each user was based on the same item candidate set of size 50. However, since LC-Rec's training is based on the full item set as the shared candidate set, it is challenging to guarantee that the model does not output items outside the size 50 candidate set for a user solely through the prompt. To address this, we implemented output constraints for the generation process of LC-Rec, ensuring that it outputs only the permitted 50 items for each user}~\cite{zheng2024adapting} is  a fine-tuning LLMREC method that incorporates collaborative filtering information by expanding the vocabulary space with special token embeddings. It is currently the state-of-the-art method for LLMREC in the full-candidate SeqRec setting.
    \item \textbf{BinLLM}\footnote{BinLLM introduces collaborative filtering knowledge to LLMs from the perspective of input text. However, it can only predict the relationship between one user and one item at a time, necessitating multiple inferences to provide recommendations for a user. To ensure a fair comparison, we modified the format of its prompt and reproduced it to make it output a list.}~\cite{zhang2024text} is a fine-tuning LLMREC method that incorporates collaborative filtering information by injecting user and item embeddings as binary text sequences into the LLM's input, without modifying the model's vocabulary space. It is currently the state-of-the-art method for LLMREC conditioned on the given user-item pair.
    \item  \textbf{Re2LLM}~\cite{wang2024re2llm} is a reflection-based LLMREC method. It first constructs a reflection knowledge base (KB) with domain knowledge, and then retrieves suitable text in the fixed KB to insert into the LLM's input, adapting the LLM to session-based recommendation.
\end{itemize}



% \textbf{SASRec}~\cite{kang2018self} exploits a unidirectional Transformer-based neural network to model the item sequences and predict the next item. 
% \textbf{FDSA}~\cite{zhang2019feature}  models both item-level and feature-level transition patterns through a dual self-attention mechanism. \textbf{LLM4RS}~\cite{dai2023uncovering} investigates the potential of LLMs in enhancing recommendation capabilities by aligning it with traditional information retrieval (IR) ranking techniques, specifically point-wise, pair-wise, and list-wise ranking. 
% \textbf{LLMRank}~\cite{hou2024large} leverages LLMs for zero-shot ranking in recommendation tasks, addressing challenges related to interaction order and bias through specialized prompting techniques.
% \textbf{LC-Rec}\footnote{To ensure a fair comparison, we ensured that each model's recommendation process for each user was based on the same item candidate set of size 50. However, since LC-Rec's training is based on the full item set as the shared candidate set, it is challenging to guarantee that the model does not output items outside the size 50 candidate set for a user solely through the prompt. To address this, we implemented output constraints for the generation process of LC-Rec, ensuring that it outputs only the permitted 50 items for each user}~\cite{zheng2024adapting} is  a fine-tuning LLMREC method that incorporates collaborative filtering information by expanding the vocabulary space with special token embeddings. It is currently the state-of-the-art method for LLMREC in the full-candidate SeqRec setting.
% is a large language model recommendation method that incorporates collaborative filtering information. LC-Rec expands the vocabulary space of the large language model backbone by introducing learnable item IDs and special token embeddings for training. LC-Rec designs various recommendation question-answering tasks involving item IDs, enabling the model to understand the relationship between special tokens and text tokens but incurring significant training costs. It is currently the state-of-the-art method for large model recommendations in the full candidate set setting.
% \textbf{BinLLM}\footnote{BinLLM introduces collaborative filtering knowledge to LLMs from the perspective of input text. However, it can only predict the relationship between one user and one item at a time, necessitating multiple inferences to provide recommendations for a user. To ensure a fair comparison, we modified the format of its prompt and reproduced it to make it output a list.}~\cite{zhang2024text} is a fine-tuning LLMREC method that incorporates collaborative filtering information by injecting user and item embeddings as binary text sequences into the LLM's input, without modifying the model's vocabulary space. It is currently the state-of-the-art method for LLMREC conditioned on the given user-item pair.
% is a LLMREC method that incorporates collaborative filtering information without modifying the vocabulary space. Researchers of BinLLM believe that altering the model's vocabulary space would compromise the original generation capabilities of LLMs, leading to a loss in performance. They propose a fine-tuning method that injects user and item embeddings as binary text sequences into the LLM's input, attempting to leverage the implicit "logical AND" capability of the LLM to understand and capture the relationship between the given user and the target item.
 % \textbf{Re2LLM}~\cite{wang2024re2llm} is a reflection-based LLMREC method. It first constructs a reflection knowledge base (KB) with domain knowledge, and then retrieves suitable text in the fixed KB to insert into the LLM's input, adapting the LLM to session-based recommendation.


\begin{figure*}[t]
    %\centering
    \setlength{\belowcaptionskip}{-5pt}
    \begin{subfigure}[h]{0.3\textwidth}
        \centering
    \includegraphics[width=\textwidth]{fig_updated/Amazon_Games_EP_reflect_iteration_trend_v7_no_title.pdf}
    %\vspace{3.2ex}
        \caption{Explicit Preference (EP) Reflect}
        \label{fig:Games:explicit:iter}
    \end{subfigure}
    \hfill
    \begin{subfigure}[h]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig_updated/Amazon_Games_IP_reflect_iteration_trend_v8_no_title.pdf}
        \caption{Implicit Preference (IP) Reflect}
        \label{fig:Games:implicit:iter}
    \end{subfigure}
    \hfill
    \begin{subfigure}[h]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{fig_updated/Amazon_Games_CF_reflect_iteration_trend_v8_no_title.pdf}
        \caption{Collaborative Filtering (CF) Reflect}
        \label{fig:Games:CF:iter}
    \end{subfigure}
    % \centering
    % \includegraphics[width=0.45\textwidth]{LaTeX/fig/Amazon_Arts_cluster_explicit_reflect_iteration_trend_v1.pdf}
    \caption{
    Impact of iteration on reflections for explicit preferences, implicit preferences, and collaborative filtering information on recommendation performance. The experiments are conducted on the Amazon Games dataset, utilizing an individual-level refining strategy.
    }
    % %\label{fig:diff:IL:IBCB}
    \label{fig:perspective:iter:comp}

\end{figure*}

\subsection{Implementation Details}
\label{app:details:imp}
%We use LLaMa-3-8B-Instruct~\cite{dubey2024llama} as the LLM backbone for our \texttt{MoRE} and LLM-based baselines.

Considering the cost and efficiency of LLMs, we perform random sampling from three datasets respectively. The principle for sampling users is to exclude those with excessively long interaction sequences before performing random sampling. For each dataset, we sample 1,000 users. Note that items are kept the same as the pre-processed datasets.

For a fair comparison, we use RecBole~\cite{zhao2021recbole} to implement all traditional SeqRec baselines (e.g. SASRec). All these baselines are optimized with Adam optimizer, and we use the grid search method to find the best hyper-parameter for each of them. Grid search space was set as: \textit{embedding size} : \{32, 64, 128\}, \textit{learning rate} : \{$1e^{-2}, 1e^{-3},1e^{-4}$\} and \textit{batch size} : \{1024, 2048, 4096\}. For LLMREC baselines that need training, we follow their origin setting and make proper adaption to our datasets. All experiments are run on a 4$\times$A800-PCIE-80GB GPUs server.

For our \texttt{MoRE} method, we train a DMF~\cite{xue2017deep} model as the source of CF Reflection Expert's CF score (Sec.~\ref{sec:multi:perspective}). The embedding size of this DMF model is 64 for both users and items. This DMF model is also used to implement the user clustering mentioned in the Refining process in Sec.~\ref{sec:meta:main}. DMF model provides embedding vectors for users in the three datasets, and these embeddings are used to cluster the users in each dataset. We define 20 clusters for each dataset, with the cluster ID being an integer in $[0, 19]$, inclusive. For the Iteration process in Sec.~\ref{sec:meta:main}, we set the total iteration to 15, and impacts of Refining and Iteration can be found in Sec.~\ref{sec:exp:ri}.

\subsection{Impact of Iteration on Different Perspective Reflections on the Amazon Games Dataset}
\label{app:perspect:details}


% Additionally, we also compared the extent to which the refining and iteration improve the reflections on explicit preferences, implicit preferences, and CF information. The experimental results are presented in Appendix A4. 

In Sec.~\ref{exp:refine}, using LLM reflections on explicit user preferences as an example, we conducted experiments that demonstrated the effectiveness of refining strategies in enhancing reflection quality and improving recommendations. 

In this section, we explore the extent to which the iteration strategy improves the quality of reflections on explicit preferences, implicit preferences, and collaborative filtering information.
As can be seen from Fig.~\ref{fig:perspective:iter:comp}, we have the following three observations.

(1) In terms of the explicit and implicit user preferences, applying the iteration strategies improve the corresponding reflections. The results further verify the effectiveness of our reflection iteration strategy.

(2) Applying iteration strategies to reflections on explicit preferences leads to greater improvements in recommendation performance compared to applying the same strategies to reflections on implicit preferences.
We attribute these differences to the reasoning capabilities of the LLM. 
It is because understanding explicit user preferences is relatively easy for LLMs, as item titles directly reflect user preferences—such as when two products have highly relevant titles. On the other hand, implicit preferences are conveyed through product attributes, which poses greater challenges for LLMs to reason.

(3) The improvement in the CF reflection through iteration strategies is not significant and shows noticeable fluctuations.
We believe that even though we circumvent the issue of CF mathematical computations by introducing a tool model for the LLM, numerical comparisons still remain a limitation for the LLM. 

% We believe this is because we represent CF information as CF scores. In LLMs, reasoning abilities based purely on text are stronger than those involving mathematical reasoning.

In short, the EP and IP reflections are more suitable for the refining and iteration than the CF reflections.


% Based on the experimental results, we recommend focusing reflections on explicit user preferences in practice to enhance LLM-based recommendations.


% we find that recommendation performance of different perspectives on Amazon-Games gradually improves and achieves each summit in different iteration time, conveying the effectiveness of the iterations.


\subsection{Case Study}
\label{app:details:case}
In Sec.~\ref{sec:exp:selection}, we conduct ablation studies to quantitatively verify the effectiveness of our reflection selection. In this section, we further validate it qualitatively through a case study. We illustrate the recommendation performances using reflections generated by \texttt{MoRE} and other strategies, shown in the green and brown boxes on the next page.

% We also discuss \texttt{MoRE}'s recommendation performance through a simple case shown in this part (detailed case text can be found in the next page) to check \texttt{MoRE}'s practicability and suitability. 
The case in the brown box illustrates how the original LLMREC, without reflections, failed to hit the recommendation target. Meanwhile, among the various reflection selection methods, the Greedy strategy, which selects reflections based on their performance on the validation set, chooses the EP perspective, ultimately hitting the target at the 7-th position in the recommendation sequence. The Random strategy, on the other hand, randomly selects the IP perspective, which did not hit the recommendation target.

As shown in the green box, \texttt{MoRE}, with the help of the selector, ultimately chooses the CF perspective, hitting the target at the 1-st position in the recommendation sequence. In this case, we observe that the user's interaction history shows a clear preference for console and action games, with a specific but subtle interest in purchasing items related to console game brands. This preference was not correctly emphasized in the reflections generated from the EP and IP perspectives. Specifically, the IP reflection 
% recognized the user's interest in certain brands but 
focuses too much on past preferences for the same brand (e.g., Nintendo games), overlooking potential shifts in the user's future brand interests. In contrast, based on the Nintendo brand and action games, the CF reflection uses CF information to infer that the user might be interested in PlayStation action games. This approach accurately captured the user's needs, leading to a correct recommendation. 

In short, in this case study, \texttt{MoRE} selects the most appropriate reflective perspective, which greatly assisted the recommendation process.


Moving forward, we believe that employing a reflection mechanism can effectively bridge the semantic gap between LLMs and CF by allowing LLMs to leverage simple score comparisons rather than struggling with the understanding of embeddings.
Invoking a straightforward model as a tool to obtain CF scores circumvents the challenge of LLMs understanding CF semantics, thereby endowing LLMs with CF knowledge. Moreover, utilizing reflection along with calling upon simple models offers a cost-effective solution to mitigate various issues LLMs face when adapting to and understanding specialized domains where they might otherwise struggle.

% In summary, within the scope of this case study, \texttt{MoRE} selects the best reflection perspective, significantly aiding the recommendation process.

% The case in the brown box describes that original LLMREC without reflection failed to hit the recommendation target. Among the various reflection selection methods, the method using the Greedy strategy, based on the performance of various reflections on the validation set, choose the EP perspective, ultimately hitting the target at the 7-th position in the recommendation sequence. 
% The Random strategy, on the other hand, randomly select the IP perspective, which did not hit the recommendation target. \texttt{MoRE}, with the help of the selector, ultimately choose the CF perspective and was able to hit the target at the 1-st position in the recommendation sequence. In this case, we can find that from the user's interaction history, there is a clear preference for console games and action games, particularly an unobvious demand for purchasing items related to console games, which is not correctly emphasized in the analysis of both EP and IP perspective reflections. Specifically, the IP reflection had already observed the user's interest in certain brands but was overly focused on past preferences of the same brand (e.g. the Nintendo games) and overlooked shifts in the user's future brand interests. In contrast, the CF reflection leveraged the user's previous behavior of purchasing Nintendo action games and used collaborative filtering information to infer that the user might be interested in Play Station action games, thus accurately capturing the user's needs and making the correct judgment and recommendation reflection. In this case, our \texttt{MoRE} chose the best perspective of reflection and helped the user most in recommendation, validating our motivation and effectiveness of \texttt{MoRE}. 

\begin{mybox_case}{Case Study: \emph{\texttt{MoRE}'s Reflection Selection}}
\vspace{0pt}
{\textit{\textbf{Prompt}: I've purchased the following products in the past in order: \{Ben 10 Omniverse 2 - Nintendo Wii U;...\}. And after last previous recommendation (maybe a failed trial), you give the following reflects:\{\color{blue}$Ref_i$\color{black}\}. Now there are {\color{blue}{$|\mathcal{C}_u|$}} candidate products that I can consider to purchase next:\{\color{blue}$\mathcal{C}_u$\color{black}\}.Please rank these {\color{blue}{$|\mathcal{C}_u|$}} products by measuring the possibilities that I would like to purchase next most, according to the given purchasing records and reflects. Please think step by step. Please show me your top 10 ranking results with order numbers. Split your output with line break. You MUST rank the given candidates. You can not generate candidates that are not in the given candidate list.% Based on these interactions, recommend a movie for me to watch next from a candidate set: \{\color{blue}$\mathcal{C}$\color{black}\}. Please recommend from the candidate set. List the top 10 recommendations in numbered bullet points. Hint: \{\color{blue}$h$\color{black}\}.
% \newline 
% \textbf{Answer by recommendation w/o reflects}, where \color{blue} $Ref$ \color{black} = `':
% \newline  ``Final Fantasy Legend", ``2. Assassin's Creed Liberation HD [Download]", ``3. Spinido iPhone 7 Plus Desk Stand Holder Compatible with All Smartphone with Cases- Gold", ``4. Phineas and Ferb Ride Again - Nintendo DS", ``5. Shadow Warrior", ``6. Saints Row IV: National Treasure - Xbox 360", ``7. Cabela's African Adventures - Wii", ``8. The Sims 2: Double Deluxe - PC", ``9. Disney INFINITY (2.0 Edition) [Download]", ``10. Metal Gear Solid HD Collection"
\newline 
\textbf{Answer by \texttt{MoRE} perspective selection}, where \color{myboxcolor!75!black}{\textbf{selected reflection (CF reflection)}} \color{blue} $Ref_i = Ref_\mathrm{CF}$ \color{black} = `\textbf{\color{myboxcolor!75!black}{PREFERENCE: The user tends to prefer gaming-related items with high CF scores, particularly those from PlayStation 4 and Xbox 360 platforms, as well as items with high CF scores from previous interactions. ANALYSIS: Although the actor's previous recommendations are diverse, some items such as \{HORI Fighting Commander 4 Controller for PlayStation 4/3, ...\}, was not included in the actor's recommendations. This suggests that the actor may have overlooked strong CF signals in favor of more diverse recommendations. SUGGESTIONS: Prioritize gaming-related items with high CF scores, especially those from PlayStation 4 and Xbox 360 platforms, as well as items with high CF scores from previous interactions. Consider including items with CF scores above 0.5, such as \{...\}, to improve the accuracy of the recommendations.}}':
\newline \textbf{{1. Street Fighter V - PlayStation 4 Standard Edition (CF score: 0.83)}}, 2. Mass Effect 2 - PC (CF score: 0.78), 3. Assassin's Creed Liberation HD [Download] (CF score: 0.76), 4. Metal Gear Solid HD Collection (CF score: 0.75), 5. Call of Duty: Advanced Warfare Atlas Limited Edition - Xbox One (CF score: 0.74), 6. Spec Ops: The Line - Playstation 3 (CF score: 0.73), 7. Cities: Skylines [Online Game Code] (CF score: 0.72), 8. Final Fantasy Crystal Chronicles: Echoes of Time - Nintendo Wii (CF score: 0.71), 9. Fatal Fury: Mark of The Wolves (CF score: 0.7), 10. .hack, Part 3: Outbreak (CF score: 0.69)
% \newline 
% \textbf{Answer by Random perspective selector}, where \color{myboxcolor2!75!black}{\textbf{random hint}} \color{blue} $Ref$ \color{black} = `\textbf{\color{myboxcolor2!75!black}{Pay attention to actors who appear in multiple movies from the watched list and consider other films featuring these actors}}':
% \newline 1. The Day After Tomorrow; 2. Taken; 3. The Bourne Identity; 4. Last Man Standing; 5. The Last Castle; 6. The Wrestler; 7. Redbelt; 8. The Stepfather; 9. Kiss of the Dragon; 10. Courage Under Fire
% \newline 
% \textbf{Answer by \texttt{MoRE}}, where \color{myboxcolor2!75!black}{\textbf{random hint}} \color{blue} $Ref$ \color{black} = `\textbf{\color{myboxcolor2!75!black}{Pay attention to actors who appear in multiple movies from the watched list and consider other films featuring these actors}}':
% \newline 1. The Day After Tomorrow; 2. Taken; 3. The Bourne Identity; 4. Last Man Standing; 5. The Last Castle; 6. The Wrestler; 7. Redbelt; 8. The Stepfather; 9. Kiss of the Dragon; 10. Courage Under Fire
}}
\vspace{0pt}
\end{mybox_case} 
\vspace{0pt}
\begin{mybox_random}{Case Study: \emph{Other Reflection Selectors}}
\vspace{0pt}
{\textit{\textbf{Prompt}: (same form as former prompt)%I've purchased the following products in the past in order: \{Ben 10 Omniverse 2 - Nintendo Wii U;...\}. And after last previous recommendation (maybe a failed trial), you give the following reflects:\{\color{blue}$Ref$\color{black}\}. Now there are 50 candidate products that I can consider to purchase next:\{\color{blue}$\mathcal{C}$\color{black}\}.Please rank these 50 products by measuring the possibilities that I would like to purchase next most, according to the given purchasing records and reflects. Please think step by step. Please show me your top 10 ranking results with order numbers. Split your output with line break. You MUST rank the given candidates. You can not generate candidates that are not in the given candidate list.Based on these interactions, recommend a movie for me to watch next from a candidate set: \{\color{blue}$\mathcal{C}$\color{black}\}. Please recommend from the candidate set. List the top 10 recommendations in numbered bullet points. Hint: \{\color{blue}$h$\color{black}\}.
% \newline 
% \textbf{Answer by recommendation w/o reflects}, where \color{blue} $Ref$ \color{black} = `':
% \newline  ``Final Fantasy Legend", ``2. Assassin's Creed Liberation HD [Download]", ``3. Spinido iPhone 7 Plus Desk Stand Holder Compatible with All Smartphone with Cases- Gold", ``4. Phineas and Ferb Ride Again - Nintendo DS", ``5. Shadow Warrior", ``6. Saints Row IV: National Treasure - Xbox 360", ``7. Cabela's African Adventures - Wii", ``8. The Sims 2: Double Deluxe - PC", ``9. Disney INFINITY (2.0 Edition) [Download]", ``10. Metal Gear Solid HD Collection"
\newline 
\textbf{Answer by recommendation w/o reflection}, where \color{myboxcolor2!75!black}{\textbf{selected reflection (EP reflection)}} \color{blue} $Ref_i$ \color{black} = `':
\newline  (\textbf{Didn't hit at any position}) 1. Final Fantasy Legend, 2. Assassin's Creed Liberation HD [Download], 3. Spinido iPhone 7 Plus Desk Stand Holder Compatible with All Smartphone with Cases- Gold, 4. Phineas and Ferb Ride Again - Nintendo DS, 5. Shadow Warrior, 6. Saints Row IV: National Treasure - Xbox 360, 7. Cabela's African Adventures - Wii, 8. The Sims 2: Double Deluxe - PC, 9. Disney INFINITY (2.0 Edition) [Download], 10. Metal Gear Solid HD Collection 
\newline 
\textbf{Answer by Greedy perspective selector}, where \color{myboxcolor2!75!black}{\textbf{selected reflection (EP reflection)}} \color{blue} $Ref_i = Ref_\mathrm{EP}$ \color{black} = `\textbf{\color{myboxcolor2!75!black}{ PREFERENCE: The user has shown a strong interest in fighting games, particularly those with a classic or retro feel, as well as console-based games. ANALYSIS: The actor's recommendations did not fully capitalize on the user's preferences for fighting games and console-based games. The recommended games did not show a strong focus on gameplay and mechanics, and did not prioritize the most engaging and popular titles in the fighting game genre. SUGGESTIONS: Prioritize recommending fighting games, particularly those with a classic or retro feel, and consider suggesting console-based games that cater to the user's interest in gameplay and mechanics.}}':
\newline  1. Fatal Fury: Mark of The Wolves, 2. Final Fantasy Crystal Chronicles: Echoes of Time - Nintendo Wii, 3. .hack, Part 3: Outbreak, 4. Capcom Classics Collection, 5. Bad News Baseball - Nintendo NES, 6. Teenage Mutant Ninja Turtles IV: Turtles in Time, \textbf{7. Street Fighter V - PlayStation 4 Standard Edition}, 8. Metal Gear Solid HD Collection, 9. Final Fantasy Legend, 10. Urban Champion
\newline 
\textbf{Answer by Random perspective selector}, where \color{myboxcolor2!75!black}{\textbf{selected reflection (IP reflection)}} \color{blue} $Ref_i = Ref_\mathrm{IP}$ \color{black} = `\textbf{\color{myboxcolor2!75!black}{ PREFERENCE: Based on the user's interaction history, it appears that they have a strong preference for games from Nintendo and PlayStation platforms, particularly games from the Wii and Wii U console platforms. The user also shows interest in games with multiplayer features, as evidenced by the inclusion of games like \{...\}. ANALYSIS: To improve the actor's recommendations, I suggest prioritizing games from Nintendo and PlayStation platforms, particularly games from the Wii and Wii U console platforms. The actor should also focus on games with multiplayer features, as this seems to be an area of interest for the user. Additionally, consider recommending games that offer unique gameplay mechanics, such as \{...\}, which the user has interacted with previously.}}':
\newline (\textbf{Didn't hit at any position}) 1. Final Fantasy Crystal Chronicles: Echoes of Time - Nintendo Wii, 2. Mike Tyson's Punch-Out!! - Nintendo NES, 3. Bad News Baseball - Nintendo NES, 4. Urban Champion - Nintendo NES, 5. Super Mario 64 DS - Nintendo DS, 6. Moshi Monsters - Nintendo DS, 7. LEGO Pirates of the Caribbean - Nintendo DS, 8. Phineas and Ferb Ride Again - Nintendo DS, 9. Cabela's African Adventures - Wii, 10. Disney Magical World - Nintendo 3DS
% \newline 
% \textbf{Answer by Random perspective selector}, where \color{myboxcolor2!75!black}{\textbf{random hint}} \color{blue} $Ref$ \color{black} = `\textbf{\color{myboxcolor2!75!black}{Pay attention to actors who appear in multiple movies from the watched list and consider other films featuring these actors}}':
% \newline 1. The Day After Tomorrow; 2. Taken; 3. The Bourne Identity; 4. Last Man Standing; 5. The Last Castle; 6. The Wrestler; 7. Redbelt; 8. The Stepfather; 9. Kiss of the Dragon; 10. Courage Under Fire
% \newline 
% \textbf{Answer by \texttt{MoRE}}, where \color{myboxcolor2!75!black}{\textbf{random hint}} \color{blue} $Ref$ \color{black} = `\textbf{\color{myboxcolor2!75!black}{Pay attention to actors who appear in multiple movies from the watched list and consider other films featuring these actors}}':
% \newline 1. The Day After Tomorrow; 2. Taken; 3. The Bourne Identity; 4. Last Man Standing; 5. The Last Castle; 6. The Wrestler; 7. Redbelt; 8. The Stepfather; 9. Kiss of the Dragon; 10. Courage Under Fire
}}
\vspace{-0pt}
\end{mybox_random} 
\newpage
\section{Appendix: Prompt design}
\subsection{Base Recommendation Prompt}
\label{app:details:base}
We provide the base recommendation prompt as follows.
\newtcolorbox{mybox_base}[1]{
    colback=white,
    colframe=black,
    fonttitle=\bfseries,
    title=#1
}
\begin{mybox_base}{Base recommendation prompt $P$}
{\textit{I've purchased the following products in the past in order:\{{\color{blue}{$\mathcal{S}_u$}}\}. Now there are {\color{blue}{$|\mathcal{C}_u|$}} candidate products that I can consider to purchase next: \{{\color{blue}{$\mathcal{C}_u$}}\}.}\\
\newline
\textit{ Please rank these {\color{blue}{$|\mathcal{C}_u|$}} products by measuring the possibilities that I would like to purchase next most, according to the given purchasing records. Please think step by step. Please show me your top 10 ranking results with order numbers. Split your output with line break. You MUST rank the given candidates. You can not generate candidates that are not in the given candidate list.}\\

% \textit{yyy}\\
% \textit{zzz}
}
\vspace{0pt}
\end{mybox_base}
where {\color{blue}{$\mathcal{S}_u$}} is user $u$'s previous interaction sequence in chronological order, {\color{blue}{$\mathcal{C}_u$}} is the candidate item set for user $u$, and {\color{blue}{$|\mathcal{C}_u|$}} is the candidate item set's size.
\subsection{Recommendation with reflection's prompt}
We provide the prompt of reflection-based recommendation as follows.
\newtcolorbox{mybox_ref}[1]{
    colback=white,
    colframe=green!75!black,
    fonttitle=\bfseries,
    title=#1
}
\begin{mybox_ref}{Recommendation prompt with reflection $P_\mathrm{REF}$}
{\textit{I've purchased the following products in the past in order:\{{\color{blue}{$\mathcal{S}_u$}}\}.}\\
\newline
\textit{And after last previous recommendation (maybe a failed trial), you give the following reflects: \{{\color{blue}{$Ref_i$}}\}.}\\
\newline
\textit{Now there are {\color{blue}{$|\mathcal{C}_u|$}} candidate products that I can consider to purchase next: \{{\color{blue}{$\mathcal{C}_u$}}\}. Please rank these {\color{blue}{$|\mathcal{C}_u|$}} products by measuring the possibilities that I would like to purchase next most, according to the given purchasing records. Please think step by step. Please show me your top 10 ranking results with order numbers. Split your output with line break. You MUST rank the given candidates. You can not generate candidates that are not in the given candidate list.}\\
}
\vspace{0pt}
\end{mybox_ref}
where {\color{blue}{$\mathcal{S}_u$}} is user $u$'s previous interaction sequence in chronological order, {\color{blue}{$\mathcal{C}_u$}} is the candidate item set for user $u$, and {\color{blue}{$|\mathcal{C}_u|$}} is the candidate item set's size. {\color{blue}{$Ref_i$}} is the text of reflection from a specific perspective, including explicit preference (EP) reflection $Ref_\mathrm{EP}$, implicit preference (IP) reflection $Ref_\mathrm{IP}$ and collaborative filtering (CF) reflection $Ref_\mathrm{CF}$.
\subsection{Explicit Preference (EP) Reflector’s Generation Prompt}
\label{app:details:EP}
In this section, we provide the detailed information about explicit preference (EP) reflector's generation prompt, including zero-shot (EP reflection prompt $P_\mathrm{EP}$) and few-shot (EP reflection prompt $P_\mathrm{EP}$: With demonstrations) version. Here, we first show the zero-shot version, which is used for the beginning of the Refining and Iteration.
\newtcolorbox{mybox}[1]{
    colback=white,
    colframe=blue!75!black,
    fonttitle=\bfseries,
    title=#1
}
\begin{mybox}{EP reflection prompt $P_\mathrm{EP}$}
{\textit{You are an expert of giving reflections to the sequential recommender actor. The actor is a sequential recommender. It receives instructions and generates item recommendations based on user's historical interactions. As an expert, you should provide reflections on the actor's previous recommendations to help improve actor's next recommendations for this user.}\\
\newline
\textit{You need to take it step by step. Step 1: Output 1 or 2 sentences starting with 'PREFERENCE:'.By analyzing the user's interaction history based on text information such as \textbf{item titles} and categories with your knowledge. (paying more attention to later items in the history), you can predict the user preferences (e.g., trends, anomalies, interest). Step 2. Output 1 or 2 sentences starting with 'ANALYSIS:'. Then analyze the problems with the 10 items recommended by the actor based on user history and preferences. Step 3. Output 1 or 2 sentences starting with 'SUGGESTIONS:'. Finally provide suggestions for the actor to make next recommendations for this user (e.g. prioritize [specific aspect or feature]).}\\
\newline
\textit{Here are the actor's recommendations you need to reflect on now (Don't output any specific titles of items):}\\
\newline
\textit{Previous instruction:\{{\color{blue}{$P$}}\}}\\
\textit{Standard answer:\{{\color{blue}{$\hat{v}$}}\}}\\
\textit{Actor's recommendations:\{{\color{blue}{$\hat{\mathcal{O}}_u$}}\}}\\
\newline
\textit{Please provide your response based on Previous recommendations below:}\\
}
\vspace{0pt}
\end{mybox}
where {\color{blue}{$P$}} stands for the previous instruction, also known as the base recommendation prompt (see in App.~\ref{app:details:base}), which includes user's previous interaction sequence and candidate item set. All items are displayed with their item titles, which represents the explicit preference of user. {\color{blue}{$\hat{v}$}} is the standard answer of {\color{blue}{$P$}}, also known as the ground truth item which user will interacted with in the next time step. {\color{blue}{$\hat{\mathcal{O}}_u$}} is actor's recommendations, also known as the previous predicted item list including each item's title. The task of $P_\mathrm{EP}$ is to generate the EP reflection $Ref_\mathrm{EP}$ based on all information mentioned above, especially the item titles which conveys the explicit preference. 
Then, we display the few-shot version, which is used for bettering Refining and Iteration's performance by giving valuable demonstrations through specific strategies.
\vspace{0pt}
\begin{mybox}{EP reflection prompt $P_\mathrm{EP}$: With demonstrations}
{\textit{You are an expert of giving reflections to the sequential recommender actor ... Finally provide suggestions for the actor to make next recommendations for this user (e.g. prioritize [specific aspect or feature]).}\\
\newline
\textit{Here are some Examples:}\\
\textit{[Example 1 start]}\\
\textit{Previous instruction:\{{\color{blue}{I've purchased the following products in the past in order: \{Ancient Secrets: Quest for the Golden Key, ... , Big City Adventure: Tokyo [Download]\}. Now there are 50 candidate products that I can consider to purchase next: \{SADES 7.1 Surround Sound Pro ... White (SA903), The Jungle Book, ... , Left 4 Dead - Game of the Year Edition -Xbox 360\}. ...  Please show me your top 10 ranking results with order numbers. ... }}\}}\\
\textit{Standard answer:\{{\color{blue}{Jewel Quest Mysteries: The Oracle of Ur [Download]}}\}}\\
\textit{Actor's recommendations:\{{\color{blue}{[1. Dark Dimensions: Wax Beauty - PC, 2. Jewel Quest Mysteries: The Oracle of Ur [Download], ... , 10. Dungeon Keeper 2 (Jewel Case) - PC]}}\}}\\
\textit{Please provide your response based on Previous recommendations below:\{{\color{blue}{"PREFERENCE: The user's interest lies in games that involve puzzle-solving, adventure, and mystery, possibly with a focus on hidden object games, as they have interacted with similar games in the past. ANALYSIS: The actor's recommendations did not fully capture the user's preferences, instead suggesting a diverse mix of games across various platforms and genres. While the top 2 recommended items, Jewel Quest Mysteries: The Oracle of Ur [Download] and Dark Dimensions: Wax Beauty - PC, align with the user's preferences, the subsequent recommendations stray away from the user's interests. SUGGESTIONS: The actor should prioritize recommending games that fit the user's preferences for puzzle-solving, adventure, and mystery, such as hidden object games or casual puzzle games, and focus on titles that have a similar tone and atmosphere to the user's previously interacted items.}}\}}\\
\textit{[Example 1 end]}\\
\textit{[Example 2 start]}\\
\textit{...}\\
\textit{[Example 2 end]}\\
\newline
\textit{Here are the actor's recommendations you need to reflect on ... Please provide your response based on Previous recommendations below:}}
\vspace{0pt}
\end{mybox}
% \subsubsection{Without examples}
% \include{LaTeX/fig_updated/EP_prompt}
% \subsubsection{With demonstrations}

\subsection{Implicit Preference (IP) Reflector's Generation Prompt}
\label{app:details:IP}
In this section, we provide the detailed information about implicit preference (IP) reflector's generation prompt, including zero-shot (IP reflection prompt $P_\mathrm{IP}$) and few-shot (IP reflection prompt $P_\mathrm{IP}$: With demonstrations) version. Here, we first show the zero-shot version, which is used for the beginning of the Refining and Iteration.
% \include{LaTeX/fig_updated/IP_prompt}
% \subsubsection{Without examples}
\newtcolorbox{mybox2}[1]{
    colback=red!5!white,
    colframe=red!75!black,
    fonttitle=\bfseries,
    title=#1
}
\begin{mybox2}{IP reflection prompt $P_\mathrm{IP}$}
{\textit{You are an expert of giving reflections based on recommended \textbf{items' attributes} to the sequential recommender actor. The actor is a sequential recommender. It receives instructions and generates item recommendations based on user's historical interactions. As an expert, you should provide reflections based on the actor's previous recommendations, \textbf{especially items' attributes} to help improve actor's next recommendations for this user.}\\
\newline
\textit{You need to take it step by step. Step 1: Output 1 or 2 sentences starting with 'PREFERENCE:'. By analyzing the user's interaction history based on both text information such as items' titles and \textbf{items' attributes} with your knowledge. (paying more attention to LATER \textbf{items' attributes} in the history), you can predict the user preferences (e.g., trends, anomalies, interest). Step 2. Output 1 or 2 sentences starting with 'ANALYSIS:'. Then analyze the problems with the 10 items recommended by the actor based on user history and preferences. Step 3. Output 1 or 2 sentences starting with 'SUGGESTIONS:'. Finally provide suggestions for the actor to make next recommendations for this user (e.g. prioritize [specific aspect, feature or \textbf{attribute}]).}\\
\newline
\textit{Here are the actor's recommendations you need to reflect on now (Don't output any specific titles of items):}\\
\newline
\textit{Previous instruction and \textbf{items' attributes (item titles, categories and brands)}:\{{\color{blue}{$P$}}\}}\\
\textit{Standard answer:\{{\color{blue}{$\hat{v}$}}\}}\\
\textit{Actor's recommendations:\{{\color{blue}{$\hat{\mathcal{O}}_u$}}\}}\\
\newline
\textit{Please provide your response based on Previous recommendations below:}}
\vspace{0pt}
\end{mybox2}
where {\color{blue}{$P$}} stands for the previous instruction, which includes user's previous interaction sequence and candidate item set. Different from $P_\mathrm{EP}$, all items are displayed with their item titles and side information (including categories and brands), which represents the implicit preference of user. {\color{blue}{$\hat{v}$}} is the standard answer of {\color{blue}{$P$}}, also known as the ground truth item which user will interacted with in the next time step. {\color{blue}{$\hat{\mathcal{O}}_u$}} is actor's recommendations, also known as the previous predicted item list including each item's title. The task of $P_\mathrm{IP}$ is to generate the IP reflection $Ref_\mathrm{IP}$ based on all information mentioned above, especially the item's side information which conveys the implicit preference. 

Then, we display the few-shot version, which is used for bettering Refining and Iteration's performance by giving valuable demonstrations through specific strategies.

\vspace{0pt}
\begin{mybox2}{IP reflection prompt $P_\mathrm{IP}$: With demonstrations}
\small{\textit{You are an expert of giving reflections based on recommended \textbf{items' attributes} to the sequential recommender actor. ... Finally provide suggestions for the actor to make next recommendations for this user (e.g. prioritize [specific aspect or feature or \textbf{attribute}]).}\\
\newline
\textit{Here are some Examples:}\\
\textit{[Example 1 start]}\\
\textit{Previous instruction and \textbf{items' attributes (item titles, categories and brands)}:\{{\color{blue}{I've purchased the following products in the past in order: \{\{title : ``Red Heart Super Saver Yarn, Hunter Green'', categories : ``Yarn'', brand : ``Red Heart''\}, ... , \{title : ``Comfort Grip Crochet Hook 10/Pkg - Assorted Colors (one color per package)'', categories : ``Crochet Hooks'', brand : ``Kahoot''\}\}. Now there are 50 candidate products that I can consider to purchase next: \{\{title : ``Liquitex Professional Gloss Gel, Medium, 8 Ounce (5708)'', categories : ``Painting, Paints'', brand : ``Liquitex''\}\} ...  Please show me your top 10 ranking results with order numbers. ... }}\}}\\
\textit{Standard answer:\{{\color{blue}{Artgraf Watercolor Graphite In Tin}}\}}\\
\textit{Actor's recommendations:\{{\color{blue}{[1. Sizzix 660097 Thinlits Die Magical Butterfly by Pete Hughes, ... , 10. addi Knitting Needle Linos Straight 8 inch (20cm) Size US 06 (4.0mm)]}}\}}\\
\textit{Please provide your response based on Previous recommendations below: \{{\color{blue}{PREFERENCE: Based on the user's interaction history, it appears that the user is interested in crafting supplies, particularly related to painting, drawing, and beading. ANALYSIS: The actor's previous recommendations seem to be a mix of crafting supplies, but they lack a clear focus on the user's preferences for painting, drawing, and beading. The recommendations also do not prioritize the user's interaction history, which suggests a strong interest in crafting supplies. SUGGESTIONS: To improve the next recommendations, I suggest prioritizing items that are related to painting, drawing, and beading, as well as considering items that are similar to the user's previous interactions. The actor should also consider recommending products from brands that are well-known for their quality and relevance to the user's interests.}}\}}\\
\textit{[Example 1 end]}\\
\textit{[Example 2 start]}\\
\textit{...}\\
\textit{[Example 2 end]}\\
\newline
\textit{Here are the actor's recommendations you need to reflect on ... Please provide your response based on Previous recommendations below:}}
\vspace{0pt}
\end{mybox2}
Note that implicit preference (side information) are provided as the tuple ``\textit{\{title: ..., categories : ..., brand: ...\}}" in user's previous interacted sequence and candidate item set.
% \subsubsection{With demonstrations}
\subsection{Collaborative Filtering (CF) Reflector's Generation Prompt}
\label{app:details:CF}
In this section, we provide the detailed information about collaborative filtering (CF) reflector's generation prompt, including zero-shot (CF reflection prompt $P_\mathrm{CF}$) and few-shot (CF reflection prompt $P_\mathrm{CF}$: With demonstrations) version. Here, we first show the zero-shot version, which is used for the beginning of the Refining and Iteration.
% \subsubsection{Without examples}
\newtcolorbox{mybox3}[1]{
    colback=yellow!50!white,
    colframe=red!50!black,
    fonttitle=\bfseries,
    title=#1
}
\begin{mybox3}{CF reflection prompt $P_\mathrm{CF}$}
{\textit{You are an expert of giving reflections based on \textbf{user \& item's collaborative filtering scores} to the sequential recommender actor. The actor is a sequential recommender. It receives instructions and generates item recommendations based on user's historical interactions. Then, \textbf{a collaborative filtering model will provide scores based on current user and generated items.} As an expert, you should provide reflections on the actor's previous recommendations, especially \textbf{user-item collaborative filtering scores} to help improve actor's next recommendations for this user.}\\
\newline
\textit{You need to take it step by step. Step 1: Output 1 or 2 sentences starting with 'PREFERENCE:'. By analyzing the user's interaction history based on both text information such as item titles and categories, and \textbf{historical items' collaborative filtering scores} with your knowledge. (paying more attention to items with \textbf{HIGHER collaborative filtering scores} in the history),you can predict the user preferences (e.g., trends, anomalies, interest). Step 2. Output 1 or 2 sentences starting with 'ANALYSIS:'. Then analyze the problems with the 0 items recommended by the actor based on user history and preferences. Step 3. Output 1 or 2 sentences starting with 'SUGGESTIONS:'. Finally provide suggestions for the actor to make next recommendations for this user (e.g. prioritize [specific aspect or feature]).}\\
\newline
\textit{Here are the actor's recommendations you need to reflect on now (Don't output any specific titles of items):}\\
\newline
\textit{Previous instruction and \textbf{items' collaborative filtering scores} (\textbf{item titles \& CF scores}):\{{\color{blue}{$P$}}\}}\\
\textit{Standard answer:\{{\color{blue}{$\hat{v}$}}\}}\\
\textit{Actor's recommendations:\{{\color{blue}{$\hat{\mathcal{O}}_u$}}\}}\\
\newline
\textit{Please provide your response based on Previous recommendations below:}
}
\vspace{0pt}
\end{mybox3}
where {\color{blue}{$P$}} stands for the previous instruction, which includes user's previous interaction sequence and candidate item set. Different from $P_\mathrm{EP}$ and $P_\mathrm{IP}$, all items are displayed with their item titles and collaborative filtering scores (the CF score, provided by a CF model), which represents the collaborative filtering information of user and items. {\color{blue}{$\hat{v}$}} is the standard answer of {\color{blue}{$P$}}, also known as the ground truth item which user will interacted with in the next time step. {\color{blue}{$\hat{\mathcal{O}}_u$}} is actor's recommendations, also known as the previous predicted item list including each item's title. The task of $P_\mathrm{CF}$ is to generate the CF reflection $Ref_\mathrm{IP}$ based on all information mentioned above, especially the user-item collaborative filtering information. 
\vspace{0pt}
\begin{mybox3}{CF reflection prompt $P_\mathrm{CF}$: With demonstrations}
\small{\textit{You are an expert of giving reflections based on \textbf{user \& item's collaborative filtering scores} to the sequential recommender actor ... Finally provide suggestions for the actor to make next recommendations for this user (e.g. prioritize [specific aspect or feature]).}\\
\newline
\textit{Here are some Examples:}\\
\textit{[Example 1 start]}\\
\textit{Previous instruction and \textbf{items' collaborative filtering scores} (\textbf{item titles \& CF scores}):\{{\color{blue}{I've purchased the following products in the past in order: \{\{title : ``Red Heart Super Saver Yarn, Earth and Sky'', CF score : ``0.99847''\}, ... , \{title : ``Red Heart Super Saver Yarn, Light Sage'', CF score : ``0.99846''\}\}. Now there are 50 candidate products that I can consider to purchase next: \{\{title : ``Sizzix Bigz Die, 5.5 by 6-Inch, Picture Wheel'', CF score : ``0.5''\}, ... , \{title : ``RED HEART E302C.0312 Super Saver Jumbo Yarn, Black'', CF score : ``0.906811''\}\}.  ...  Please show me your top 10 ranking results with order numbers. ... }}\}}\\
\textit{Standard answer:\{{\color{blue}{RED HEART E302C.0312 Super Saver Jumbo Yarn, Black}}\}}\\
\textit{Actor's recommendations:\{{\color{blue}{[1. Red Heart Super Saver Yarn, Earth and Sky, ... , 10. Red Heart Super Saver Yarn, Melonberry Print]}}\}}\\
\textit{Please provide your response based on Previous recommendations below: \{{\color{blue}{PREFERENCE: Based on the user's interaction history, it appears that they tend to prefer yarn and fabric related items with high CF scores. The user's CF scores are highest for Red Heart yarn products, indicating a strong interest in these types of items. ANALYSIS: The actor's previous recommendations did not fully leverage the user's preferences, prioritizing items with lower CF scores. The recommended items, although diverse, did not seem to align with the user's interests in crafts, DIY projects, and art supplies. SUGGESTIONS: To improve the next set of recommendations, I suggest prioritizing items that align with the user's preferences and CF scores. The actor should consider recommending items related to crafts, DIY projects, and art supplies, such as yarn, fabric, and art materials.}}\}}\\
\textit{[Example 1 end]}\\
\textit{[Example 2 start]}\\
\textit{...}\\
\textit{[Example 2 end]}\\
\textit{Here are the actor's recommendations you need to reflect on ... Please provide your response based on Previous recommendations below:}}
\vspace{0pt}
\end{mybox3}
Note that collaborative filtering information are denoted as the tuple ``\textit{\{title: ..., CF score: ...\}}" in user's previous interacted sequence and candidate item set.
% \subsubsection{With demonstrations}
